Robust Combiners and Universal Constructions for Quantum Cryptography

A robust combiner combines many candidates for a cryptographic primitive and generates a new candidate for the same primitive. Its correctness and security hold as long as one of the original candidates satisfies correctness and security. A universal construction is a closely related notion to a robust combiner. A universal construction for a primitive is an explicit construction of the primitive that is correct and secure as long as the primitive exists. It is known that a universal construction for a primitive can be constructed from a robust combiner for the primitive in many cases. Although robust combiners and universal constructions for classical cryptography are widely studied, robust combiners and universal constructions for quantum cryptography have not been explored so far. In this work, we define robust combiners and universal constructions for several quantum cryptographic primitives including one-way state generators, public-key quantum money, quantum bit commitments, and unclonable encryption, and provide constructions of them. On a different note, it was an open problem how to expand the plaintext length of unclonable encryption. In one of our universal constructions for unclonable encryption, we can expand the plaintext length, which resolves the open problem.

==> Old_Commit.tex <==
% !TEX root = main.tex
\section{Robust Canonical Quantum Commitment Combiner}
\begin{definition}[Robust Canonical Quantum Commitment Combiner]
    Let $\{\Sigma_i\seteq\{Q_{i,0}(\secp),Q_{i,1}(\secp)\}_{\secp\in\N}\}_{i\in [n(\secp)]}$ be $n$-candidates of canonical quantum commitments.
    A robust canonical quantum commitment combiner is a sequence of QPT unitaries $\{Q_0(\secp),Q_1(\secp)\}_{\secp\in\N}$ acting on the registers $(C,R)$ generated by a classical Turing machine $\cM$ that takes as input $(1^\secp,\{Q_{i,0}(\secp),Q_{i,1}(\secp)\}_{i\in[N]})$, and halts within $\poly(\secp,\abs{\{Q_{i,0}(\secp),Q_{i,1}(\secp)\}_{i\in[N]}})$ steps.
    We require that $\{Q_0(\secp),Q_1(\secp)\}_{\secp\in\N}$ satisfies the following properties:
    \paragraph{Statistical Binding.}
    For all sufficiently large $\secp\in\N$,
    \begin{align}
        \norm{(\bra{0}Q_1^{\dagger}(\secp))_{\mathbf{CR}} (I_{\mathbf{C}}\otimes U_{\mathbf{RZ}})(Q_0(\secp)\ket{0}_{\mathbf{CR}}\ket{\tau}_{\mathbf{Z}}) }\leq \negl(\secp).
    \end{align}
    \paragraph{Computational Hiding.}
    If one of $\{\Sigma_i\}_{i\in[n]}$ satisfies either (computationally hiding, statistically binding) or (statistically hiding, computationally binding), then 
    $\Tr_{\mathbf{R}}(Q_0\ket{0}_{\mathbf{CR}})$ is $\negl(\secp)$-computationally indistinguishable from $\Tr_{\mathbf{R}}(Q_1\ket{0}_{\mathbf{CR}})$ for all sufficiently large $\secp\in\N$.
\end{definition}

In this section, we show the \cref{thm:combiner_com}.
\begin{theorem}\label{thm:combiner_com}
    There exists a robust canonical quantum commitments combiner.
\end{theorem}
First, let us introduce the following \cref{lem:amp_binding_com}.
\begin{lemma}\label{lem:amp_binding_com}
    Let $\Sigma=\{Q_0(\secp),Q_1(\secp)\}_{\secp\in\N}$ be a candidate of a canonical quantum commitment. There exists a canonical quantum commitment $\Sigma^*\seteq \{Q_0^*(\secp),Q_1^*(\secp)\}_{\secp\in\N}$ such that:
    \begin{enumerate}
        \item $\Sigma^*$ satisfies statistically-binding.
        \item If $\Sigma$ satisfies either $\{\mbox{computaiontally binding},\mbox{statistically hiding}\}$ or $\{\mbox{statistically binding},\mbox{computationally hiding}\}$, then $\Sigma^*$ satisfies computationally hiding.
    \end{enumerate}
\end{lemma}


The proof of \cref{lem:amp_binding_com} consists of \cref{lem:converting_flavor} and \cref{lem:amp}.
\begin{lemma}[Converting Flavors:\cite{EC:HMY23}]\label{lem:converting_flavor}
Let $\{Q_0(\secp),Q_1(\secp)\}_{\secp\in\N}$ be a candidate of canonical quantum commitment.
Let $\{\widetilde{Q_{0}}(\secp),\widetilde{Q_{1}}(\secp)\}_{\secp\in\N}$ be a candidate of canonical quantum commitment described as follows:
\begin{itemize}
    \item The role of commitment and reveal registers are swapped from $(Q_{0}(\secp),Q_{1}(\secp))$ and the commitment register is augmented by an additional one-qubit register which we denote $\mathbf{D}$.
    In other words, if $\mathbf{C}$ and $\mathbf{R}$ are the commitment and reveal registers of $(Q_{0}(\secp),Q_{1}(\secp))$, then the commitment and reveal registers of $(\widetilde{Q_{0}}(\secp),\widetilde{Q_{1}}(\secp))$ are defined as $\widetilde{\mathbf{C}}\seteq (\mathbf{R},\mathbf{D})$ and $\widetilde{\mathbf{R}}\seteq \mathbf{C}$, where $\mathbf{D}$ is an additional one-qubit register.
    \item For $b\in\bit$, the unitary $\widetilde{Q_b}(\secp)$ is defined as follows:
    \begin{align}
        \widetilde{Q_{b}}(\secp)\seteq \left(Q_{0}(\secp)\otimes \ket{0}\bra{0}_{\mathbf{D}}+Q_{1}(\secp)\otimes \ket{1}\bra{1}_{\mathbf{D}}\right)\left(I_{\mathbf{RC}}\otimes Z^b_{\mathbf{D}}H_{\mathbf{D}}\right).
    \end{align}
\end{itemize}
The following holds for $X,Y\in\{\mbox{statistically, computationally}\}$.
\begin{enumerate}
\item 
If $(Q_{0}(\secp),Q_{1}(\secp))$ satisfies $c$-$X$ hiding, then $(\widetilde{Q_{0}},\widetilde{Q_{1}})$ satisfies $\sqrt{c}$-$X$ binding.
\item
If $(Q_{0}(\secp),Q_{1}(\secp))$ satisfies $\negl(\secp)$-$Y$ binding, then $(\widetilde{Q_{0}}(\secp),\widetilde{Q_{1}}(\secp))$ satisfies $\negl(\secp)$-$Y$ hiding.
\end{enumerate}
\end{lemma}

\begin{remark}
The previous work \cite{EC:HMY23} considered the case where the original commitment $(Q_0,Q_1)$ satisfies $\negl(\secp)$-$X$ hiding. 
However, for our purpose, we need to analyze the case where the original commitment $(Q_0,Q_1)$ does not satisfy $\negl(\secp)$-X hiding but $c$-X hiding for some constant $c$ instead.
Remark that we can prove the statement in the same way as the previous work. For the reader's convenience, we describe the proof in \cref{sec:convert}.
\end{remark}

\begin{lemma}[Amplifying Binding]\label{lem:amp}
    Let $\{Q_{0}(\secp),Q_{1}(\secp)\}_{\secp\in\N}$ be uniform QPT unitaries.
    Let $\{Q_{0}^*(\secp),Q_{1}^*(\secp)\}_{\secp\in\N}$ be uniform QPT unitaries described as follows:
    \begin{itemize}
        \item If $\mathbf{C}$ and $\mathbf{R}$ are the commitment and reveal registers of $(Q_{0}(\secp),Q_{1}(\secp))$, and $\mathbf{\widetilde{C}}$ and $\mathbf{\widetilde{R}}$ are the commitment and reveal registers of $(\widetilde{Q_{0}}(\secp),\widetilde{Q_{1}}(\secp))$, then the commitment and reveal registers of $(Q^*_{0}(\secp),Q_{1}^*(\secp))$ are defined as $\mathbf{C}^*\seteq \left(\mathbf{C}^{\otimes \secp},\mathbf{\widetilde{C}}^{\otimes \secp} \right)$, and $\mathbf{R^*}\seteq \left(\mathbf{R}^{\otimes \secp},\widetilde{\mathbf{R}}^{\otimes \secp}\right)$.
        \item For $b\in\bit$, the unitary $Q_b(\secp)$ is defined as follows:
        \begin{align}
            Q_{b}^*(\secp)\seteq (Q_{b}(\secp)\otimes \widetilde{Q_{b}}(\secp))^{\otimes \secp}.
        \end{align}
    \begin{enumerate}
        \item $(Q_{0}^*(\secp),Q_{1}^*(\secp))$ satisfies statistically binding.
        \item If $(Q_{0}(\secp),Q_{1}(\secp))$ satisfies either (statistically hiding, computationally binding) or (computationally hiding, statistically binding), then $(Q_{0}^*(\secp),Q_{1}^*(\secp))$ satisfies computationally hiding.
    \end{enumerate}
    \end{itemize}
\end{lemma}
\begin{proof}[Proof of \cref{lem:amp}]
Below, we fix the security parameter $\secp$, and write $(Q_0,Q_1)$, $(\widetilde{Q_0},\widetilde{Q_1})$ and $(Q_0^*,Q_1^*)$ to mean $(Q_0(\secp),Q_1(\secp))$, $(\widetilde{Q_0}(\secp),\widetilde{Q_1}(\secp))$ and $(Q_0^*(\secp),Q_1^*(\secp))$, respectively. 
\paragraph{Proof of the first item}
    We define 
\begin{align}
    \rho_{b}\seteq\Tr_{\mathbf{R}}(Q_{b}\ket{0}_{\mathbf{C,R}})\mbox{\,\,\,and\,\,\,}
    \widetilde{\rho_{b}}\seteq \Tr_{\mathbf{\widetilde{R}}}(\widetilde{Q_{b}}\ket{0}_{\mathbf{\widetilde{C},\widetilde{R}}})\mbox{\,\,\,and\,\,\,}\rho_b^*\seteq \Tr_{\mathbf{R^*}}(Q_b^*\ket{0}_{\mathbf{C^*,R^*}})
\end{align}
From the construction of $Q_0^*$ and $Q_1^*$, we have
\begin{align}
    \rho_b\otimes \widetilde{\rho_b}\seteq \Tr_{\mathbf{R^*}}(Q_b^*\ket{0}_{\mathbf{C^*,R^*}})
\end{align}
Let $0\leq f\leq 1$ be a constant such that 
\begin{align}
    F(\rho_{0},\rho_{1})=f.
\end{align}

We have
\begin{align}
    \mathsf{TD}(\rho_{0},\rho_{1})\leq \sqrt{1-F(\rho_{0},\rho_{1})}\leq \sqrt{1-f}.
\end{align}
In particular, this implies that $(Q_{0},Q_{1})$ satisfies $\sqrt{1-f}$-statistically hiding.
From \cref{lem:converting_flavor}, this implies that $(\widetilde{Q_{0}},\widetilde{Q_{1}})$ satisfies $(1-f)^{1/4}$-statistically binding.
Furthermore, this implies that
\begin{align}
    F(\widetilde{\rho_{0}},\widetilde{\rho_{1}})\leq (1-f)^{1/2},
\end{align}
which we prove later.



Therefore, we have
\begin{align}
    &F(\rho_0^*,\rho_1^*)=F\left((\rho_{0}\otimes\widetilde{\rho_{0}})^{\otimes \secp},(\rho_{1}\otimes\widetilde{\rho_{1}})^{\otimes \secp}\right)
    \leq F(\rho_{0},\rho_{1})^{\secp}F(\widetilde{\rho_{0}},\widetilde{\rho_{1}})^{\secp}\leq f^\secp(1-f)^{\secp/2}\leq 2^{-\secp/2},
\end{align}
which implies that $(Q_{0}^*,Q_{1}^*)$ satisfies statistically binding.

\taiga{It might be OK to skip the explanation red part below.}
\color{red}
Now, we show that if $(\widetilde{Q_{0}},\widetilde{Q_{1}})$ satisfies $(1-f)^{1/4}$-statistically binding, then
$
    F(\widetilde{\rho_{0}},\widetilde{\rho_{1}})\leq (1-f)^{1/2}.
$
For contradiction, assume that 
$
    F(\widetilde{\rho_{0}},\widetilde{\rho_{1}})>(1-f)^{1/2},
$
and then show that $(\widetilde{Q_{0}},\widetilde{Q_{1}})$ does not satisfies $(1-f)^{1/4}$-statistically binding.
From the Uhlmann's Theorem, there exists some unitary $U_{\mathbf{\widetilde{R}}}$ acting on the register $\mathbf{\widetilde{R}}$ such that
\begin{align}
F(\widetilde{\rho_{0}},\widetilde{\rho_{1}})=
\abs{\bra{0}_{\mathbf{\widetilde{C},\widetilde{R}}}\widetilde{Q_0}^{\dagger}(I_{\mathbf{\widetilde{C}}}\otimes U_{\mathbf{\widetilde{R}}})\widetilde{Q_1}\ket{0}_{\mathbf{\widetilde{C},\widetilde{R}}}}^2>(1-f)^{1/2}.
\end{align}
Now, we have
\begin{align}
    &\norm{\left(\bra{0}_{\mathbf{\widetilde{C},\widetilde{R}}}\widetilde{Q_0}^{\dagger}\otimes I_{\mathbf{\widetilde{C},\widetilde{Z}}}\right)(I_{\mathbf{\widetilde{C},\widetilde{Z}}}\otimes U_{\mathbf{\widetilde{R}}})\widetilde{Q_1}\ket{0}_{\mathbf{\widetilde{C},\widetilde{R}}}\ket{\tau}_{\mathbf{\widetilde{Z}}}}\\
    &=\norm{\left(\bra{0}_{\mathbf{\widetilde{C},\widetilde{R}}}\widetilde{Q_0}^{\dagger}(I_{\mathbf{\widetilde{C}}}\otimes U_{\mathbf{\widetilde{R}}})\widetilde{Q_1}\ket{0}_{\mathbf{\widetilde{C},\widetilde{R}}}\right) \ket{\tau}_{\mathbf{\widetilde{Z}}}}
    =\abs{\bra{0}_{\mathbf{\widetilde{C},\widetilde{R}}}\widetilde{Q_0}^{\dagger}(I_{\mathbf{\widetilde{C}}}\otimes U_{\mathbf{\widetilde{R}}})\widetilde{Q_1}\ket{0}_{\mathbf{\widetilde{C},\widetilde{R}}}}>(1-f)^{\frac{1}{4}},
\end{align}
which contradicts that$(\widetilde{Q_{0}},\widetilde{Q_{1}})$ satisfies $(1-f)^{1/4}$-statistically binding.
\color{black}





\paragraph{Proof of the second item.}
We prove that $(Q_{0}^*,Q_{1}^*)$ satisfies computationally hiding if $(Q_0,Q_1)$ satisfies either (statistically binding, computationally hiding) or (computationally\ hiding, statistically binding).
Assume that $(Q_{0},Q_{1})$ satisfies both computationally hiding and statistically binding, and thus $(\widetilde{Q}_0,\widetilde{Q}_1)$ satisfies statistically hiding and computationally binding.
In that case, we can reduce the computational hiding of $(Q_{0}^*,Q_{1}^*)$ to that of $(Q_{0},Q_{1})$ and statistically-hiding of $(\widetilde{Q}_0,\widetilde{Q}_1)$ by a standard hybrid argument.
On the other hand, if $(Q_{0},Q_{1})$ satisfies both statistically hiding and computationally binding, then $(\widetilde{Q_{0}},\widetilde{Q_{1}})$ satisfies both computationally hiding and statistically binding.
In that case, we can reduce the computationally hiding of $(Q_{0}^*,Q_{1}^*)$ to that of $(\widetilde{Q_{0}},\widetilde{Q_{1}})$ and statistically-hiding of $(Q_0,Q_1)$ by a standard hybrid argument.






\end{proof}







\begin{proof}[Proof of \cref{thm:combiner_com}]


For a candidate of canonical quantum commitment scheme $\Sigma_i\seteq \{Q_{i,0}(\secp),Q_{i,1}(\secp)\}_{\secp\in\N}$, let $\Sigma_i^*\seteq \{Q_{i,0}^*(\secp),Q_{i,1}^*(\secp)\}_{\secp\in\N}$ be a canonical quantum commitment such that 
\begin{enumerate}
    \item $\Sigma_i^*$ satisfies statistically binding.
    \item $\Sigma_i^*$ satisfies computational hiding if $\Sigma_i$ satisfies either (statistically hiding, computationally binding) or (computationally hiding, statistically binding).
\end{enumerate}
Note that such a canonical quantum commitment is obtained from \cref{lem:amp_binding_com}.


We construct a robust canonical quantum commitment combiner
$\Comb.\Sigma\seteq \{\Comb.Q_0(\secp),\Comb.Q_1(\secp)\}_{\secp\in\N}$ as follows:
\begin{itemize}
    \item If $\mathbf{C_{i}^*}$ and $\mathbf{R_{i}^*}$ are the commitment register and the reveal register, then the commitment and reveal registers of $(Q_{i,0}^*(\secp),Q_{i,1}^*(\secp))$, then the commitment and reveal register of $(\Comb.Q_0(\secp),\Comb.Q_1(\secp))$ are defined as $\mathbf{C}\seteq \{\mathbf{C_i^*}\}_{i\in[n]}$ and $\mathbf{R}=(\{\mathbf{R_i^*}\}_{i\in[n]},\{\mathbf{D_i^*}\}_{i\in[n]})$, where $\mathbf{D_i^*}$ is an additional one-qubit register for $i\in[n]$.
    \item For $b\in\bit$, the unitary $Q_b$ is defined as follows:
    \begin{align}
        \Comb.Q_b(\secp)\seteq\left(\sum_{r\in\bit^n}\bigotimes_{i\in[n]} (Q^*_{i,r_i}(\secp)\otimes \ket{r_i}\bra{r_i}_{\mathbf{D_i^*}})\right)\left(\bigotimes_{i\in[n]}I_{\mathbf{C_i^*,R_i^*}}\otimes X^b_{\mathbf{D_1^*}}\bigotimes_{i\in[n]}  \mathsf{CNOT}_{\mathbf{D_1^*,D_i^*}}\bigotimes_{i\in\{2,\cdots,n\}} H_{\mathbf{D_i^*}}\right).
    \end{align}
    Here, $\mathsf{CNOT}_{\mathbf{D_1^*,D_i^*}}$ is a CNOT gate, where $\mathbf{D_1^*}$ is a target register and $\mathbf{D_i^*}$ is a control register.
\end{itemize}
Note that we have
\begin{align}
    \Comb.Q_b(\secp)\ket{0}_{\mathbf{C,R}}=\frac{1}{2^{(n-1)/2}}\sum_{\{r: \sum_{i\in[n]}r_i=b\}}\bigotimes_{i\in[n]}(Q_{i,r_i}^*(\secp)\ket{0}_{\mathbf{C_i^*,R_i^*}}\otimes \ket{r_i}_{\mathbf{D_i^*}}).
\end{align}
Obviously, $\Comb.Q_b(\secp)$ can be obtained by some classical Turing machine $\cM$ that takes as input $(1^\secp,\abs{\{Q_{i,0}(\secp),Q_{i,1}(\secp)\}_{i\in[N]}})$, and halts within $\poly(\secp,\abs{\{ Q_{i,0},Q_{i,1}\}_{i\in[N]}})$ steps.
Furthermore, we have the following \cref{thm:binding,thm:preserve}, which we prove later.
Therefore, \cref{thm:combiner_com} holds.
\begin{lemma}\label{thm:binding}
    $\Comb.\Sigma$ satisfies statistically binding.
\end{lemma}
\begin{lemma}\label{thm:preserve}
    If one of $\{\Sigma_i\}_{i\in[n]}$ satisfies (computationally hiding, statistically binding) or (statistically hiding, computationally binding), then $\Comb.\Sigma$ satisfies computationally hiding.
\end{lemma}
\end{proof}

\begin{proof}[Proof of \cref{thm:binding}]
    Below, we fix security parameter $\secp$, and write $\{Q_{i,0}^*,Q_{i,1}^*\}_{i\in[N]}$ and $(\Comb.Q_0,\Comb.Q_1)$ to mean $\{Q_{i,0}^*(\secp),Q_{i,1}^*(\secp)\}_{i\in[N]}$ and $(\Comb.Q_0(\secp),\Comb.Q_1(\secp) )$, respectively.
    From \cref{lem:amp}, all $\Sigma_i^*$ satisfies statistical binding.
    This implies that if we write ${\rho_{i,b}^*}_{\mathbf{C_i}}\seteq \Tr(Q^*_{i,b}\ket{0}_{\mathbf{C_i,R_i}})$, then $\mathsf{TD}(\rho_{i,0}^*,\rho_{i,1}^*)\geq 1-\negl(\secp)$.
    Then, there exists a two-outcome POVM measurement $\{\Pi_{i,0}^*,\Pi_{i,1}^*\}$ such that
    \begin{align}
        \Tr\left(\Pi_{i,0}^*(\rho_{i,0}^*-\rho_{i,1}^*)\right)=\Tr\left(\Pi_{i,1}^*(\rho_{i,0}^*-\rho_{i,1}^*)\right)\geq 1-\negl(\secp).
    \end{align}
    We write $\Comb.\rho_b\seteq \Tr_{\mathbf{R}}(\Comb.Q_b\ket{0}_{\mathbf{C,R}})$ and write $R$ to mean $\sum_{i\in[n]}r_i$.
    Note that we have 
    \begin{align}
        \Comb.\rho_b= \frac{1}{2^{n-1}}\sum_{\{r:R=b \}}\bigotimes_{i\in[n]}\rho_{i,r_i}^*.
    \end{align}
    Now, we show that 
    \begin{align}
    \mathsf{TD}(\Comb.\rho_0,\Comb.\rho_1)\geq 1-\negl(\secp).
    \end{align}
    For that, it is sufficient to show that there exists a POVM measurement that distinguishes $\Comb.\rho_0$ from $\Comb.\rho_1$.
    
    We introduce a two-outcome POVM measurement $\{\Comb.\Pi_0\seteq\sum_{\{r:R=0\}}\bigotimes_{i\in[n]}\Pi_{i,r_i}^*,\Comb.\Pi_1\seteq\sum_{\{r:R=1\}}\bigotimes_{i\in[n]}\Pi_{i,r_i}^*\}$.
    Then, we have
    \begin{align}
        \mathsf{TD}(\Comb.\rho_0,\Comb.\rho_1)&\geq\Tr(\Comb.\Pi_0(\Comb.\rho_0-\Comb.\rho_1))\\
        &=
        \frac{1}{2^{n-1}}\Tr(\Comb.\Pi_0\left(\sum_{\{r:R=0\}}\bigotimes_{i\in[n]}\rho_{i,r_i}^*-\sum_{\{r:R=1\}}\bigotimes_{i\in[n]}\rho_{i,r_i}^*\right))\\
        &=\frac{1}{2^{n-1}}\Tr(\Comb.\Pi_0\bigotimes_{i\in[n]}\left(\rho^*_{i,0}-\rho_{i,1}^*\right))\\
        &=\frac{1}{2^{n-1}}\Tr(\left(\sum_{\{r:R=0\}}\bigotimes_{i\in[n]}\Pi^*_{i,r_i}\right)\left(\bigotimes_{i\in[n]}\rho^*_{i,0}-\rho_{i,1}^*\right))\\
        &=\frac{1}{2^{n-1}}\Tr(\sum_{\{r:R=0\}}\left(\bigotimes_{i\in[n]}\Pi^*_{i,r_i}\left(\rho^*_{i,0}-\rho_{i,1}^*\right)\right))\\
        &=\frac{1}{2^{n-1}}\sum_{\{r:R=0\}}\Tr(\bigotimes_{i\in[n]}\Pi^*_{i,r_i}\left(\rho^*_{i,0}-\rho_{i,1}^*\right))\\
        &=\frac{1}{2^{n-1}}\sum_{\{r:R=0\}}\prod_{i\in[n]}\Tr(\Pi^*_{i,r_i}\left(\rho^*_{i,0}-\rho_{i,1}^*\right))\\
       &=\prod_{i\in[n]}\Tr(\Pi^*_{i,0}\left(\rho^*_{i,0}-\rho_{i,1}^*\right))\geq (1-\negl(\secp))^n\geq 1-n\cdot\negl(\secp). 
    \end{align}
    Here, we have used that $\Tr(A+B)=\Tr(A)+\Tr(B)$ in the fifth equation, and in the sixth equation we have used $\Tr(A\otimes B)=\Tr(A)\Tr(B)$, and we have used that
    \begin{align}
        \Tr(\Pi_{i,0}^*(\rho_{i,0}^*-\rho_{i,1}^*) )=\Tr(\Pi_{i,1}^*(\rho_{i,0}^*-\rho_{i,1}^*))
    \end{align}
    for all $i\in[n]$ in the final equation.
    
    Furthermore, we have
    $F(\Comb.\rho_0,\Comb.\rho_1)\leq 1-\mathsf{TD}(\Comb.\rho_0,\Comb.\rho_1)^2\leq 2n\cdot\negl(\secp)$.
    From Uhlmann's theorem, this implies that $\Comb.\Sigma$ satisfies statistical binding.
\end{proof}


\begin{proof}[Proof of \cref{thm:preserve}]
    Below, we fix security parameter $\secp$, and write $\{Q_{i,0}^*,Q_{i,1}^*\}_{i\in[N]}$ and $(\Comb.Q_0,\Comb.Q_1)$ to mean $\{Q_{i,0}^*(\secp),Q_{i,1}^*(\secp)\}_{i\in[N]}$ and $(\Comb.Q_0(\secp),\Comb.Q_1(\secp) )$, respectively.
    Let us show that $\Comb.\Sigma$ satisfies computationally hiding.
    Let us assume that $\Sigma_{x}$ satisfies either (computationally hiding, statistically binding) or (statistically binding, computationally hiding). Then, from \cref{lem:amp}, $\Sigma_{x}^*$ satisfies computationally hiding.
    Let us describe the sequence of a hybrid experiment against QPT adversary $\cA$.
    \begin{description}
        \item[$\mathsf{Hyb}_0(b)$:]This is the original hiding experiment of $\Comb.\Sigma$.
        \begin{enumerate}
            \item The challenger sends $\Comb.\rho_b$ to $\cA$.
            \item $\cA$ outputs $b^*$.
        \end{enumerate}
        \item[$\mathsf{Hyb}_1(b)$:]$ $
        \begin{enumerate}
            \item The challenger randomly samples $r_{i}\la\bit$ for all $i\in[n]\backslash x$. We
            write $R$ to mean $\sum_{i\in[n]\backslash x}r_i$
            \item The challenger sends $\rho_{1,r_1}^*\otimes \cdots \otimes\rho_{x-1,r_{x-1}}^*\otimes \rho_{x,R+b}^*\otimes \rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*$ to $\cA$.
            \item $\cA$ outputs $b^*$.
        \end{enumerate}
        \item[$\mathsf{Hyb}_2(b)$:] $ $
        \begin{enumerate}
            \item The challenger randomly samples $r_i\la\bit$ for all $i\in[n]\backslash x$.
            \item The challenger sends $\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^* \otimes\rho_{x+1,r_{x+1}}^* \otimes\cdots\otimes\rho_{n,r_{n}}^*$.
            \item $\cA$ outputs $b^*$.
        \end{enumerate}
    \end{description}
    We have the following \cref{prop:hyb_0_hyb_1_com,prop:hyb_1_hyb_2_com,prop:hyb_2_com}. Therefore, we have
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_0(0)=1]-\Pr[\mathsf{Hyb}_0(1)=1]}\leq \negl(\secp),
    \end{align}
    which implies that $\Comb,\Sigma$ satisfies computationally hiding.
    \begin{proposition}\label{prop:hyb_0_hyb_1_com}
        $\Pr[\mathsf{Hyb}_0(b)=1]=\Pr[\mathsf{Hyb}_1(b)=1]$ for $b\in\bit$.
    \end{proposition}
    \begin{proposition}\label{prop:hyb_1_hyb_2_com}
        If $\Sigma_x^*$ satisfies computationally hiding, then 
        \begin{align}
            \abs{\Pr[\mathsf{Hyb}_1(b)=1]-\Pr[\mathsf{Hyb}_2(b)=1]}\leq \negl(\secp)
        \end{align}
        for each $b\in\bit$.
    \end{proposition}
    \begin{proposition}\label{prop:hyb_2_com}
        $\Pr[\mathsf{Hyb}_2(0)=1]=\Pr[\mathsf{Hyb}_2(1)=1]$.
    \end{proposition}
    
    \cref{prop:hyb_0_hyb_1_com,prop:hyb_2_com} trivially follows, and thus we omit the proof.

\begin{proof}[Proof of \cref{prop:hyb_1_hyb_2_com}]
    For simplicity, we write $\sum_r$ to mean that $\sum_{\{r:r_i\in\bit\mbox{\,\,for\,\,} i\in[n]\backslash x\}} $, and remind that $R\seteq \sum_{i\in[n]\backslash x}r_i$.
    We show that 
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1(0)=1]-\Pr[\mathsf{Hyb}_2(0)=1]}\leq \negl(\secp).
    \end{align}

    
    We have
    \begin{align}
        &\Pr[\mathsf{Hyb}_1(0)=1]-\Pr[\mathsf{Hyb}_2(0)=1]\\
        &=\frac{1}{2^{n-1}}\sum_{r}\left(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,R}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\right)\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\frac{1}{2^{n-1}}\sum_{r}\left(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\right)\\
        &=\frac{1}{2^{n-1}}\sum_{r}\bigg(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,R}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\bigg)\\
        &=\frac{1}{2^{n-1}}\sum_{\{r:R=1\}}\bigg(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\bigg)
        \\
        &=\frac{1}{2^{n-1}}\sum_{\{r:R=1\}}\bigg(\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\bigg).
    \end{align}
    For showing a contradiction, assume that there exists some  polynomial $p$ and an adversary $\cA$ such that
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1(0)=1]-\Pr[\mathsf{Hyb}_2(0)=1]}\geq  1/p(\secp),
    \end{align}
    and then construct an algorithm $\cB_x$ that breaks the hiding of $\Sigma_x^*$.
    \begin{enumerate}
        \item $\cB_x$ receives $\rho_{x,b}^*$ from the challenger of $\Sigma_x^*$, where $b$ is randomly sampled from $\bit$.
        \item $\cB_x$ randomly samples $r_i\la\bit$ for all $i\in[n]\backslash x$.
        \item $\cB_x$ sends $\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,b}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^* $ to $\cA$.
        \item $\cB_x$ receives $b^*$ from $\cA$.
        \item $\cB_x$ outputs $b^*+1$ if $R=1$, and outputs $0$ otherwise, where $R= \sum_{i\in[n]\backslash x}r_i$.
    \end{enumerate}
    We compute $\abs{\Pr[1\la\cB:b=0]-\Pr[1\la\cB:b=1]}$.
    It holds that
    \begin{align}
        &\abs{\Pr[1\la\cB:b=0]-\Pr[1\la\cB:b=1]}\\
        &=\frac{1}{2}\abs{\Pr[0\la\cA: b=0,R=1]-\Pr[0\la\cA:b=1,R=1]}\\
        &=\frac{1}{2^{n}}\Bigg|\sum_{\{r:R=1\}}\left(\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\right)\\
        &-\sum_{\{r:R=1\}}\left(\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\right) \Bigg|\\
        &=\frac{1}{2^{n}}\Bigg|\sum_{\{r:R=1\}}\bigg(\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\\
        &-\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\bigg)\Bigg|\\
        &=\frac{1}{2}\abs{\Pr[\mathsf{Hyb}_1(0)=1]-\Pr[\mathsf{Hyb}_2(0)=1]}.
    \end{align}
    This implies that if $\abs{\Pr[\mathsf{Hyb}_1(0)=1]-\Pr[\mathsf{Hyb}_2(0)=1]}\geq 1/p(\secp)$ for some polynomial, then $\cB$ breaks the computationally hiding of $\Sigma_x^*$.

In a similar way, we can prove that
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1(1)=1]-\Pr[\mathsf{Hyb}_2(1)=1]}\leq \negl(\secp).
    \end{align}
\end{proof}




\if0
\begin{proof}[Proof of \cref{prop:hyb_1_hyb_2_com}]
    For simplicity, we write $\sum_r$ to mean that $\sum_{\{r:r_i\in\bit\mbox{\,\,for\,\,} i\in[n]\backslash x\}} $, and remind that $R\seteq \sum_{i\in[n]\backslash x}r_i$.
    
    We have
    \begin{align}
        &\Pr[\mathsf{Hyb}_1(0)=1]-\Pr[\mathsf{Hyb}_2(0)=1]\\
        &=\frac{1}{2^{n-1}}\sum_{r}\left(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,R}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\right)\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\sum_{r}\left(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\right)\\
        &=\frac{1}{2^{n-1}}\sum_{r}\bigg(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,R}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\bigg)\\
        &=\frac{1}{2^{n-1}}\sum_{\{r:R=1\}}\bigg(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\bigg)
        \\
        &=\frac{1}{2^{n-1}}\sum_{\{r:R=1\}}\bigg(\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\bigg).
    \end{align}
    Similarly, we have
    \begin{align}
        &\Pr[\mathsf{Hyb}_1(1)=1]-\Pr[\mathsf{Hyb}_2(1)=1]\\
        &=\frac{1}{2^{n-1}}\sum_{\{r:R=0\}}\bigg(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\\
        &\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,-\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes \rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^*\otimes\rho_{x+1,r_{x+1}}^*\otimes \cdots\otimes \rho_{n,r_n}^*) ]\bigg).
    \end{align}
    For showing a contradiction, assume that there exists a non-negligible $p$ and an adversary $\cA$ such that either
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1(0)=1]-\Pr[\mathsf{Hyb}_2(0)=1]}\geq p(\secp)
    \end{align}
    or
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1(1)=1]-\Pr[\mathsf{Hyb}_2(1)=1]}\geq p(\secp),
    \end{align}
    and then construct an algorithm $\cB$ that breaks the hiding of $\Sigma_x^*$.
    \begin{enumerate}
        \item $\cB$ receives $\rho_{x,b}^*$ from the challenger of $\Sigma_x^*$, where $b$ is randomly sampled from $\bit$.
        \item $\cB$ randomly samples $r_i\la\bit$ for all $i\in[n]\backslash x$.
        \item $\cB$ sends $\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,b}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^* $ to $\cA$.
        \item $\cB$ receives $b^*$ from $\cA$.
        \item $\cB$ outputs $b^*+R$, where $R\seteq \sum_{i\in[n]\backslash x}r_i$.
    \end{enumerate}
    We compute $\abs{\Pr[1\la\cB:b=0]-\Pr[1\la\cB:b=1]}$.
    It holds that
    \begin{align}
        &\abs{\Pr[1\la\cB:b=0]-\Pr[1\la\cB:b=1]}\\
        &=\abs{\Pr[\left(1+R\right)\la\cA: b=0]-\Pr[\left(1+R\right)\la\cA:b=1]}\\
        &=\frac{1}{2^{n-1}}\Bigg|\sum_{r}\left(\Pr[\left(1+R\right)\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\right)\\
        &-\sum_{r}\left(\Pr[\left(1+R\right)\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\right) \Bigg|\\
        &=\frac{1}{2^{n-1}}\Bigg|\sum_{\{r:R=0\}}\bigg(\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\\
        &-\Pr[1\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\bigg)\\
        &+\sum_{\{r:R=1\}}\bigg(\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,0}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\\
        &-\Pr[0\la\cA(\rho_{1,r_1}^*\otimes\cdots\otimes\rho_{x-1,r_{x-1}}^*\otimes\rho_{x,1}^* \otimes\rho_{x+1,r_{x+1}}^*\otimes\cdots \otimes\rho_{n,r_n}^*)]\bigg) \Bigg|\\
        &=\abs{\left(\Pr[\mathsf{Hyb}_1(1)=1]-\Pr[\mathsf{Hyb}_2(1)=1]\right)+\left(\Pr[\mathsf{Hyb}_1(0)=1]-\Pr[\mathsf{Hyb}_2(0)=1]\right)}.
    \end{align}
    This implies that if either $\abs{\Pr[\mathsf{Hyb}_2(1)=1]-\Pr[\mathsf{Hyb}_1(1)=1]}$ or $\abs{\Pr[\mathsf{Hyb}_2(0)=1]-\Pr[\mathsf{Hyb}_1(0)=1]}$ is non-negligible.
\end{proof}
\fi

\end{proof}





\subsection{Universal Construction}
\begin{definition}
    We say that a sequence of uniform QPT unitary $\Sigma_{\mathsf{Univ}}=\{Q_0(\secp),Q_1(\secp)\}_{\secp\in\N}$ is a universal construction of canonical quantum commitment when $\Sigma_{\mathsf{Univ}}$ is canonical quantum commitment if there exists canonical quantum commitment.
\end{definition}

\begin{theorem}\label{thm:univ_com}
    There exists a universal construction of canonical quantum commitment.
\end{theorem}
The proof is almost the same as \cref{thm:univ_owsg}, and thus we skip the proof.

==> Old_Money.tex <==

\if0
\section{Robust Mini-Scheme Combiner}
\begin{definition}[Robust Mini-Scheme Combiner]
    Let $\{\Sigma_{i}\}_{i\in[n]}$ be $n$-candidates of mini-scheme promised that all $\{\Sigma_i\}_{i\in[n]}$ satisfy efficiency.
    A robust mini-scheme combiner $\Sigma$ consists of two algorithms $\Sigma\seteq(\Mint,\Vrfy)$ defined as follows:
    \begin{description}
        \item[$\Mint(1^\secp,\{\Sigma_i\}_{i\in[n]})$:]
        It takes as input a security parameter $1^\secp$, $\{\Sigma_i\}_{i\in[n]}$, and outputs a serial number $s$ and a quantum state $\rho_s$.
        \item[$\Vrfy(1^\secp,s,\rho,\{\Sigma_i\}_{i\in[n]})$:]
        It takes as input a security parameter $1^\secp$, $s$, $\rho$ and $\{\Sigma_i\}_{i\in[n]}$, and outputs $\top$ or $\bot$.
    \end{description}
    \paragraph{Efficiency.} $\Sigma\seteq (\Mint,\Vrfy)$ are uniform QPT algorithms.
    \paragraph{Correctness.} 
    For all security parameters $\secp\in\N$,
    \begin{align}
        \Pr[\top\la\Vrfy(1^\secp,s,\rho_s,\{\Sigma_i\}_{i\in[n]}): (s,\rho_s)\la\Mint(1^\secp,\{\Sigma_i\}_{i\in[n]})]\geq 1-\negl(\secp).
    \end{align}
    \paragraph{Security.}
    If at least one of the mini-scheme candidates $\{\Sigma_i\}_{i\in[n]}$ satisfies correctness and security, then $\Sigma$ satisfies 
    \begin{align}
        \Pr[\top\la\Vrfy(1^\secp,s,\sigma[1])\wedge \top\la\Vrfy(1^\secp,s,\sigma[2]):(s,\rho_s)\la\Mint(1^\secp,),\sigma\la\cA(\rho_s)]\leq\negl(\secp)
    \end{align}
    Here, $\sigma$ is a quantum state on $2$ registers, $R[1],R[2]$ each of which is of $\abs{\rho_s}$ qubits, and where $\sigma[1]\seteq \Tr_{R[2]}(\sigma)$ and $\sigma[2]\seteq \Tr_{R[1]}(\sigma)$.
\end{definition}






\begin{theorem}\label{thm:combiner_money}
    A robust mini-scheme combiner exists.
\end{theorem}
For proving \cref{thm:combiner_money}, we introduce the following \cref{lem:amp_cor_money}.
\begin{lemma}\label{lem:amp_cor_money}
    Let $\Sigma=(\mathsf{Mint},\Vrfy)$ be a candidate for mini-scheme.
    There exists a mini-scheme $\Sigma^*=(\mathsf{Mint}^*,\Vrfy^*)$ such that
    \begin{enumerate}
        \item If $\Sigma$ is a uniform QPT algorithm, then $\Sigma^*$ is a uniform QPT algorithm.
        \item $\Sigma^*$ satisfies correctness.
        \item If $\Sigma$ satisfies both correctness and security, then $\Sigma^*$ satisfies security.
    \end{enumerate}
\end{lemma}

\begin{proof}[Proof of \cref{lem:amp_cor_money}]
Let us describe $\Sigma^*$.
\begin{description}
    \item[$\Mint^*(1^\secp)$:]$ $
    \begin{itemize}
        \item Run $\mathsf{Check}(\Sigma)$, where $\mathsf{Check}$ works as follows:
        \begin{itemize}
        \item Run $(s_i,\rho_{s_i})\la\Mint(1^\secp)$ for all $i\in[\secp]$.
        \item Run $\Vrfy(1^\secp,s_i,\rho_{s_i})$ for all $i\in[\secp]$.
        \item Output $1$ if the number of $\top\la\Vrfy(1^\secp,s_i,\rho_{s_i})$ is at least $\frac{11\secp}{12}$, and output $0$ otherwise.
        \end{itemize}
        \item If $1\la\mathsf{Check}(\Sigma)$, then run $(s_i,\rho_{s_i})\la\Mint(1^\secp)$ for all $i\in[\secp]$ and output $s^*\seteq \{s_i\}_{i\in[\secp]} $ and $\rho_{s}^*\seteq \bigotimes_{i\in[\secp]}\rho_{s_i}$. 
        \item If $0\la\mathsf{Check}(\Sigma)$, then run $(s_i,\rho_{s_i})\la\Mint(1^\secp)$ for all $i\in[\secp]$ and output $s\seteq \top$ and $\rho_{s^*}\seteq \bigotimes_{i\in[\secp]}\rho_{s_i}$.
    \end{itemize}
    \item[$\Vrfy^*(1^\secp, s^*,\rho)$:]$ $ 
    \begin{itemize}
        \item Let $\rho$ be a quantum state on the $\secp$ registers $R[1]\cdots R[\secp]$. Let $\rho[i]\seteq \Tr_{R[1]\cdots R[i-1]R[i+1]\cdots R[\secp]}(\rho)$ for all $i\in[\secp]$.
        \item If $s^*= \top$, output $\top$.
        \item If $s^* \neq \top$, then parse $s^*= \{s_i\}_{i\in[\secp]}$ and run $\Vrfy(1^\secp,s_i,\rho[i])$ for all $i\in[\secp]$.
        Output $\top$ if the number of $\top\la\Vrfy(1^\secp,s_i,\rho[i])$ is at least $\frac{3\secp}{4}$.
    \end{itemize}
\end{description}
\paragraph{Proof of the first item.}
This trivially holds.

\paragraph{Proof of the second item.} 
First, assume that $\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]<5/6$, and compute $\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]$.
\begin{align}
    &\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\\
    &\geq\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 0\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\Pr[0\la\mathsf{Check}(\Sigma)]\\
    &\geq \Pr[0\la\mathsf{Check}(\Sigma)]\\
    &\geq 1-2\exp(-\secp/72)).
\end{align}
Here in the third inequality, we have used that 
$\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]<5/6$ and \cref{lem:hoefd}, which we will show later.

Next, assume that $\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]\geq 5/6$, and compute $\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]$.
\begin{align}
    &\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\\
    &\geq\bigg(\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 0\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\Pr[0\la\mathsf{Check}(\Sigma)]\\
    &+\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\Pr[1\la\mathsf{Check}(\Sigma)]\bigg)\\
    &= \Pr[0\la\mathsf{Check}(\Sigma)]+\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\Pr[1\la\mathsf{Check}(\Sigma)]\\
    &=1-\Pr[1\la\mathsf{Check}(\Sigma)]\left(1-\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\right)\\
    &\geq \Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\\
    &\geq 1-2\exp(-\secp/72)).
\end{align}
Here in the final inequality, we have used that $ \Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]\geq 5/6$ and \cref{lem:hoefd}, which we will prove later.
Therefore, the $\Sigma^*$ satisfies the correctness.

We will prove the skipped part.
Assume $\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]<5/6$ and show $\Pr[0\la\mathsf{Check}(\Sigma)]\geq 1-2\exp(-\secp/72)$.
We consider the random variable $X_{i}$ as $1$ if $\top\la\Vrfy(1^\secp,s_i,\rho_{s_i})$ for the $i$-th running of the verification algorithm while running $\mathsf{Check}$, and consider $X_i$ as $0$ if $\bot\la\Vrfy(1^\secp,s_i,\rho_{s_i})$. 
If we denote $S_{\secp}\seteq\sum_{i\in[\secp]}X_{i}$, then
$1\la\mathsf{Check}(\Sigma) $ if and only if $S_{\secp}\geq \frac{11\secp}{12}$.
On the other hand,
because $\Exp[S_{\secp}]<\frac{5\secp}{6}$, $\abs{S_{\secp}-\Exp[S_{\secp}]}\geq \frac{\secp}{12}$ must hold for $S_{\secp}\geq \frac{11\secp}{12}$.
Therefore, from \cref{lem:hoefd}, we have
\begin{align}
    \Pr[1\la\mathsf{Check}(\Sigma)]\leq \Pr[\abs{S_{\secp}-\Exp[S_{\secp}]}\geq \frac{\secp}{12}]\leq2\exp(-\frac{\secp}{72}).
\end{align}
In the same way, we can prove that 
\begin{align}
    \Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}):1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\geq 1-2\exp(-\secp/72)
\end{align}
when $\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]\geq 5/6$.




\paragraph{Proof of the third item.}
We prove that $\Sigma^*$ satisfies security if $\Sigma$ satisfies correctness and security.
Assume that there exists a QPT adversary $\cA$ that breaks the security of $\Sigma^*$, and then construct a QPT adversary $\cB$ that breaks $\Sigma$ as follows.
\begin{enumerate}
    \item $\cB$ receives $\rho_s$ from the challenger of $\Sigma$.
    \item $\cB$ samples $I\in[\secp]$, and sets $\rho_{s_I}\seteq \rho_s$.
    \item $\cB$ generates $(s_j,\rho_{s_j})\la\Mint(1^\secp)$ for all $j\in[\secp]\backslash I$, and sends $\bigotimes_{j\in[\secp]}\rho_{s_j}$ to $\cA$.
    \item $\cB$ receives $\sigma$ consisting of $2\secp$ registers $R[1],\cdots,R[2\secp]$. We write $\sigma[j]\seteq \Tr_{R[1]\cdots R[j-1]R[j+1]\cdots R[2\secp]}(\sigma)$ for all $j\in[\secp]$.
    \item $\cB$ runs $\Vrfy(1^\secp,s_i,\sigma[i])$ and $\Vrfy(1^\secp,s_i,\sigma[i+\secp])$ for all $i\in[\secp]\backslash I$.
    \item $\cB$ sends $\sigma[I]\otimes \sigma[I+\secp]$ to the challenger, and it computes $\Vrfy(1^\secp,s,\sigma[I])$ and $\Vrfy(1^\secp,s,\sigma[I+\secp])$.
\end{enumerate}
Clearly, $\cB$ simulates the challenger of $\Sigma^*$ conditioned on $1\la\mathsf{Check}(\Sigma)$.
Because we assume that $\Sigma$ satisfies the correctness, $1\la\mathsf{Check}(\Sigma)$ occurs with overwhelming probability.
Therefore, if $\cA$ breaks the security of $\Sigma^*$, then the number of $i\in[\secp]$ is at least $\frac{3\secp}{4}$ with non-negligible probability that satisfies $\top\la\Vrfy(1^\secp,s_i,\sigma[i])$ and $\top\la\Vrfy(1^\secp,s_i,\sigma[i+\secp])$.
Because $I$ is uniformly random and independent from $\cA$, $\top\la\Vrfy(1^\secp,s_I,\sigma[I])$ and $\top\la\Vrfy(1^\secp,s_I,\sigma[I+\secp])$ with non-negligible probability.
This completes the proof.
\end{proof}






\begin{proof}[Proof of \cref{thm:combiner_money}]
      First, let us introduce some notations.
\paragraph{Notations.}
\begin{itemize}
    \item Let $\Sigma_i$ be a candidate of mini-scheme for $i\in[n]$.
    \item For a candidate of mini-scheme $\Sigma_i$, let $\Sigma_i^*\seteq(\Mint_i^*,\Vrfy_i^*)$ be a candidate of mini-scheme derived from \cref{lem:amp_cor_money}, which satisfies:
    \begin{itemize}
        \item $\Sigma_i^*$ is uniform QPT algorithm if $\Sigma_i$ is uniform QPT algorithm.
        \item $\Sigma_i^*$ satisfies correctness.
        \item $\Sigma_i^*$ satisfies security if $\Sigma_i$ satisfies both correctness and security.
    \end{itemize}
\end{itemize}

      
    \paragraph{Construction of Robust Mini-Scheme Combiner:}
    We describe the robust mini-scheme combiner $\Sigma=(\Comb.\Mint,\Comb.\Vrfy)$:
\begin{description}
\item[$\Comb.\mathsf{Mint}(1^\secp,\{\Sigma_i\}_{i\in[n]})$:]$ $ 
    \begin{itemize}
        \item For all $i\in[n]$, run $(s_i^*,\rho_{s_i}^*)\la \Mint_i^*(1^\secp)$.
        \item Output $s\seteq \{s_i^*\}_{i\in[n]}$ and $\rho_s\seteq\bigotimes_{i\in[n]}\rho_{s_i}^*$.
    \end{itemize}
    \item[$\Comb.\Vrfy(1^\secp,s,\rho,\{\Sigma_i\}_{i\in[n]})$:]$ $
    \begin{itemize}
        \item Parse $s= \{s_i\}_{i\in[n]}$ Let $\rho$ be a quantum state on $n$ registers, $\{R[i]\}_{i\in[n]}$, each of which is of $\abs{\rho_{s_i}}$ qubits, and let $\rho[i]\seteq \Tr_{R[1]\cdots R[i-1]R[i+1]\cdots R[n]}(\rho)$.
        \item For all $i\in[n]$, run $\Vrfy_{i}^*(1^\secp,s_i,\rho[i])$.
        If $\top\la\Vrfy_i^*(1^\secp,s_i,\rho[i])$ for all $i\in[n]$, output $\top$. Otherwise, output $\bot$.
    \end{itemize}
\end{description}
\cref{thm:combiner_money} follows from the following \cref{lem:money_eff,lem:money_cor,lem:money_sec}.
\begin{lemma}\label{lem:money_eff}
    $\Sigma$ satisfies efficiency.
\end{lemma}
\begin{lemma}\label{lem:money_cor}
    $\Sigma$ satisfies correctness.
\end{lemma}
\begin{lemma}\label{lem:money_sec}
    $\Sigma$ satisfies security.
\end{lemma}
\cref{lem:money_eff} trivially follows.
\cref{lem:money_cor} follows because $\Sigma_i^*$ satisfies correctness for all $i\in[n]$.
\begin{proof}[Proof of \cref{lem:money_sec}]
We can prove \cref{lem:money_sec} via a standard hybrid argument.
For a reader's convenience, we describe the proof.
Let $\Sigma_x$ be a candidate of mini-scheme that satisfies both correctness and security.
Then, $\Sigma_x^*$ satisfies security from \cref{lem:amp_cor_money}.
Assume that there exists a QPT adversary $\cA$ that breaks the security of $\Sigma$, and then construct an adversary $\cB_x$ that breaks the security of $\Sigma_x^*$.
For some polynomial $t$, we describe the $\cB_x$:
\begin{enumerate}
    \item $\cB_x$ receives $\rho_{s_x}^*$ from the challenger of $\Sigma_x^*$.
    \item $\cB_x$ runs $(s_i^*,\rho_{s_i}^*)\la\Mint_i^*(1^\secp)$ for all $i\in[n]\backslash x$, and sends $\{\rho_{s_i}^*\}_{i\in[n]}$ to $\cA$.
    \item $\cB_x$ receives $\sigma$ from $\cA$. Here, $\sigma$ is a quantum state on $2n$ registers, $\{R[i]\}_{i\in[2n]}$, where $R[i]$ and $R[i+\secp]$ are a register acting on $\abs{\rho_{s_i}^*}$-length qubits.
    Let $\sigma[i]\seteq\Tr_{R[1]\cdots R[i-1]R[i+1]\cdots R[2n]}$ for $i\in[2n]$.
    \item $\cB_x$ sends $\sigma[x]\otimes \sigma[x+n]$ to the challenger of $\Sigma_x^*$.
    \item The challenger runs $\Vrfy_x^*(1^\secp,s_x^*,\sigma[x])$ and $\Vrfy(1^\secp,s_x^*,\sigma[x+n])$, and outputs $\top$ if both of them are $\top$.
\end{enumerate}
Clearly, $\cB_x$ perfectly simulates the challenge of $\Sigma$.
Because $\cA$ breaks the security of $\Sigma$, $\cA$ outputs $\sigma$ such that $\Vrfy_i^*(1^\secp,s_i^*,\sigma[i])$ and $\Vrfy_i^*(1^\secp,s_i^*,\sigma[i+n])$ for all $i\in[n]$ with non-negligible probability. 
Therefore, the challenger outputs $\top$ with non-negligible probability, which implies that $\cB_x$ breaks the security of $\Sigma_x^*$.
This completes the proof.
\end{proof}
\end{proof}


\subsection{Universal Construction}
\begin{definition}
    We say that a set of uniform algorithms $\Sigma_{\mathsf{Univ}}=(\Mint,\Vrfy)$ is a universal construction of mini-scheme when $\Sigma_{\mathsf{Univ}}$ is mini-scheme if there exists a mini-scheme.
\end{definition}

\begin{theorem}\label{thm:univ_money}
    There exists a universal construction of mini-scheme.
\end{theorem}
The proof is almost the same as \cref{thm:univ_owsg}, and thus we skip the proof.


\if0
Before proving \cref{thm:univ_money}, let us introduce the following \cref{prop:money_time}.
\begin{proposition}\label{prop:money_time}
If there exists public-key quantum money, then there exists public-key quantum money $\Sigma=(\keygen[x^*],\Mint[y^*],\Vrfy[z^*])$ such that each Turing machine $x^*$, $y^*$, and $z^*$ halt within $\secp^2$ steps for all sufficiently large security parameters $\secp\in\N$.  
\end{proposition}
This can be shown by a standard padding argument.
For the reader's convenience, we describe the proof in \cref{sec:padding}.


\begin{proof}[Proof of \cref{thm:univ_money}]
First, let us describe some notations:
\paragraph{Notations.}
\begin{itemize}
    \item For a set of classical Turing machines $\cM\seteq x||y||z\in \bit^*$, we write $\Sigma[\cM]\seteq(\keygen[x],\Mint[y],\Vrfy[x])$ to mean the candidate of public-key quantum money, where $\keygen$, $\Mint$, and $\Vrfy$ are described by a classical Turing machines $x$, $y$, and $z$ that generates a general quantum circuits, respectively.
    \item For a candidate of public-key quantum money $\Sigma[\cM]\seteq (\keygen[x],\Mint[y],\Vrfy[z])$, $\widetilde{\Sigma}[\cM]\seteq  (\widetilde{\keygen}[x],\widetilde{\Mint}[y],\widetilde{\Vrfy}[z])$ is a candidate of public-key quantum money such that if, for security parameter $\secp$, one of classical Turing machine $x$, $y$, and $z$ does not halt within $\secp^2$, then $\widetilde{\keygen}[x]$, $\widetilde{\Mint}[y]$, and $\widetilde{\Vrfy}[z]$ automatically outputs $\top$ so that $\widetilde{\Sigma}[\cM]$ satisfies efficiency.
    \item We write $\Comb.\Sigma\seteq \Comb.(\keygen,\Mint,\Vrfy)$ to mean a robust public-key quantum money combiner.
    \item For $n\in\N$, we write $\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(n)}}$ to mean $\{\widetilde{\Sigma}[x||y||z]\seteq (\widetilde{\keygen}[x],\widetilde{\Mint}[y],\widetilde{\Vrfy}[z])\}_{\{x\in\bit^{\leq\log(\secp)}, y\in\bit^{\leq\log(\secp)},z\in\bit^{\leq\log(\secp)} \}}$.
\end{itemize}
\paragraph{Construction.}
We give a description of $\Sigma_{\mathsf{Univ}}\seteq (\keygen_{\mathsf{Univ}},\Mint_{\mathsf{Univ}},\Vrfy_{\mathsf{Univ}})$
\begin{description}
    \item[$\keygen_{\mathsf{Univ}}(1^\secp)$:]$ $
    \begin{itemize}
        \item Output $k\la \Comb.\keygen(1^\secp, \{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(\secp)}} )$.
    \end{itemize}
    \item[$\Mint_{\mathsf{Univ}}(1^\secp,k)$:]$ $
    \begin{itemize}
        \item Run $\Comb.\Mint(1^\secp,k,\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq3\log(\secp)}})$, and output its output.
    \end{itemize}
    \item[$\Vrfy(1^\secp,k,\psi_k)$:]$ $
    \begin{itemize}
        \item Run $\Comb.\Vrfy(1^\secp,k,\psi_k,\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(\secp)}})$ and output its output.
    \end{itemize}
\end{description}

\cref{thm:univ_money} follows fromt the following \cref{lem:univ_money_eff,lem:univ_money_cor,lem:univ_money_sec}.
\begin{lemma}\label{lem:univ_money_eff}
    $\Sigma_{\mathsf{Univ}}$ satisfies efficiency.
\end{lemma}

\begin{lemma}\label{lem:univ_money_cor}
    $\Sigma_{\mathsf{Univ}}$ satisfies correctness.
\end{lemma}

\begin{lemma}\label{lem:univ_money_sec}
   If there exist public-key quantum money, then $\Sigma_{\mathsf{Univ}}$ satisfies security.
\end{lemma}

\cref{lem:univ_money_eff,lem:univ_money_cor} trivially follows because $\widetilde{\Sigma[x||y||z]}$ satisfies efficiency for all $x\in\bit^{\leq \log(\secp)}$, $y\in\bit^{\leq \log(\secp)}$, and $z\in\bit^{\leq \log(\secp)}$ and the robust public-key quantum money combiner $\Comb.\Sigma$ satisfies efficiency and correctness, and thus we skip the proofs of them.
\begin{proof}[Proof of \cref{lem:univ_money_sec}]
Assume that there exists public-key quantum money. Then, from \cref{prop:money_time}, there exists a public-key quantum money scheme $\Sigma[\cM^*]\seteq(\keygen[x^*],\Mint[y^*],\Vrfy[z^*])$, where each Turing machine $x^*\in\bit^*$, $y^*\in\bit^*$, and $z^*\in\bit^*$ halt within $\secp^2$ steps for all sufficiently large security parameters $\secp\in\N$.

For all sufficiently large $\secp\in\N$, $\{\cM\}_{\cM\in\bit^{\leq 3\log(\secp)}}$ contains $\cM^*$.
Therefore, $\Sigma_{\mathsf{Univ}}$ satisfies security
because one of $\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq3\log(\secp)}}$ satisfies correctness and security for all sufficiently large security parameters $\secp\in\N$ and $\Comb.\Sigma$ is a robust public-key quantum money combiner.
\end{proof}
\end{proof}
\fi































\if0
\section{Robust Public-Key Quantum Money Combiner}
\begin{definition}[Robust Public-Key Quantum Money Combiner]
    Let $\{\Sigma_{i}\}_{i\in[n]}$ be $n$-candidates of public-key quantum money promised that all $\{\Sigma_i\}_{i\in[n]}$ satisfy efficiency.
    A robust public-key money combiner $\Sigma$ consists of three algorithms $\Sigma\seteq(\keygen,\Mint,\Vrfy)$ defined as follows:
    \begin{description}
        \item[$\keygen(1^\secp,\{\Sigma_i\}_{i\in[n]})$:] It takes as input a security parameter $1^\secp$ and $\{\Sigma_i\}_{i\in[n]}$, and outputs a classical key pair $(\sk,\pk)$.
        \item[$\Mint(1^\secp,\sk,\{\Sigma_i\}_{i\in[n]})$:]
        It takes as input a security parameter $1^\secp$, $\sk$ and $\{\Sigma_i\}_{i\in[n]}$, and a quantum state $\psi_s$.
        \item[$\Vrfy(1^\secp,\pk,\psi,\{\Sigma_i\}_{i\in[n]})$:]
        It takes as input a security parameter $1^\secp$, $\pk$, $\psi$ and $\{\Sigma_i\}_{i\in[n]}$, and outputs $\top$ or $\bot$.
    \end{description}
    \paragraph{Efficiency.} $\Sigma\seteq (\keygen,\Mint,\Vrfy)$ are uniform QPT algorithms.
    \paragraph{Correctness.} 
    For all security parameters $\secp\in\N$,
    \begin{align}
        \Pr[\top\la\Vrfy(\pk,\psi_{\sk},\{\Sigma_i\}_{i\in[n]}):(\sk,\pk)\la\keygen(1^\secp,\{\Sigma_i\}_{i\in[n]}), \psi_\sk\la\Mint(\sk,\{\Sigma_i\}_{i\in[n]})]\geq 1-\negl(\secp).
    \end{align}
    \paragraph{Security.}
    If at least one of the public-key quantum money candidates $\{\Sigma_i\}_{i\in[n]}$ satisfies correctness and security, then $\Sigma$ satisfies 
    \begin{align}
        \Pr[\mathsf{Count}(1^\secp,\pk,\rho)\geq t+1:\psi_\sk\la\Mint(1^\secp,\sk),\rho\la\cA(\psi_\sk^{\otimes t})]\leq\negl(\secp)
    \end{align}
    for all non-uniform QPT adversaries $\cA$, all polynomials $t$, and all sufficiently large security parameters $\secp\in\N$.
    Here, $\rho$ is a quantum state on $\ell$ registers, $R_1,\cdots,R_{\ell}$ each of which is of $\abs{\psi_\sk}$ qubits, and $\mathsf{Count}$ is the following QPT algorithm: on input $\xi$, it runs $\top/\bot\la\ \Vrfy(1^\secp,\pk,\xi_j,\{\Sigma_i\}_{i\in[n]})$ for each $j\in[\ell]$, where $\xi_j$ is a quantum state of $\xi$ in the register $R_j$, and outputs the total number of $\top$.
\end{definition}






\begin{theorem}\label{thm:combiner_money}
    A robust public-key quantum money combiner exists.
\end{theorem}
For proving \cref{thm:combiner_money}, we introduce the following \cref{lem:amp_cor_money}.
\begin{lemma}\label{lem:amp_cor_money}
    Let $\Sigma=(\keygen,\mathsf{Mint},\Vrfy)$ be a candidate for public-key quantum money.
    There exists a public-key quantum money $\Sigma^*=(\keygen^*,\mathsf{Mint}^*,\Vrfy^*)$ such that
    \begin{enumerate}
        \item If $\Sigma$ is a uniform QPT algorithm, then $\Sigma^*$ is a uniform QPT algorithm.
        \item $\Sigma^*$ satisfies correctness.
        \item If $\Sigma$ satisfies both correctness and security, then $\Sigma^*$ satisfies security.
    \end{enumerate}
\end{lemma}
\begin{proof}[Proof of \cref{lem:amp_cor_money}]
Without loss of generality, $\Vrfy(1^\secp,\pk,\cdot)$ can be considered as the algorithm working in the following way:

For some input $\psi$, append auxiliary state $\ket{0\cdots0}\bra{0\cdots 0}$ to $\psi$, apply a unitary $U_{\Vrfy,\pk}$ on $\psi\otimes\ket{0\cdots 0}\bra{0\cdots 0} $, obtain $\rho_{\psi}$, and measure the first qubit of $\rho_{\psi}$ with the computational basis and output $\top$ if the measurement result is $1$ and $\bot$ otherwise.
Let $m$ be the length of $\psi\otimes\ket{0\cdots 0}\bra{0\cdots 0}$.


First, let us describe $\Sigma^*$.
\begin{description}
    \item[$\keygen^*(1^\secp)$:]$ $
    \begin{itemize}
        \item Run $(\sk,\pk)\la\keygen(1^\secp)$.
        \item Output $\sk^*\seteq(\sk,\pk)$ and $\pk^*\seteq \pk$.
    \end{itemize}
    \item[$\mathsf{Mint}^*(1^\secp,\sk^*)$:]$ $
    \begin{itemize}
        \item Run $\psi_{\sk}\la\mathsf{Mint}(\sk)$.
        \item Run $U_{\Vrfy,\pk}$ on $\psi_{\sk}\otimes \ket{0\cdots 0}\bra{0\cdots 0}$, obtain $\rho_{{\sk}}\seteq U_{\Vrfy,\pk}(\psi_{\sk}\otimes \ket{0\cdots 0}\bra{0\cdots 0}) U_{\Vrfy,\pk}^{\dagger} $, measures the first qubit of $\rho_{{\sk}}$, and obtains the measurement result $b$ and post-measurement quantum state $\rho_{b,\sk}$.
        \begin{itemize}
        \item If the measurement result is $1$, then output the $(m+1)$-length quantum state $\psi_{\sk}^*\seteq U_{\Vrfy,\pk}^{\dagger}(\ket{1}\bra{1}\otimes \rho_{1,\sk})U_{\Vrfy,\pk}\otimes \ket{1}\bra{1}$.
        \item 
        If the measurement result is $0$, then output the $(m+1)$-length quantum state $\psi_{\sk}^*\seteq \ket{0^{m+1}}\bra{0^{m+1}}$.
        \end{itemize}
    \end{itemize}
    \item[$\Vrfy^*(1^\secp,\pk^*,\psi)$:]$ $
    \begin{itemize}
        \item Measure the last qubit of $\psi$ with $\{\ket{0}\bra{0},\ket{1}\bra{1}\}$.
        \begin{itemize}
        \item If $\ket{0}\bra{0}$ is obtained, then the algorithm outputs $\top$.
        \item Otherwise, run $U_{\Vrfy,\pk}$ on the first $m$-qubit of $\psi$ and measures the first qubit in the computational basis, and outputs $\top$ if the measurement result is $1$ and $\bot$ otherwise.
        \end{itemize}
    \end{itemize}
\end{description}

\paragraph{Proof of the first item.} 
For appropriate quantum states $\rho_{0,\sk}$ and $\rho_{1,\sk}$, we can represent $\rho_{\sk}$ as follows:
\begin{align}
    \rho_{\sk} =p_0\ket{0}\bra{0}\otimes \rho_{0,s}+p_1\ket{1}\bra{1}\otimes \rho_{1,s}.
\end{align}
Let us consider the case where $0$ is obtained if we measure the first bit of $\rho_{\sk}$ in the computational basis.
In that case, $\psi_{\sk}^*=\ket{0^{m+1}}\bra{0^{m+1}}$, and thus $\Vrfy^*$ perfectly outputs $\top$.

On the other hand, if $1$ is obtained, then $\Mint^*$ outputs $\psi_{\sk}^*=U_{\Vrfy,\pk}^{\dagger}\left(\ket{1}\bra{1}\otimes \rho_{1,s}\right)U_{\Vrfy,\pk}\otimes \ket{1}\bra{1}$.
When $\Vrfy^*$ measures the last bit of $\psi_{\sk}^*$ with $\{\ket{0}\bra{0}, \ket{1}\bra{1}\}$, the measurement perfectly outputs $1$.
Since $\psi_{\sk}^*=U_{\Vrfy,\pk}^{\dagger}\left(\ket{1}\bra{1}\otimes \rho_{1,\sk}\right)U_{\Vrfy,\pk}\otimes \ket{1}\bra{1}$, we obtain $1$ as the measurement result when $\Vrfy^*$ runs $U_{\Vrfy,\pk}$ on the first $m$-qubit of $\psi_{\sk}^*$, and measures the first qubit in the computational basis.
Therefore, $\Vrfy^*$ perfectly outputs $\top$.
The discussion above implies that $\Sigma^*$ satisfies correctness.


\paragraph{Proof of the second item.}


We prove that $\Sigma^*$ satisfies security if $\Sigma$ satisfies correctness and security.
Because we assume that $\Sigma$ satisfies correctness,
we have
\begin{align}
    \rho_{\sk}=\negl(\secp)\ket{0}\bra{0}\otimes\rho_{0,\sk}+(1-\negl(\secp))\ket{1}\bra{1}\otimes \rho_{1,\sk}
\end{align}
for some appropriate quantum state $\rho_{0,\sk}$ and $\rho_{1,\sk}$.
From the gentle measurement lemma (\cref{lem:gentle}), we have
\begin{align}
\norm{\rho_{\sk}-\rho_{1,\sk}}_1\leq  \negl(\secp).
\end{align}
In particular, this implies that
\begin{align}
    \norm{\psi_{\sk}\otimes \ket{0}\bra{0}-\psi_{\sk}^*}\leq\negl(\secp).
\end{align}

Now, assume that $\cA$ breaks the security of $\Sigma^*$, and then construct $\cB$ that breaks the security of $\Sigma$.
\if0
Because $\cA$ breaks the security of $\Sigma^*$, for some polynomial $t$ and $p$, we have
\begin{align}
    \Pr[\mathsf{Count}^*(\pk^*,\rho)\geq t+1:(\sk^*,\pk^*)\la\keygen^*(1^{\secp}),\psi_{\sk}^*\la\Mint^*(\sk^*),\rho\la\cA(\pk^*,\psi_{\sk}^{*\otimes t})]\geq p(\secp),
\end{align}
where $\rho$ is a quantum state on $\ell$ registers, $R_1,\cdots,R_\ell$ each of which is of $\abs{\psi_{\sk}^*}$ qubits, and $\mathsf{Count}^*$ is the following QPT algorithm: on input $\xi$, it runs $\top\backslash\bot\la\Vrfy^*(\pk^*,\xi_j)$ for each $j\in[\ell]$, where $\xi_j$ is a quantum state of $\xi$ in the register $R_j$ and outputs the total number of $\top$.
\fi
Let us describe the $\cB$.
\begin{enumerate}
    \item $\cB$ receives $\pk$ from the challenger of $\Sigma$ and sends $\pk$ to $\cA$.
    \item $\cB$ receives $t$-copies of $\psi_{\sk}$ and sends $(\psi_{\sk}\otimes \ket{0}\bra{0})^{\otimes t}$ to $\cA$ if $\cA$ wants to receives $t$-copies of money states.
    \item $\cB$ receives $\rho $ and sends $\rho $ to the challenger of $\Sigma$.
    \item The challenger runs $\mathsf{Count}(1^\secp,\pk,\rho)$.
    If $\mathsf{Count}(1^\secp,\pk,\rho)$, then the experiment outputs $1$ indicating that $\cB$ wins, and outputs $0$ otherwise.
\end{enumerate}
Clearly, $\cB$ simulates the challenger of $\Sigma^*$ except that $\cB$ sends $\psi_{\sk}\otimes \ket{0}\bra{0}$ instead of $\psi_{\sk}^*$.
However, because $\norm{(\psi_{\sk}\otimes \ket{0}\bra{0})-\psi_{\sk}^*}\leq \negl(\secp)$, $\cB$ wins the security experiment above with non-negligible probability for some polynomial $t$ if $\cA$ breaks the security of $\Sigma^*$.
This completes the proof.


\end{proof}






\begin{proof}[Proof of \cref{thm:combiner_money}]
      First, let us introduce some notations.
\paragraph{Notations.}
\begin{itemize}
    \item Let $\Sigma_i$ be a candidate of public-key quantum money for $i\in[n]$.
    \item For a candidate of public-key quantum money $\Sigma_i$, let $\Sigma_i^*\seteq(\keygen_i^*,\Mint_i^*,\Vrfy_i^*)$ be a candidate of public-key money derived from \cref{lem:amp_cor_money}, which satisfies:
    \begin{itemize}
        \item $\Sigma_i^*$ satisfies correctness.
        \item $\Sigma_i^*$ satisfies security if $\Sigma_i$ satisfies both correctness and security.
    \end{itemize}
\end{itemize}

      
    \paragraph{Construction of Robust Public-Key Quantum Money Combiner:}
    We describe the robust public-key quantum money combiner $\Sigma=(\Comb.\keygen,\Comb.\Mint,\Comb.\Vrfy)$:
\begin{description}
\item[$\Comb.\keygen(1^\secp,\{\Sigma_i\}_{i\in[n]})$:]$ $
\begin{itemize}
    \item For all $i\in[n]$, run $(\sk_i^*,\pk_i^*)\la\keygen_i^*(1^{\secp})$.
    \item Output $\sk\seteq\{\sk_i^*\}_{i\in[n]}$ and $\pk\seteq\{\pk_i^*\}_{i\in[n]}$.
\end{itemize}
\item[$\Comb.\mathsf{Mint}(1^\secp,\sk,\{\Sigma_i\}_{i\in[n]})$:]$ $ 
    \begin{itemize}
        \item For all $i\in[n]$, run $\psi_{\sk_i}^*\la \Mint_i^*(1^\secp,\sk_i^*)$.
        \item Output $\psi_\sk\seteq\bigotimes_{i\in[n]}\psi_{\sk_i}^*$.
    \end{itemize}
    \item[$\Comb.\Vrfy(1^\secp,\pk,\psi,\{\Sigma_i\}_{i\in[n]})$:]$ $
    \begin{itemize}
        \item Let $\psi$ be a quantum state on $n$ registers, $R_1,\cdots,R_n$, each of which is of $\abs{\psi_{\sk_i}^*}$ qubits, and we write $\psi_{i}$ to mean a quantum state of $\psi$ in the register $R_i$.
        \item For all $i\in[n]$, run $\Vrfy_{i}^*(1^\secp,\pk_i^*,\psi_{i})$.
        If $\top\la\Vrfy_i^*(1^\secp,\pk_i^*,\psi_{i})$ for all $i\in[n]$, output $\top$. Otherwise, output $\bot$.
    \end{itemize}
\end{description}
\cref{thm:combiner_money} follows from the following \cref{lem:money_eff,lem:money_cor,lem:money_sec}.
\begin{lemma}\label{lem:money_eff}
    $\Sigma$ satisfies efficiency.
\end{lemma}
\begin{lemma}\label{lem:money_cor}
    $\Sigma$ satisfies correctness.
\end{lemma}
\begin{lemma}\label{lem:money_sec}
    $\Sigma$ satisfies security.
\end{lemma}
\cref{lem:money_eff} trivially follows.
\cref{lem:money_cor} follows because $\Sigma_i^*$ satisfies correctness for all $i\in[n]$.
\begin{proof}[Proof of \cref{lem:money_sec}]
We can prove \cref{lem:money_sec} via a standard hybrid argument.
For a reader's convenience, we describe the proof.
Let $\Sigma_x$ be a candidate of public-key quantum money that satisfies both correctness and security.
Then, $\Sigma_x^*$ satisfies security from \cref{lem:amp_cor_money}.
Assume that there exists a QPT adversary $\cA$ that breaks the security of $\Sigma$, and then construct an adversary $\cB_x$ that breaks the security of $\Sigma_x^*$.
For some polynomial $t$, we describe the $\cB_x$:
\begin{enumerate}
    \item $\cB_x$ receives $\pk_{x}^*$ from the challenger of $\Sigma_x^*$.
    \item $\cB_x$ runs $(\sk_i^*,\pk_{i}^*)\la\keygen_i^*(1^\secp)$ for all $i\in[n]\backslash x$, and sends $\{\pk_i^*\}_{i\in[n]}$ to $\cA$.
    \item  If $\cA$ wants to receive $t$-copies of money states, $\cB_x$ receives $t$-copies of $\psi_{\sk_x}^*$ from the challenger of $\Sigma_x^*$ and runs $\psi_{\sk_i}^*\la\Mint_i^*(\sk_i^*)$ $t$-times for all $i\in[n]$, and sends $\bigotimes_{i\in[n]}\psi_{\sk_i}^{*\otimes t}$ to $\cA$. 
    Let us denote $m[i]$ to mean the length of $\psi_{\sk_i}^*$.
    \item $\cB_x$ receives $\rho$ from $\cA$. Here, $\rho$ is a quantum state on $n\ell$ registers, $\{R_1[i]\}_{i\in[n]},\cdots,\{R_\ell[i]\}_{i\in[n]} $, where, for each $j\in[\ell]$ and $i\in[n]$, $R_j[i]$ is $m[i]$-length.
    We write $\rho_i[j]$ to mean a quantum state in the register $R_i[j]$, and write $\rho[j]$ to mean a quantum state in the registers $\{R_i[j]\}_{i\in[\ell]}$.
    \item $\cB_x$ sends the registers $\{R_j[x]\}_{j\in[\ell]}$ to the challenger of $\Sigma_x^*$.
    \item The challenger runs $\mathsf{Count}_x^*(1^\secp,\pk_x^*,\rho[x])$.
    The experiment outputs $1$ indicating $\cB_x$ wins if $\mathsf{Count}_x^*(1^\secp,\pk_x^*,\rho[x])\geq t+1$, and outputs $0$ otherwise.
    Here, for $j\in[n]$, $\mathsf{Count}_j^*$ works as follows:
    on input $\rho[j]$ consisting of $\ell$ registers, $R_1[j],\cdots,R_\ell[j]$, it runs $\Vrfy_j^*(1^\secp,\pk_j^*,\rho_i[j])$ for each $i\in[\ell]$ and outputs the total number of $\top$.
\end{enumerate}
Clearly, $\cB_x$ perfectly simulates the challenge of $\Sigma$.
Because $\cA$ breaks the security of $\Sigma$, $\cA$ outputs $\rho$ such that $\mathsf{Count}_i^*(1^\secp,\pk_i^*,\rho[i])\geq t+1$ for all $i\in[n]$ for some polynomial $t$ with non-negligible probability. 
Therefore, the experiment outputs $\top$ with non-negligible probability for some polynomial $t$, which implies that $\cB_x$ breaks the security of $\Sigma_x^*$.
This completes the proof.
\end{proof}
\end{proof}


\subsection{Universal Construction}
\taiga{In this Section, it might be good to explain the details}
\begin{definition}
    We say that a construction of public-key quantum money $\Sigma_{\mathsf{Univ}}=(\keygen,\Mint,\Vrfy)$ is a universal construction of public-key quantum money when $\Sigma_{\mathsf{Univ}}$ is public-key quantum money if there exists public-key quantum money.
\end{definition}

\begin{theorem}\label{thm:univ_money}
    There exists a universal construction of public-key quantum money.
\end{theorem}
The proof is almost the same as \cref{thm:univ_owsg}, and thus we skip the proof.


\if0
Before proving \cref{thm:univ_money}, let us introduce the following \cref{prop:money_time}.
\begin{proposition}\label{prop:money_time}
If there exists public-key quantum money, then there exists public-key quantum money $\Sigma=(\keygen[x^*],\Mint[y^*],\Vrfy[z^*])$ such that each Turing machine $x^*$, $y^*$, and $z^*$ halt within $\secp^2$ steps for all sufficiently large security parameters $\secp\in\N$.  
\end{proposition}
This can be shown by a standard padding argument.
For the reader's convenience, we describe the proof in \cref{sec:padding}.


\begin{proof}[Proof of \cref{thm:univ_money}]
First, let us describe some notations:
\paragraph{Notations.}
\begin{itemize}
    \item For a set of classical Turing machines $\cM\seteq x||y||z\in \bit^*$, we write $\Sigma[\cM]\seteq(\keygen[x],\Mint[y],\Vrfy[x])$ to mean the candidate of public-key quantum money, where $\keygen$, $\Mint$, and $\Vrfy$ are described by a classical Turing machines $x$, $y$, and $z$ that generates a general quantum circuits, respectively.
    \item For a candidate of public-key quantum money $\Sigma[\cM]\seteq (\keygen[x],\Mint[y],\Vrfy[z])$, $\widetilde{\Sigma}[\cM]\seteq  (\widetilde{\keygen}[x],\widetilde{\Mint}[y],\widetilde{\Vrfy}[z])$ is a candidate of public-key quantum money such that if, for security parameter $\secp$, one of classical Turing machine $x$, $y$, and $z$ does not halt within $\secp^2$, then $\widetilde{\keygen}[x]$, $\widetilde{\Mint}[y]$, and $\widetilde{\Vrfy}[z]$ automatically outputs $\top$ so that $\widetilde{\Sigma}[\cM]$ satisfies efficiency.
    \item We write $\Comb.\Sigma\seteq \Comb.(\keygen,\Mint,\Vrfy)$ to mean a robust public-key quantum money combiner.
    \item For $n\in\N$, we write $\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(n)}}$ to mean $\{\widetilde{\Sigma}[x||y||z]\seteq (\widetilde{\keygen}[x],\widetilde{\Mint}[y],\widetilde{\Vrfy}[z])\}_{\{x\in\bit^{\leq\log(\secp)}, y\in\bit^{\leq\log(\secp)},z\in\bit^{\leq\log(\secp)} \}}$.
\end{itemize}
\paragraph{Construction.}
We give a description of $\Sigma_{\mathsf{Univ}}\seteq (\keygen_{\mathsf{Univ}},\Mint_{\mathsf{Univ}},\Vrfy_{\mathsf{Univ}})$
\begin{description}
    \item[$\keygen_{\mathsf{Univ}}(1^\secp)$:]$ $
    \begin{itemize}
        \item Output $k\la \Comb.\keygen(1^\secp, \{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(\secp)}} )$.
    \end{itemize}
    \item[$\Mint_{\mathsf{Univ}}(1^\secp,k)$:]$ $
    \begin{itemize}
        \item Run $\Comb.\Mint(1^\secp,k,\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq3\log(\secp)}})$, and output its output.
    \end{itemize}
    \item[$\Vrfy(1^\secp,k,\psi_k)$:]$ $
    \begin{itemize}
        \item Run $\Comb.\Vrfy(1^\secp,k,\psi_k,\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(\secp)}})$ and output its output.
    \end{itemize}
\end{description}

\cref{thm:univ_money} follows fromt the following \cref{lem:univ_money_eff,lem:univ_money_cor,lem:univ_money_sec}.
\begin{lemma}\label{lem:univ_money_eff}
    $\Sigma_{\mathsf{Univ}}$ satisfies efficiency.
\end{lemma}

\begin{lemma}\label{lem:univ_money_cor}
    $\Sigma_{\mathsf{Univ}}$ satisfies correctness.
\end{lemma}

\begin{lemma}\label{lem:univ_money_sec}
   If there exist public-key quantum money, then $\Sigma_{\mathsf{Univ}}$ satisfies security.
\end{lemma}

\cref{lem:univ_money_eff,lem:univ_money_cor} trivially follows because $\widetilde{\Sigma[x||y||z]}$ satisfies efficiency for all $x\in\bit^{\leq \log(\secp)}$, $y\in\bit^{\leq \log(\secp)}$, and $z\in\bit^{\leq \log(\secp)}$ and the robust public-key quantum money combiner $\Comb.\Sigma$ satisfies efficiency and correctness, and thus we skip the proofs of them.
\begin{proof}[Proof of \cref{lem:univ_money_sec}]
Assume that there exists public-key quantum money. Then, from \cref{prop:money_time}, there exists a public-key quantum money scheme $\Sigma[\cM^*]\seteq(\keygen[x^*],\Mint[y^*],\Vrfy[z^*])$, where each Turing machine $x^*\in\bit^*$, $y^*\in\bit^*$, and $z^*\in\bit^*$ halt within $\secp^2$ steps for all sufficiently large security parameters $\secp\in\N$.

For all sufficiently large $\secp\in\N$, $\{\cM\}_{\cM\in\bit^{\leq 3\log(\secp)}}$ contains $\cM^*$.
Therefore, $\Sigma_{\mathsf{Univ}}$ satisfies security
because one of $\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq3\log(\secp)}}$ satisfies correctness and security for all sufficiently large security parameters $\secp\in\N$ and $\Comb.\Sigma$ is a robust public-key quantum money combiner.
\end{proof}
\end{proof}
\fi
\color{black}
\fi
\fi


\section{Proof of \cref{lem:amp_cor_money}}
To show \cref{lem:amp_cor_money}, we use the following \cref{lem:hoefd}.
\begin{lemma}[Hoeffding's inequality]\label{lem:hoefd}
    Let $X_i\in\bit$ be a two-outcome independent random variable,
    and let $S_n\seteq\sum_{i\in[n]} X_i$.
    Then, we have
    \begin{align}
        \Pr[\abs{S_n-\Exp[S_n]}\geq t]\leq 2\exp(-2t^2/n).
    \end{align}
\end{lemma}
\begin{proof}[Proof of \cref{lem:amp_cor_money}]
Let us describe $\Sigma^*$.
\begin{description}
    \item[$\Mint^*(1^\secp)$:]$ $
    \begin{itemize}
        \item Run $\mathsf{Check}(\Sigma)$, where $\mathsf{Check}$ works as follows:
        \begin{itemize}
        \item Run $(s_i,\rho_{s_i})\la\Mint(1^\secp)$ for all $i\in[\secp]$.
        \item Run $\Vrfy(1^\secp,s_i,\rho_{s_i})$ for all $i\in[\secp]$.
        \item Output $1$ if the number of $\top\la\Vrfy(1^\secp,s_i,\rho_{s_i})$ is at least $\frac{11\secp}{12}$, and output $0$ otherwise.
        \end{itemize}
        \item If $1\la\mathsf{Check}(\Sigma)$, then run $(s_i,\rho_{s_i})\la\Mint(1^\secp)$ for all $i\in[\secp]$ and output $s^*\seteq \{s_i\}_{i\in[\secp]} $ and $\rho_{s}^*\seteq \bigotimes_{i\in[\secp]}\rho_{s_i}$. 
        \item If $0\la\mathsf{Check}(\Sigma)$, then run $(s_i,\rho_{s_i})\la\Mint(1^\secp)$ for all $i\in[\secp]$ and output $s\seteq \top$ and $\rho_{s^*}\seteq \bigotimes_{i\in[\secp]}\rho_{s_i}$.
    \end{itemize}
    \item[$\Vrfy^*(1^\secp, s^*,\rho)$:]$ $ 
    \begin{itemize}
        \item Let $\rho$ be a quantum state on the $\secp$ registers $R[1]\cdots R[\secp]$. Let $\rho[i]\seteq \Tr_{R[1]\cdots R[i-1]R[i+1]\cdots R[\secp]}(\rho)$ for all $i\in[\secp]$.
        \item If $s^*= \top$, output $\top$.
        \item If $s^* \neq \top$, then parse $s^*= \{s_i\}_{i\in[\secp]}$ and run $\Vrfy(1^\secp,s_i,\rho[i])$ for all $i\in[\secp]$.
        Output $\top$ if the number of $\top\la\Vrfy(1^\secp,s_i,\rho[i])$ is at least $\frac{3\secp}{4}$.
    \end{itemize}
\end{description}
We have the following \cref{prop:money_eff_2,prop:money_cor_2,prop:money_sec_2}.
\begin{proposition}\label{prop:money_eff_2}
    If $\Sigma$ satisfies efficiency, then $\Sigma^*$ satisfies efficiency.
\end{proposition}

\begin{proposition}\label{prop:money_cor_2}
    If $\Sigma$ satisfies correctness, then $\Sigma^*$ satisfies correctness.
\end{proposition}

\begin{proposition}\label{prop:money_sec_2}
    If $\Sigma$ satisfies efficiency, correctness, and security, then $\Sigma^*$ satisfies security.
\end{proposition}
We skip the proof of \cref{prop:money_eff_2}.


\begin{proof}[Proof of \cref{prop:money_cor_2}]
First, assume that $\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]<5/6$, and compute $\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]$.
\begin{align}
    &\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\\
    &\geq\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 0\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\Pr[0\la\mathsf{Check}(\Sigma)]\\
    &\geq \Pr[0\la\mathsf{Check}(\Sigma)]\\
    &\geq 1-2\exp(-\secp/72)).
\end{align}
Here in the third inequality, we have used that 
$\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]<5/6$ and \cref{lem:hoefd}, which we will show later.

Next, assume that $\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]\geq 5/6$, and compute $\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]$.
\begin{align}
    &\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\\
    &\geq\bigg(\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 0\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\Pr[0\la\mathsf{Check}(\Sigma)]\\
    &+\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\Pr[1\la\mathsf{Check}(\Sigma)]\bigg)\\
    &= \Pr[0\la\mathsf{Check}(\Sigma)]+\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\Pr[1\la\mathsf{Check}(\Sigma)]\\
    &=1-\Pr[1\la\mathsf{Check}(\Sigma)]\left(1-\Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\right)\\
    &\geq \Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}): 1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\\
    &\geq 1-2\exp(-\secp/72)).
\end{align}
Here in the final inequality, we have used that $ \Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]\geq 5/6$ and \cref{lem:hoefd}, which we will prove later.
Therefore, the $\Sigma^*$ satisfies the correctness.

We will prove the skipped part.
Assume $\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]<5/6$ and show $\Pr[0\la\mathsf{Check}(\Sigma)]\geq 1-2\exp(-\secp/72)$.
We consider the random variable $X_{i}$ as $1$ if $\top\la\Vrfy(1^\secp,s_i,\rho_{s_i})$ for the $i$-th running of the verification algorithm while running $\mathsf{Check}$, and consider $X_i$ as $0$ if $\bot\la\Vrfy(1^\secp,s_i,\rho_{s_i})$. 
If we denote $S_{\secp}\seteq\sum_{i\in[\secp]}X_{i}$, then
$1\la\mathsf{Check}(\Sigma) $ if and only if $S_{\secp}\geq \frac{11\secp}{12}$.
On the other hand,
because $\Exp[S_{\secp}]<\frac{5\secp}{6}$, $\abs{S_{\secp}-\Exp[S_{\secp}]}\geq \frac{\secp}{12}$ must hold for $S_{\secp}\geq \frac{11\secp}{12}$.
Therefore, from \cref{lem:hoefd}, we have
\begin{align}
    \Pr[1\la\mathsf{Check}(\Sigma)]\leq \Pr[\abs{S_{\secp}-\Exp[S_{\secp}]}\geq \frac{\secp}{12}]\leq2\exp(-\frac{\secp}{72}).
\end{align}
In the same way, we can prove that 
\begin{align}
    \Pr[\top\la\Vrfy^*(1^\secp,s^*,\rho_{s^*}):1\la\mathsf{Check}(\Sigma)\wedge (s^*,\rho_{s^*})\la\Mint^*(1^\secp)]\geq 1-2\exp(-\secp/72)
\end{align}
when $\Pr[\top\la\Vrfy(1^\secp,s,\rho_s):(s,\rho_s)\la\Mint(1^\secp)]\geq 5/6$.
\end{proof}



\begin{proof}[Proof of \cref{prop:money_sec_2}]
Let us introduce the following sequence of hybrids as follows.

\begin{description}
    \item[$\mathsf{Hyb_0}$:] This is the original security experiment of $\Sigma^*$.
    \begin{enumerate}
        \item The challenger first runs $\mathsf{Check}(\Sigma)$.
        \begin{itemize}
            \item If $1\la\mathsf{Check}(\Sigma)$, then run $(s_i,\rho_{s_i})\la\Mint (1^\secp)$ for all $i\in[\secp]$ and send $(\{s_i\}_{i\in[\secp]},\bigotimes_{i\in[\secp]}\rho_{s_i})$ to $\cA$.
            \item If $0\la\mathsf{Check}(\Sigma)$, then run $(s_i,\rho_{s_i})\la\Mint (1^\secp)$ for all $i\in[\secp]$ and send $(\bot,\bigotimes_{i\in[\secp]}\rho_{s_i})$ to $\cA$.
        \end{itemize}
        \item $\cA$ sends $\sigma$ consisting of $2\secp$ registers $\{R[1]\cdots R[2\secp]\}$. Let $\sigma[i]\seteq\Tr_{R[1]\cdots R[i-1]R[i+1]\cdots R[2\secp]}(\sigma)$.
        \item The challenger does the following.
        \begin{itemize}
            \item If $1\la\mathsf{Check}(\Sigma)$, then run $\Vrfy(s_i,\sigma[i])$ for all $i\in[\secp]$ and set $A=1$ if the number of $\top$ is at least $3\secp/4$, and set $A=0$ otherwise. 
            Run
            $\Vrfy(s_i,\sigma[\secp+i])$ for all $i\in[\secp]$ and set $B=1$ if the number of $\top$ is at least $3\secp/4$, and set $B=0$ otherwise. 
            If $A=B=1$, then the challenge outputs $\top$, and outputs $\bot$ otherwise.
            \item If $0\la\mathsf{Check}(\Sigma)$, then the challenger always outputs $\top$.
        \end{itemize}
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:] This is the same as $\mathsf{Hyb_0}$ except that the challenger always behaves the same way as the case of $1\la\mathsf{Check}(\Sigma)$.
\end{description}
Because $\Sigma$ satisfies correctness, $1\la\mathsf{Check}(\Sigma)$ occurs with overwhelming probability, and thus we have
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\leq \negl(\secp).
\end{align}

Furthermore, we can show that 
\begin{align}
    \Pr[\mathsf{Hyb_1}=1]\leq \negl(\secp)
\end{align}
as long as $\Sigma$ satisfies security as follows.
For contradiction assume that there exists a QPT adversary $\cA$ such that 
\begin{align}
    \Pr[\mathsf{Hyb_1}=1]
\end{align}
is non-negligible, and then construct a QPT adversary $\cB$ that breaks $\Sigma$ as follows.
\begin{enumerate}
    \item $\cB$ receives $(s,\rho_s)$ from the challenger of $\Sigma$.
    \item $\cB$ samples $I\in[\secp]$, and sets $s_I=s$ and $\rho_{s_I}\seteq \rho_s$.
    \item $\cB$ generates $(s_j,\rho_{s_j})\la\Mint(1^\secp)$ for all $j\in[\secp]\backslash I$, and sends $\left(\{s_j\}_{j\in[\secp]},\bigotimes_{j\in[\secp]}\rho_{s_j}\right)$ to $\cA$.
    \item $\cB$ receives $\sigma$ consisting of $2\secp$ registers $R[1],\cdots,R[2\secp]$. We write $\sigma[j]\seteq \Tr_{R[1]\cdots R[j-1]R[j+1]\cdots R[2\secp]}(\sigma)$ for all $j\in[\secp]$.
    \item $\cB$ runs $\Vrfy(1^\secp,s_i,\sigma[i])$ and $\Vrfy(1^\secp,s_i,\sigma[i+\secp])$ for all $i\in[\secp]\backslash I$.
    \item $\cB$ sends $\sigma[I]\otimes \sigma[I+\secp]$ to the challenger, and it computes $\Vrfy(1^\secp,s,\sigma[I])$ and $\Vrfy(1^\secp,s,\sigma[I+\secp])$.
\end{enumerate}
Clearly, $\cB$ simulates the challenger of $\mathsf{Hyb_1}$.
We write $\mathsf{First}$ to mean the event such that the number of $\top\la\Vrfy(s_i,\sigma[i])$ within $i\in[\secp]$ is at least $3\secp/4$.
Similarly, we write $\mathsf{Second}$ to mean the event such that the number of $\top\la\Vrfy(s_i,\sigma[i+\secp])$ within $i\in[\secp]$ is at least $3\secp/4$.
Because $\Pr[\mathsf{Hyb_1}=1]$ is non-negligible, both $\mathsf{First}$ and $\mathsf{Second}$ occurs at the same time with non-negligible probability. 
This implies that, with non-negligible probability, $\cA$ outputs $\sigma$ such that the number of $i\in[\secp]$ satisfying both $\top\la\Vrfy(s_i,\sigma[i])$ and $\top\la\Vrfy(s_i,\sigma[i+\secp])$ is at least $\secp/2$.
Because $I$ is uniformly random and independent from $\cA$, 
 $\top\la\Vrfy(1^\secp,s_I,\sigma[I])$ and $\top\la\Vrfy(1^\secp,s_I,\sigma[I+\secp])$ occurs at the same time with non-negligible probability.
 This is a contradiction that $\Sigma$ satisfies security. Therefore, we have $\Pr[\mathsf{Hyb_1}]\leq \negl(\secp)$.
\end{proof}

\end{proof}






==> Old_OWSG.tex <==
% !TEX root = main.tex
\section{Robust OWSGs Combiner}
\begin{definition}[Robust OWSGs Combiner]
Let $\{\Sigma_i\seteq(\keygen_i,\StateGen_i,\Vrfy_i)\}_{i\in[n]}$ be $n$-candidates of OWSGs promised that all candidates $\{\Sigma_i\}_{i\in[n]}$ satisfy efficiency.
A robust OWSG combiner $\Sigma$ consists of three algorithms $(\keygen,\StateGen,\Vrfy)$ defined as follows:
\begin{itemize}
    \item[$\keygen(1^\secp,\{\Sigma_i\}_{i\in[n]})$:]$ $
    It takes as input a security parameter $\secp$ and $\{\Sigma_i\}_{i\in[n]}$ and outputs a classical key $k$.
    \item[$\StateGen(1^\secp,k,\{\Sigma_i\}_{i\in[n]})$:]$ $
    It takes as input a security parameter $1^\secp$, $k$ and $\{\Sigma_i\}_{i\in[n]}$, and outputs a quantum state $\psi_k$.
    \item[$\Vrfy(1^\secp,k,\psi_k,\{\Sigma_i\}_{i\in[n]})$:]$ $
    It takes as input a security parameter $1^\secp$, $k$, $\psi_k$, and $\{\Sigma_i\}_{i\in[n]}$, and outputs $\top$ or $\bot$.
\end{itemize}
We require the following three properties:
\paragraph{Efficiency.}
The algorithms $(\keygen,\StateGen,\Vrfy)$ are uniform QPT algorithms.

\paragraph{Correctness.}
For all security parameters $\secp\in\N$,
\begin{align}
    \Pr[\top\la\Vrfy(1^\secp,k,\psi_k,\{\Sigma_i\}_{i\in[n]}):k\la\keygen(1^\secp,\{\Sigma_i\}_{i\in[n]}),\psi_k\la\StateGen(1^\secp,k,\{\Sigma_i\}_{i\in[n]})]\geq 1-\negl(\secp).
\end{align}

\paragraph{Security}
If at least one of the OWSG candidates $\{\Sigma_i\}_{i\in[n]}$ satisfies correctness and security, then for all sufficiently large security parameters $\secp\in\N$, $\Sigma$ also satisfies 
\begin{align}
\Pr[\top\la\Vrfy(1^\secp,k^*,\psi_k):k\la\keygen(1^\secp),\psi_k\la\StateGen(1^\secp,k),k^*\la\cA(\psi_k^{\otimes t(\secp)})]\leq \negl(\secp)
\end{align}
for all non-uniform QPT adversaries $\cA$ and all polynomials $t$.
\end{definition}



\begin{theorem}\label{thm:OWSG_combiner}
   A robust OWSG combiner exists.
\end{theorem}

For proving \cref{thm:OWSG_combiner}, we introduce the following \cref{lem:amp_OWSG_cor}.
\begin{lemma}\label{lem:amp_OWSG_cor}
    Let $\Sigma=(\keygen,\StateGen,\Vrfy)$ be a candidate of OWSGs. There exists a OWSGs $\Sigma^*$ such that
    \begin{enumerate}
        \item If $\Sigma$ is uniform QPT algorithm, $\Sigma^*$ is uniform QPT algorithm.
        \item $\Sigma^*$ satisfies perfect correctness.
        \item If $\Sigma$ satisfies correctness and security, then $\Sigma^*$ satisfies security.
    \end{enumerate}
\end{lemma}
\begin{proof}[Proof of \cref{lem:amp_OWSG_cor}]
    Without loss of generality, $\Vrfy(1^\secp,k,\psi)$ can be considered as the algorithm working in the following way:

For input $(1^\secp,k,\psi)$, run a classical Turing machine $\cM$ on $(1^\secp,k,\abs{\psi})$, obtain $U_{\Vrfy,k}$, append auxiliary state $\ket{0\cdots0}\bra{0\cdots 0}$ to $\psi$, apply a unitary $U_{\Vrfy,k}$ on $\psi\otimes\ket{0\cdots 0}\bra{0\cdots 0} $, obtain $\rho_{\psi}$, and measure the first qubit of $\rho_{\psi}$ with the computational basis and output $\top$ if the measurement result is $1$ and $\bot$ otherwise.


We describe the $\Sigma^*\seteq(\keygen^*,\StateGen^*,\Vrfy^*)$.
\begin{description}
    \item[$\keygen^*(1^\secp):$]$ $
    \begin{itemize}
        \item Run $k\la\keygen(1^\secp)$.
        \item Output $k^*\seteq k$.
    \end{itemize}
    \item[$\StateGen(1^\secp,k^*)$:]$ $
    \begin{itemize}
        \item Parse $k^*=k$. 
        \item Run $ \psi_k\la \StateGen(1^\secp,k)$.
        \item Run $U_{\Vrfy,k}$ on $\psi_k\otimes\ket{0\cdots 0}\bra{0\cdots 0}$, obtain $\rho_k\seteq U_{\Vrfy,k}\left(\psi_{k} \otimes \ket{0\cdots 0}\bra{0\cdots 0}\right)U_{\Vrfy,k}^{\dagger}$, measures the first bit of $\rho_k$ in the computational basis, and obtains the measurement result $b$ and post-measurement quantum state $\rho_{b,k}$.
        \begin{itemize}
            \item If the measurement result is $1$, then output $\psi_k^*\seteq U_{\Vrfy,k}^{\dagger}(\ket{1}\bra{1}\otimes \rho_{1,k})U_{\Vrfy,k}\otimes \ket{1}\bra{1}$.
            \item If $0$ is obtained, then output $\psi_k^*\seteq U_{\Vrfy,k}^{\dagger}(\ket{0}\bra{0}\otimes \rho_{0,k})U_{\Vrfy,k}\otimes \ket{0}\bra{0}$.
        \end{itemize}
    \end{itemize}
    \item[$\Vrfy^*(1^\secp,k^*,\psi^*)$:]$ $
    \begin{itemize}
        \item Parse $k^*=k$ and $\psi^*\seteq \rho\otimes \ket{b}\bra{b}$.
        \item Measure the last bit of $\psi^*$ in the computational basis.
        \begin{itemize}
            \item If $1$ is obtained, then measure the first bit of $U_{\Vrfy,k}\rho U_{\Vrfy,k}^{\dagger} $ in the computational basis, and output $\top$ if the measurement outcome is $1$ and $\bot$ otherwise.
            \item If $0$ is obtained, then outputs $\top$.
        \end{itemize}
    \end{itemize}
\end{description}
The first item and the second item straightforwardly follow.

\paragraph{Proof of the third item.}
Assume that $\cA$ breaks the security of $\Sigma^*$, and then construct $\cB$ that breaks the security of $\Sigma$.
\if0
Let us describe the sequence of hybrids
\begin{description}
    \item[$\mathsf{Hyb_0}$:] This is the original security experiment of $\Sigma^*$. 
    \item[$\mathsf{Hyb_1}$:] This is $\mathsf{Hyb_0}$ except that it halts if the $0$ is obtained as the measurement result while running $\StateGen^*(1^\secp,k)$. 
    \item[$\mathsf{Hyb_2}$:] This is $\mathsf{Hyb_1}$ except that the challenger sends $\psi_k\otimes \ket{0\cdots 0}\bra{0\cdots 0}\otimes \ket{1}\bra{1}$ instead of $\psi_k^*$.
\end{description}
\fi
\begin{enumerate}
    \item $\cB$ receives $\psi_k^{\otimes (t+1)}$ from the challenger of $\Sigma$.
    \item $\cB$ sends $\left(\psi_k\otimes \ket{0\cdots 0}\bra{0\cdots 0}\otimes \ket{1}\bra{1}\right)^{\otimes t}$ to $\cA$.
    \item $\cB$ receives $k^*$ from $\cA$.
    \item $\cB$ runs $\Vrfy^*\left(1^\secp,k^*,(\psi_k\otimes \ket{0\cdots 0}\bra{0\cdots 0}\otimes \ket{1}\bra{1})\right)$, and if the result is $\top$, sends $k^*$ to the challenger of $\Sigma$.
\end{enumerate}
From the construction of $\cB$, $\cB$ simulates the security experiment of $\Sigma^*$ except that it uses $\psi_k\otimes \ket{0\cdots 0}\bra{0\cdots 0}\otimes \ket{1}\bra{1}$ instead of $\psi_{k}^*$.
Because we assume that $\Sigma$ satisfies correctness,
\begin{align}
    U_{\Vrfy,k}(\psi_k\otimes \ket{0\cdots 0}\bra{0\cdots 0}) U_{\Vrfy,k}^{\dagger} =\negl(\secp)\ket{0}\bra{0}\otimes\rho_{0,k}+(1-\negl(\secp))\ket{1}\bra{1}\otimes \rho_{1,k}
\end{align}
where $k\la\keygen(1^\secp)$, $\psi_k\la\StateGen(1^\secp,k)$, and $\rho_{0,\sk}$ and $\rho_{1,\sk}$ are some appropriate quantum state.

From the gentle measurement lemma (\cref{lem:gentle}), we have
\begin{align}
\norm{U_{\Vrfy,k}(\psi_k\otimes \ket{0\cdots 0}\bra{0\cdots 0}) U_{\Vrfy,k}^{\dagger}-\ket{1}\bra{1}\otimes\rho_{1,k}}_1\leq  \negl(\secp).
\end{align}
In particular, this implies that
\begin{align}
    \norm{\psi_{k}\otimes \ket{0\cdots 0}\bra{0\cdots 0}\otimes \ket{1}\bra{1}-\psi_{k}^*}\leq\negl(\secp).
\end{align}

If $\cA$ breaks the security of $\Sigma^*$, then $\top\la\Vrfy^*\left(1^\secp,k^*,(\psi_k\otimes \ket{0\cdots 0}\bra{0\cdots 0}\otimes \ket{1}\bra{1})\right)$ with non-negligible probability 
because 
\begin{align}
    \norm{\psi_{k}\otimes \ket{0\cdots 0}\bra{0\cdots 0}\otimes \ket{1}\bra{1}-\psi_{k}^*}\leq\negl(\secp).
\end{align}
This implies that the challenger of $\Sigma$ outputs $\top$ with non-negligible probability, which is a contradiction.

\end{proof}


\begin{proof}[Proof of \cref{thm:OWSG_combiner}]
First, let us introduce some notations.

\paragraph{Notations:}
\begin{itemize}
    \item Let $\{\Sigma_i\seteq(\keygen_i,\StateGen_i,\Vrfy_i)\}$ be a candidate of OWSGs for $i\in[n]$.
    \item For a candidate of OWSGs $\Sigma_i$, let $\Sigma_i^*\seteq(\keygen_i^*,\StateGen_i^*,\Vrfy_i^*)$ be a candidate of OWSGs derived from \cref{lem:amp_OWSG_cor}. that satisfies:
    \begin{itemize}
        \item If $\Sigma_i$ satisfies efficiency, then $\Sigma_i^*$ satisfies efficiency.
        \item $\Sigma_i^*$ satisfies correctness.
        \item If $\Sigma_i$ satisfies both correctness and security, then $\Sigma_i^*$ satisfies security.
    \end{itemize}
\end{itemize}

\paragraph{Construction of Robust OWSG Combiner:}
We describe $\Sigma=(\Comb.\keygen,\Comb.\StateGen,\Comb.\Vrfy)$:
\begin{description}
    \item[$\Comb.\keygen(1^\secp,\{\Sigma_i\}_{i\in[n]})$:]$ $ 
    \begin{itemize}
        \item For all $i\in[n]$, run $k_i^*\la\keygen_i^*(1^\secp)$.
        \item Output $k\seteq\{k_i^*\}_{i\in[n]}$.
    \end{itemize}
    \item[$\Comb.\StateGen(1^\secp,k,\{\Sigma_i\}_{i\in[n]})$:]$ $
    \begin{itemize}
        \item Parse $k=k_1^*||\cdots ||k_n^*$.
        \item For all $i\in[n]$, run $\psi_{k_i^*}\la\StateGen_i^*(k_i^*)$
        \item Output $\psi_{k}\seteq \bigotimes_{i\in[n]}\psi_{k_i^*}$.
    \end{itemize}
    \item[$\Comb.\Vrfy(1^\secp,k,\psi_k,\{\Sigma_i\}_{i\in[n]})$:]$ $
    \begin{itemize}
        \item Parse $k=k_1||\cdots ||k_n$ and $\psi_k=\bigotimes_{i\in[n]}\psi_{k_i}$.
        \item For all $i\in[n]$, run $\Vrfy_i^*(k_i,\psi_{k_i})$.
        If $\top\la\Vrfy_i^*(k_i^*,\psi_{k_i^*})$ for all $i\in[n]$, output $\top$. Otherwise, output $\bot$.
    \end{itemize}
\end{description}
\cref{thm:OWSG_combiner} follows from the following \cref{lem:OWSG_eff,lem:OWSG_cor,lem:OWSG_sec}, which we prove later

\begin{lemma}\label{lem:OWSG_eff}
$\Sigma$ satisfies efficiency.
\end{lemma}

\begin{lemma}\label{lem:OWSG_cor}
    $\Sigma$ satisfies correctness.
\end{lemma}

\begin{lemma}\label{lem:OWSG_sec}
    $\Sigma$ satisfies security.
\end{lemma}
\cref{lem:OWSG_eff} trivially follows. \cref{lem:OWSG_cor} follows because $\Sigma_i^*$ satisfies correctness for all $i\in[n]$.
The proof of \cref{lem:OWSG_sec} is similar to \cref{lem:money_sec}, and thus we skip the proof.
\end{proof}



\subsection{Universal Construction}
\begin{definition}
    We say that a set of uniform QPT algorithms $\Sigma_{\mathsf{Univ}}=(\keygen,\StateGen,\Vrfy)$ is a universal construction of OWSGs when $\Sigma_{\mathsf{Univ}}$ is OWSGs if there exists a OWSGs.
\end{definition}

\begin{theorem}\label{thm:univ_owsg}
    There exists a universal construction of OWSGs.
\end{theorem}
Before proving \cref{thm:univ_owsg}, let us introduce the following \cref{prop:owsg_time}.
\begin{proposition}\label{prop:owsg_time}
If there exists OWSGs, then there exists OWSGs $\Sigma=(\keygen[x^*],\StateGen[y^*],\Vrfy[z^*])$ such that each classical polyonomial Turing machine $x^*$, $y^*$, and $z^*$ halt within $\secp^2$ steps for all sufficiently large security parameters $\secp\in\N$.  
\end{proposition}
This can be shown by a standard padding argument.
For the reader's convenience, we describe the proof in \cref{sec:padding}.


\begin{proof}[Proof of \cref{thm:univ_owsg}]
First, let us describe some notations:
\paragraph{Notations.}
\begin{itemize}
    \item For a set of classical Turing machines $\cM\seteq x||y||z\in \bit^*$, we write $\Sigma[\cM]\seteq(\keygen[x],\StateGen[y],\Vrfy[x])$ to mean the candidate of OWSGs, where uniform QPT algorithms $\keygen$, $\StateGen$, and $\Vrfy$ are described by a classical Turing machine $x$, $y$, and $z$ that generates a general quantum circuit, respectively.
    \item For a candidate of OWSGs $\Sigma[\cM]\seteq (\keygen[x],\StateGen[y],\Vrfy[z])$, $\widetilde{\Sigma}[\cM]\seteq  (\widetilde{\keygen}[x],\widetilde{\StateGen}[y],\widetilde{\Vrfy}[z])$ is a candidate of OWSGs such that $\widetilde{\keygen}[x]$, $\widetilde{\StateGen}[y]$, and $\widetilde{\Vrfy}[z]$ automatically outputs $\top$ so that $\widetilde{\Sigma}[\cM]$ satisfies efficiency if one of classical Turing machine $x$, $y$, and $z$ does not halt within $\secp^2$ for all security parameters $\secp\in\N$.
    \item We write $\Comb.\Sigma\seteq \Comb.(\keygen,\StateGen,\Vrfy)$ to mean a robust OWSGs combiner.
    \item For $n\in\N$, we write $\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(n)}}$ to mean\\ $\{\widetilde{\Sigma}[x||y||z]\seteq (\widetilde{\keygen}[x],\widetilde{\StateGen}[y],\widetilde{\Vrfy}[z])\}_{\{x\in\bit^{\leq\log(\secp)}, y\in\bit^{\leq\log(\secp)},z\in\bit^{\leq\log(\secp)} \}}$.
\end{itemize}
\paragraph{Construction.}
We give a description of $\Sigma_{\mathsf{Univ}}\seteq (\keygen_{\mathsf{Univ}},\StateGen_{\mathsf{Univ}},\Vrfy_{\mathsf{Univ}})$.
\begin{description}
    \item[$\keygen_{\mathsf{Univ}}(1^\secp)$:]$ $
    \begin{itemize}
        \item Output $k\la \Comb.\keygen(1^\secp, \{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(\secp)}} )$.
    \end{itemize}
    \item[$\StateGen_{\mathsf{Univ}}(1^\secp,k)$:]$ $
    \begin{itemize}
        \item Run $\Comb.\StateGen(1^\secp,k,\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq3\log(\secp)}})$, and output its output.
    \end{itemize}
    \item[$\Vrfy(1^\secp,k,\psi_k)$:]$ $
    \begin{itemize}
        \item Run $\Comb.\Vrfy(1^\secp,k,\psi_k,\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq 3\log(\secp)}})$ and output its output.
    \end{itemize}
\end{description}

\cref{thm:univ_owsg} follows fromt the following \cref{lem:univ_owsg_eff,lem:univ_owsg_cor,lem:univ_owsg_sec}.
\begin{lemma}\label{lem:univ_owsg_eff}
    $\Sigma_{\mathsf{Univ}}$ satisfies efficiency.
\end{lemma}

\begin{lemma}\label{lem:univ_owsg_cor}
    $\Sigma_{\mathsf{Univ}}$ satisfies correctness.
\end{lemma}

\begin{lemma}\label{lem:univ_owsg_sec}
   If there exist OWSGs, then $\Sigma_{\mathsf{Univ}}$ satisfies security.
\end{lemma}

\cref{lem:univ_owsg_eff,lem:univ_owsg_cor} straightforwardly follows because $\widetilde{\Sigma}[x||y||z]$ satisfies efficiency for all $x\in\bit^{\leq \log(\secp)}$, $y\in\bit^{\leq \log(\secp)}$, and $z\in\bit^{\leq \log(\secp)}$ and the robust OWSG combiner $\Comb.\Sigma$ satisfies efficiency and correctness, and thus we skip the proofs of them.
\begin{proof}[Proof of \cref{lem:univ_owsg_sec}]
Assume that there exists OWSG. Then, from \cref{prop:owsg_time}, there exists a OWSG scheme $\Sigma[\cM^*]\seteq(\keygen[x^*],\StateGen[y^*],\Vrfy[z^*])$, where each Turing machine $x^*\in\bit^*$, $y^*\in\bit^*$, and $z^*\in\bit^*$ halt within $\secp^2$ steps for all sufficiently large security parameters $\secp\in\N$.

For all sufficiently large $\secp\in\N$, $\{\cM\}_{\cM\in\bit^{\leq 3\log(\secp)}}$ contains $\cM^*$.
Therefore, $\Sigma_{\mathsf{Univ}}$ satisfies security
because one of $\{\widetilde{\Sigma}[\cM]\}_{\cM\in\bit^{\leq3\log(\secp)}}$ satisfies correctness and security for all sufficiently large security parameters $\secp\in\N$ and $\Comb.\Sigma$ is a robust OWSGs combiner.

\end{proof}


\end{proof}



\if0
\begin{proof}[Proof of \cref{lem:OWSG_cor}]
For $i\in[n]$, we write $\fail_i$ to mean the event that $\mathsf{Check}(\Sigma_i)$ outputs $\top$ although the correctness of $\Sigma_i$ is below $2/3$. 
We compute $\Pr[\mathsf{fail_i}]$ when the correctness of $\Sigma_i$ is at most $2/3$.
We consider the random variable $X_{i,j}$ as $1$ if $\top\la\Vrfy_i(k,\phi_k)$ for the $j$-th running of the verification algorithm while running $\mathsf{Check}$, and consider $X_j$ as $0$ if $\bot\la\Vrfy_i(k,\phi_k)$. 
If we denote $S_{i,\secp}\seteq\sum_{j\in[\secp]}X_{i,j}$, then $\Exp[S_{i,\secp}]\leq\frac{2\secp}{3}$, and thus $\abs{S_{i,\secp}-\Exp[S_{i,\secp}]}\geq \frac{\secp}{6}$ must hold for $S_{i,\secp}\geq \frac{5\secp}{6}$.
Therefore, from \cref{lem:hoefd}, we have
\begin{align}
    \Pr[\fail_i]\leq \Pr[\abs{S_{i,\secp}-\Exp[S_{i,\secp}]}\geq \frac{\secp}{6}]\leq2\exp(-\frac{\secp}{18}).
\end{align}
In particular,
because $\fail_i$ is an independent event, we have
\begin{align}
    \Pr[\bigcap_{i\in[n]}\overline{\fail_i}]
    &=\prod_{i\in[\secp]}\Pr[\bigcap_{i\in[n]}\overline{\fail_i}]\\
    &= \left(1-2\exp(-\secp/18)\right)^n\\
    &\geq 1-2n\exp(-\secp/18).
\end{align}

We compute the probability $\Pr_{k_i,\psi_{k_i}}[\top\la\mathsf{Mult}.\Vrfy_i(k_i,\psi_{k_i})]$ promised that $\Sigma_i$ satisfies $\frac{2}{3}$-correctness.
Here, $k_i\seteq \{k_i^j\}_{j\in[\secp]}$ and $\psi_{k_i}\seteq\bigotimes_{j\in[\secp]}\psi_{k_i^j}$, where $k_i^j\la\keygen_i(1^{\secp})$ and $\psi_{k_i^j}\la\StateGen_i(k_i^j)$ for $j\in[\secp]$.
We consider $X_{i,j}$ as $1$ if $\top\la\Vrfy_i(k_i^j,\psi_{k_i^j})$, and consider $X_{i,j}$ as $0$ otherwise.
If we denote $S_{i,\secp}\seteq \sum_{j\in[\secp]}X_{i,j}$, then $\Exp[S_{i,\secp}]\geq \frac{2\secp}{3}$, and thus $\abs{S_{i,\secp}-\Exp[S_{i,\secp}]}\geq \frac{\secp}{6}$ must hold when $S_{i,\secp}\leq \frac{\secp}{2}$.
Then, by \cref{lem:hoefd}, we have
\begin{align}
    \Pr_{k_i,\psi_{k_i}}[\top\la\mathsf{Mult}.\Vrfy_i(k_i,\psi_{k_i})]
    &=1-\Pr_{k_i,\psi_{k_i}}[\bot\la\mathsf{Mult}.\Vrfy(k_i,\psi_{k_i})]\\
    &\geq 1-\Pr[\abs{S_{i,\secp}-\Exp[S_{i,\secp}]}\geq\frac{\secp}{6} ]\geq 1-2\exp(-\frac{\secp}{18}).
\end{align}
In particular, because $\top\la\mathsf{Mult}.\Vrfy_i(k_i,\psi_{k_i})$ is an independent event, if $\Sigma_i$ satisfies $2/3$-correctness for all $i\in[n]$, then we have
\begin{align}    \Pr_{k,\psi_{k}}[\bigcap_{i\in[n]}\left(\top\la\mathsf{Mult}.\Vrfy_i(k_i,\psi_{k_i})\right)]=\prod_{i\in[n]}\Pr_{k_i,\psi_{k_i}}[\top\la\mathsf{Mult}.\Vrfy_i(k_i,\psi_{k_i})]\geq (1-2\exp(-\secp/18))^n\geq 1-2n\exp(-\secp/18).
\end{align}



Finally, we compute $\Pr_{\substack{k\la\Comb.\keygen(1^\secp)\\ \psi_k\la\Comb.\StateGen(k)}}[\top\la\Vrfy(k,\psi_k)]$.
\begin{align}
    &\Pr_{\substack{k\la\Comb.\keygen(1^\secp)\\ \psi_k\la\Comb.\StateGen(k)}}[\top\la\Vrfy(k,\psi_k)]\\
    &\geq\Pr_{\substack{k\la\Comb.\keygen(1^\secp)\\ \psi_k\la\Comb.\StateGen(k)}}[\top\la\Comb.\Vrfy(k,\psi_k)\wedge \bigcap_{i\in[n]}\overline{\fail_i}]\\
    &\geq \Pr_{\substack{k\la\Comb.\keygen(1^\secp)\\ \psi_k\la\Comb.\StateGen(k)}}[\top\la\Comb.\Vrfy(k,\psi_k): \bigcap_{i\in[n]}\overline{\fail_i}]\Pr[\bigcap_{i\in[n]}\overline{\fail_i}]\\
    &\geq (1-2n\exp(-\secp/18))^2\geq 1-4n\exp(-\secp/18).
\end{align}
Here in the third inequality, we have used that $\Sigma_i$ satisfies $\frac{2}{3}$-correctness or $\mathsf{Mult}.\Vrfy_i(k_i,\psi_{k_i})$ always outputs $\top$ when $\fail_i$ does not occur.

\end{proof}


\begin{proof}[Proof of \cref{lem:OWSG_sec}]
    For simplicity, we omit $\{\Sigma_i\}_{i\in[n]}$ from $\Comb.\keygen(1^\secp,\{\Sigma_i\}_{i\in[n]})$, $\Comb.\StateGen(k,\{\Sigma_i\}_{i\in[n]})$, and $\Comb.\Vrfy(k,\psi_k,\{\Sigma_i\}_{i\in[n]})$, and for some event $X$ we write $\Pr_{k,\psi_k,k^*}[X]$ to mean $\Pr_{\substack{k\la\Comb.\keygen(1^{\secp})\\\psi_k\la\Comb.\StateGen(k)\\k^*\la\cA(\psi^{\otimes t})}}[X]$.
    
    Let us assume that $\Sigma_{x}$ satisfies both correctness and security.
    We note that there exists a negligible $\negl$ such that $\Pr[\bot\la\mathsf{Check}(\Sigma_x)]\leq \negl(\secp)$ because $\Sigma_x$ satisfies correctness.
    For contradiction, let us assume that $\cA $ breaks the security of $\Sigma$, and then construct a QPT algorithm $\cB$ that breaks the security of $\Sigma_x$.
    We have
    \begin{align}
      &\Pr_{k,\psi_k,k^*}[\top\la\Comb.\Vrfy(k^*,\psi_k)]  \\
      &=\Pr_{k,\psi_k,k^*}[\top\la\Comb.\Vrfy(k^*,\psi_k)\wedge\bot\la\mathsf{Check}(\Sigma_x)]
    +\Pr_{k,\psi_k,k^*}[\top\la\Comb.\Vrfy(k^*,\psi_k)\wedge\top\la\mathsf{Check}(\Sigma_x)]\\
      &\leq\Pr_{k,\psi_k,k^*}[\bot\la\mathsf{Check}(\Sigma_x)]+\Pr_{k,\psi_k,k^*}[\top\la\mathsf{Mult}.\Vrfy_x(k^*_x,\psi_{k_x})\wedge\top\la\mathsf{Check}(\Sigma_x)]\\
      &\leq\negl(\secp)+\Pr_{k,\psi_k,k^*}[\top\la\mathsf{Mult}.\Vrfy_x(k^*_x,\psi_{k_x})\wedge\top\la\mathsf{Check}(\Sigma_x)].
    \end{align}
    Here in the first inequality, we have used the fact that the output of $\mathsf{Mult}.\Vrfy$ is $\top$ when the output of $\Comb.\Vrfy$ is $\top$, and in the second inequality, we have used $\Pr[\bot\la\mathsf{Check}(\Sigma_x)]\leq \negl(\secp)$.
     Because we assume that $\cA$ breaks the security of $\Comb.\Sigma$, $\Pr_{k,\psi_k,k^*}[\top\la\Comb.\Vrfy(k^*,\psi_k)]$ is non-negligible, and thus
    \begin{align}
    \Pr_{k,\psi_k,k^*}[\top\la\mathsf{Mult}.\Vrfy_x(k^*_x,\psi_{k_x})\wedge\top\la\mathsf{Check}(\Sigma_x)]\geq p(\sep)
    \end{align}
    for some non-negligible $p$.
    Furthermore, the \cref{prop:comb_owsg} holds, which we prove later.
    \color{red}
    \begin{proposition}\label{prop:comb_owsg}
    \begin{align}
        \Pr_{k,\psi_k,k^*}[\top\la\mathsf{Mult}.\Vrfy_x(k^*_x,\psi_{k_x})\wedge\top\la\mathsf{Check}(\Sigma_x)]\leq \frac{1}{n}\sum_{y\in[n]}\Pr_{k,\psi_k,k^*}[\top\la\Vrfy_x(k_x^{*y},\psi_{k_x^y})\wedge\top\la\mathsf{Check}(\Sigma_x)].
    \end{align}
    \end{proposition}
    \color{black}
    \taiga{I skip the red part, and I think that I need to modify the inequality above.}
    
    Now, let us describe the $\cB$.
    \begin{enumerate}
        \item $\cB$ runs $b_i\la\mathsf{Check}(\Sigma_i)$ for all $i\in[n]$.
        If $\bot\la\mathsf{Check}(\Sigma_x)$, then $\cB$ aborts the protocol.
        \item $\cB$ does the followings for all $i\in[n]\backslash x$:
        \begin{itemize}
            \item If $b_i=\top$, run $k_{i}^j\la\keygen(1^{\secp})$ for all $j\in[\secp]$ and set $k_i\seteq\{k_i^j\}_{j\in[\secp]}$.
            \item Otherwise, set $k_{i}\seteq \bot$.
        \end{itemize}
        \item For all $i\in[n]\backslash x$:
        \begin{itemize}
            \item If $k_i\seteq\bot$, then set $\psi_{k_i}\seteq\bot$.
            \item Otherwise, set $\psi_{k_i}\seteq\bigotimes_{i\in[n]}\psi_{k_i^j}$ where $\psi_{k_i^j}\la\StateGen_i(k_i^j)$. 
        \end{itemize}
        \item The challenger samples $k'_x\la\keygen_x(1^\secp)$, and sends $\psi_{k'_x}^{\otimes t}$ to $\cB$.
        \item $\cB$ samples $y\la[\secp]$, and sets $\psi_{k_x}\seteq\bigotimes_{j\in[\secp]}\psi_{k_x^j}$, where $\psi_{k_x^j}\la\keygen_x(k_x^j)$ for $j\in[\secp]\backslash y$ and $\psi_{k_x^y}\seteq \psi_{k'_x}$.
        \item $\cB$ sends $\left(\psi_{k_1}\otimes\cdots\otimes \psi_{k_n}\right)^{\otimes t}$ to $\cA$.
        \item $\cB$ receives $k^*\seteq \{k_1^{*j}\}_{j\in[\secp]}||\cdots ||\{k_n^{*j}\}_{j\in[\secp]}$ from the $\cA$.
        \item $\cB$ sends $k_x^{*y}$ to the challenger.
    \end{enumerate}
    Now, we compute the probability that $\cB$ breaks the security of $\Sigma_x$.
    Note that when $\top\la\Sigma_x$, $\cB$ perfectly simulates the challenger of $\Comb.\Sigma$.
    \begin{align}
        &\Pr[\cB\mbox{ \,\,wins}]\\
        &=\Pr_{k,\psi_{k},y,k^*}[\top\la\Vrfy_x(k_x^{*y},\psi_{k'_x})\wedge \top\la\mathsf{Check}(\Sigma_x)]\\
        &=\frac{1}{n}\sum_{y\in[n]}\Pr_{k,\psi_{k},k^*}[\top\la\Vrfy_x(k_x^{*y},\psi_{k'_x})\wedge \top\la\mathsf{Check}(\Sigma_{x})]
    \end{align}
    From \cref{prop:comb_owsg}, $\Pr[\cB\mbox{\,\, wins}]$ is non-negligible, which contradicts to $\Sigma_x$ satisfies security.
    Now, we show the remaining \cref{prop:comb_owsg}.
    \begin{proof}[Proof of \cref{prop:comb_owsg}]
        
    \end{proof}
\end{proof}
\fi

==> Old_Unclone.tex <==
% !TEX root = main.tex
\section{Robust Combiner for Unclonable Encryption}\label{sec:unc}
\begin{definition}[Robust Combiner for Unclonable Secret-Key Encryption]
    A robust combiner for (one-time) unclonable secret-key encryption with $\ell(\secp)$-bit plaintexts is a deterministic classical polynomial-time Turing machine $\cM$ with the following properties:
    \begin{itemize}
        \item $\cM$ takes as input $1^n$ with $n\in\N$ and $n$-candidates (one-time) unclonable secret-key encryption with $\ell(\secp)$-bit plaintexts $\{\Sigma_i\seteq(\keygen_i,\Enc_i,\Dec_i)\}_{i\in[n]}$ promised that all candidates satisfies efficiency, and outputs a set of algorithms $\Sigma\seteq(\keygen,\Enc,\Dec)$.
        \item If all of $\{\Sigma_i\}_{i\in[n]}$ satisfies efficiency and at least one of $\{\Sigma_i\}_{i\in[n]}$ satisfies correctness, (one-time) IND-CPA security and (one-time) unclonable IND-CPA security, then $\Sigma$ is (one-time) unclonable secret-key encryption for $\ell(\secp)$-bit plaintexts that satisfies efficiency, correctness, (one-time) IND-CPA security and (one-time) unclonable IND-CPA security.
    \end{itemize}
\end{definition}


\if0
\begin{definition}[Robust Unclonable Secret-Key Encryption Combiner]
A $(1,n)$-robust unclonable secret-key encryption for $\ell(\secp)$-bit plaintexts combiner $\Comb.\Sigma$ consists of three algorithms $(\Comb.\keygen,\Comb.\Enc,\Comb.\Dec)$, where $n$ and $\ell$ are some polynomial.
For $i\in\N$, let $\Sigma_i$ be a candidate of unclonable secret-key encryption for $\ell(\secp)$-bit plaintexts promised that $\Sigma_i$ satisfies efficiency. 
A $(1,n)$-robust unclonable secret-key encryption for $\ell(\secp)$-bit plaintexts combiner $(\Comb.\keygen,\Comb.\Enc,\Comb.\Dec)$ has the following syntax:
    \begin{description}
        \item[$\Comb.\keygen(1^{\secp},\{\Sigma_i\}_{i\in[n(\secp)]})$:]
        It takes as input a security parameter $1^\secp$, and $n(\secp)$-candidates of unclonable secret-key encryption $\{\Sigma_i\}_{i\in[n(\secp)]}$, and outputs a classical key $\sk$.
        \item[$\Comb.\Enc(1^\secp,\sk,m, \{\Sigma_i\}_{i\in[n(\secp)]})$:]
        It takes as input a security parameter $1^\secp$, $\sk$, $m\in\bit^{\ell(\secp)}$ and $\{\Sigma\}_{i\in[n(\secp)]}$ and outputs a quantum ciphertext $\ct$.
        \item[$\Comb.\Dec(1^\secp,\sk,\ct,\{\Sigma_i\}_{i\in[n]})$:]
        It takes as input a security parameter $1^\secp$, $\sk$, $\ct$ and $\{\Sigma_i\}_{i\in[n(\secp)]}$ and outputs $m$.
    \end{description}
    \paragraph{Efficiency.} $(\Comb.\keygen,\Comb.\Enc,\Comb.\Dec)$ are uniform QPT algorithms.
    \paragraph{Correctness.}
    For all security parameters $\secp\in\N$ and $m\in\bit^{\ell(\secp)}$,
    \begin{align}
        \Pr\left[m\la\Comb.\Dec(1^\secp,\sk,\ct,\{\Sigma_i\}_{i\in[n(\secp)]})
        \ \middle |
        \begin{array}{ll}
              \sk\la\Comb.\keygen(1^{\secp},\{\Sigma_i\}_{i\in[n(\secp)]}) \\
              \ct\la\Comb.\Enc(1^\secp,\sk,m,\{\Sigma_i\}_{i\in[n(\secp)]})
        \end{array}
        \right]
        \geq 1-\negl(\secp).
    \end{align}
    \paragraph{IND-CPA security.}
    If $\Sigma_i$ satisfies both correctness and IND-CPA security for some $i\in[n(\secp)]$, then $\Comb.\Sigma$ satisfies the IND-CPA security defined below.
    Given a $(1,n)$-robust unclonable encryption combiner $\Comb.\Sigma$, we consider the following security experiment $\mathsf{Exp}_{\Comb.\Sigma,\cA}^{\mathsf{IND\mbox{-}CPA}}(1^\secp,\{\Sigma_i\}_{i\in[n(\secp)]})$ against $\cA$.
    \begin{enumerate}
        \item The challenger runs $\sk\la\Comb.\keygen(1^\secp,\{\Sigma_i\}_{i\in[n(\secp)]})$.
        \item $\cA$ can query $\Comb.\Enc(1^\secp,\sk,\{\Sigma_i\}_{i\in[n(\secp)]}, \cdot)$ polynomially many times.
        \item $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger samples $b\la\bit$, runs $\ct_b\la\Comb.\Enc(1^\secp,\sk,\{\Sigma_i\}_{i\in[n(\secp)]}, m_b)$, and sends $\ct_b$ to $\cA$.
        \item $\cA$ outputs $b'$.
        \item The experiment outputs $1$ indicating win if $b=b'$ and $0$ otherwise.
    \end{enumerate}
    We say that $\Comb.\Sigma$ is unclonable IND-CPA secure if for all non-uniform QPT adversaries $\cA$, 
    \begin{align}
        \Pr[\mathsf{Exp}_{\Comb.\Sigma,\cA}^{\mathsf{IND\mbox{-}CPA}}(1^\secp,\{\Sigma_i\}_{i\in[n(\secp)]})=1]\leq \frac{1}{2}+\negl(\secp).
    \end{align}
    
    \paragraph{Unclonable IND-CPA Security.}
    If $\Sigma_i$ satisfies both correctness and unclonable IND-CPA security for some $i\in[n(\secp)]$, then $\Comb.\Sigma$ satisfies the unclonable IND-CPA security defined below.
    Given a $(1,n)$-robust unclonable encryption combiner $\Comb.\Sigma$, we consider the following security experiment $\mathsf{Exp}_{\Comb.\Sigma,(\cA,\cB,\cC)}^{\mathsf{unclone}}(1^\secp,\{\Sigma_i\}_{i\in[n(\secp)]})$ against $(\cA,\cB,\cC)$.
    \begin{enumerate}
        \item The challenger runs $\sk\la\Comb.\keygen(1^\secp,\{\Sigma_i\}_{i\in[n(\secp)]})$.
        \item $\cA$ can query $\Comb.\Enc(1^\secp,\sk,\{\Sigma_i\}_{i\in[n(\secp)]}, \cdot)$ polynomially many times.
        \item $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger samples $b\la\bit$, runs $\ct_b\la\Comb.\Enc(1^\secp,\sk,\{\Sigma_i\}_{i\in[n(\secp)]}, m_b)$, and sends $\ct_b$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\sk$ and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ indicating win if $b_\cB=b_\cC=b$ and $0$ otherwise.
    \end{enumerate}
We say that $\Comb.\Sigma$ is unclonable IND-CPA secure if for all non-uniform QPT adversaries $(\cA,\cB,\cC)$,
\begin{align}
    \Pr[\mathsf{Exp}_{\Comb.\Sigma,(\cA,\cB,\cC)}^{\mathsf{unclone}}(\secp,\{\Sigma_i\}_{i\in[n(\secp)]})=1]\leq \frac{1}{2}+\negl(\secp).
\end{align}
\end{definition}
\begin{remark}
    In this work, we also consider a robust one-time unclonable secret-key encryption.
    The difference is that the inputs of the algorithms $\Sigma\seteq (\keygen,\StateGen,\Vrfy)$ are candidates of one-time unclonable secret-key encryption instead of unclonable secret-key encryption, and if one of the candidates is correct and secure one-time secret-key encryption, then $\Sigma$ satisfies one-time IND-CPA security and one-time unclonable IND-CPA security.
\end{remark}
\fi


In this section, we prove the following \cref{thm:unclone_ske_comb}.
\begin{theorem}\label{thm:unclone_ske_comb}
   There exists a robust combiner for (one-time) unclonable secret-key encryption with $\ell(\secp)$-bit plaintexts for all polynomial $\ell$. 
\end{theorem}

As a corollary, we obtain the following \cref{cor:unclone_pke}.
\begin{corollary}\label{cor:unclone_pke}
    There exists a robust combiner for unclonable public-key encryption with $\ell(\secp)$-bit plaintexts for all polynomial $\ell$.
\end{corollary}
\begin{proof}[Proof of \cref{cor:unclone_pke}]
We give a rough sketch of the proof.

\cref{cor:unclone_pke} follows from the following observations. 
We can trivially obtain one-time unclonable SKE from unclonable PKE.
From \cref{thm:unclone_ske_comb}, we have a robust combiner for one-time unclonable SKE. 
Furthermore, we can trivially construct PKE with quantum ciphertext from unclonable PKE. It is known that there exists a robust PKE combiner~\cite{EC:HKNRR05}, and we observe that we can also construct a robust combiner for PKE with quantum ciphertext in the same way.
Moreover, we can construct unclonable PKE from one-time unclonable SKE, and PKE with quantum ciphertext.
This is because we can construct unclonable PKE from one-time SKE and receiver non-committing encryption with quantum ciphertext 
~\footnote{
\cite{TCC:AK21} shows that unclonable PKE can be constructed from one-time unclonable SKE and PKE with classical ciphertext.
Note that it is unclear whether we can construct unclonable PKE from one-time SKE and PKE with ``quantum'' ciphertext in the same way as \cite{TCC:AK21}.
This is because they use the existence of OWFs in their proof although it is unclear whether PKE with quantum ciphertext implies OWFs.
Therefore, we use the technique of \cite{Asia:HMNY21} instead.
(For the detail, see \cref{sec:app_unc_pke})
} (For the detail, see \cref{sec:app_unc_pke}),
and
receiver non-committing encryption with quantum ciphertext can be constructed from PKE with quantum ciphertext in the same way as the classical ciphertext case~\cite{TCC:CanHalKat05,C:KNTY19}.

By combining these observations, we can construct a robust combiner for unclonable PKE as follows.
Given candidates of unclonable PKE $\{\Sigma_i\}_{i\in[n]}$, we first use a robust combiner for one-time unclonable SKE, and obtain a new candidate of one-time unclonable SKE $\Sigma_{\SKE}$.
Next, we use a robust combiner for PKE with quantum ciphertext and obtain a new candidate of PKE with quantum ciphertext $\Sigma_{\PKE}$.
Then, we construct a receiver non-committing encryption with quantum ciphertext $\Sigma_{\NCE}$ from $\Sigma_{\PKE}$.
Finally, we construct unclonable PKE $\Sigma_{\unc}$ from one-time unclonable SKE $\Sigma_{\SKE}$ and receiver non-committing encryption with quantum ciphertext $\Sigma_{\NCE}$.
\end{proof}

For proving \cref{thm:unclone_ske_comb}, we introduce the following \cref{lem:unclone_ske_cor}.


    


\begin{lemma}\label{lem:unclone_ske_cor}
    Let $\Sigma$ be a candidate for (one-time) unclonable secret-key encryption with $\ell(\secp)$-bit plaintexts.
    From $\Sigma$, we can construct a (one-time) unclonable secret-key encryption with $\ell(\secp)$-bit plaintexts  $\Sigma^*\seteq(\keygen^*,\Enc^*,\Dec^*)$ such that:
    \begin{enumerate}
        \item $\Sigma^*$ is a uniform QPT algorithm, if $\Sigma$ is a uniform QPT algorithm.
        \item $\Sigma^*$ satisfies perfect correctness.
        \item $\Sigma^*$ satisfies (one-time) IND-CPA security and (one-time) unclonable IND-CPA security if $\Sigma$ is a uniform QPT algorithm and satisfies correctness, (one-time) IND-CPA security and (one-time) unclonable IND-CPA security.
    \end{enumerate}
\end{lemma}
The proof is almost the same as \cref{lem:amp_OWSG_cor}.
For the reader's convenience, we describe the construction of $\Sigma^*$ in \cref{sec:app_unclone_comb}.


\begin{proof}[Proof of \cref{thm:unclone_ske_comb}]
    Below, we consider a fixed constant $n$ and a fixed polynomial $\ell$.
    Let us describe some notations:
    \paragraph{Notations.}
    \begin{itemize}
        \item Let $\Sigma_i$ be a candidate of (one-time) unclonable secret-key encryption with $\ell(\secp)$-length for $i\in[n]$.
        \item For a candidate of (one-time) unclonable secret-key encryption with $\ell(\secp)$-bit plaintexts $\Sigma_i$, let $\Sigma_i^*\seteq(\keygen^*_i,\Enc^*_i,\Dec^*_i)$ be a candidate of (one-time) unclonable secret-key encryption with $\ell(\secp)$-bit plaintexts derived from \cref{lem:unclone_ske_cor}, which satisfies:
        \begin{itemize}
            \item $\Sigma_i^*$ is a uniform QPT algorithm, if $\Sigma_i$ is a uniform QPT algorithm.
            \item $\Sigma_i^*$ satisfies correctness.
            \item $\Sigma_i^*$ satisfies (one-time) IND-CPA security and
            (one-time) unclonable IND-CPA security if $\Sigma_i$ is uniform QPT algorithm and satisfies correctness, (one-time) IND-CPA security, and
            (one-time) unclonable IND-CPA security.
        \end{itemize}
    \end{itemize} 
    \paragraph{Construction of Robust (One-Time) Unclonable Secret-Key Encryption.}
    A robust combiner for (one-time) unclonable secret-key encryption with $\ell(\secp)$-bit plaintexts is a deterministic classical polynomial-time Turing machine that takes as input $1^n$ and $\{\Sigma_i\}_{i\in[n]}$, and outputs the following set of algorithms  
    $\Sigma=(\keygen,\Enc,\Dec)$:
    \begin{description}
        \item[$\keygen(1^\secp)$:]$ $
        \begin{itemize}
            \item For all $i\in[n]$, run $\sk_i^*\la \keygen_i^*(1^{\secp})$.
            \item Output $\sk\seteq \{\sk_i^*\}_{i\in[n]}$.
        \end{itemize}
        \item[$\Enc(1^\secp,\sk,m)$:]$ $
        \begin{itemize}
        \item For all $i\in[n]$, sample $r_i\la\bit^{\ell(\secp)}$ promised that $\sum_{i\in[n]}r_i=m$, where the $\ell(\secp)$ is the length of plaintext $m$.
        \item For all $i\in[n]$, run $\ct_i^*\la\Enc_i^*(1^\secp,\sk_i^*,r_i)$ for all $i\in[n]$.
        \item Output $\ct\seteq \{\ct_i^*\}_{i\in[n]}$.
        \end{itemize}
        \item[$\Dec(1^\secp,\sk,\ct) $:]$ $
        \begin{itemize}
            \item Run $r_i^*\la\Dec_i^*(1^\secp,\sk_i^*,\ct_i^*)$ for all $i\in[n]$.
            \item Output $\sum_{i\in[n]}r_i^*$.
        \end{itemize}
    \end{description}
    
    \cref{thm:unclone_ske_comb} follows from the following \cref{lem:eff_unc_comb,lem:cor_unc_comb,lem:ind_sec_unc_comb,lem:sec_unc_comb}.
    \begin{lemma}\label{lem:eff_unc_comb}
        If all of $\{\Sigma_i\}_{i\in[n]}$ satisfies efficiency, $\Sigma$ satisfies efficiency.
    \end{lemma}
    \begin{lemma}\label{lem:cor_unc_comb}
        $\Sigma$ satisfies correctness.
    \end{lemma}
    \begin{lemma}\label{lem:ind_sec_unc_comb}
        If all of $\{\Sigma_i\}_{i\in[n]}$ satisfies efficiency and one of $\{\Sigma_i\}_{i\in[n]}$, satisfies both correctness and (one-time) IND-CPA security, then $\Sigma$ satisfies (one-time) IND-CPA security.
    \end{lemma}
    \begin{lemma}\label{lem:sec_unc_comb}
        If all of $\{\Sigma_i\}_{i\in[n]}$ satisfies efficiency and one of $\{\Sigma_i\}_{i\in[n]}$, satisfies both correctness and (one-time) unclonable IND-CPA security, then $\Sigma$ satisfies (one-time) unclonable IND-CPA security.
    \end{lemma}
\cref{lem:eff_unc_comb,lem:cor_unc_comb} trivially follows, and thus we skip the proof.
The proof of \cref{lem:ind_sec_unc_comb} is the same as that of \cref{lem:sec_unc_comb}, and thus we skip the proof.
\begin{proof}[Proof of \cref{lem:sec_unc_comb}]
    We prove the \cref{lem:sec_unc_comb} via a standard hybrid argument.
    For the reader's convenience, we describe the proof.
    For simplicity, we consider the one-time case where $\Sigma_i$ is a candidate of one-time unclonable secret-key encryption for each $i\in[n]$.
    We show that $\Sigma$ satisfies unclonable IND-CPA security as long as all of $\{\Sigma_i\}_{i\in[n]}$ satisfy efficiency and one of $\{\Sigma_i\}_{i\in[n]}$ satisfies one-time unclonable IND-CPA security.
    Let $\Sigma_x$ be the candidate for one-time unclonable secret-key encryption that satisfies both correctness and one-time unclonable IND-CPA security.
    Then, $\Sigma_x^*$ satisfies unclonable IND-CPA security from \cref{lem:unclone_ske_cor}.
    Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ that breaks the one-time unclonable IND-CPA security of $\Sigma$, and then construct a set of QPT adversaries $(\widetilde{\cA_x},\widetilde{\cB_x},\widetilde{\cC_x})$ that breaks the one-time unclonable security of $\Sigma_x^*$. 
    \begin{enumerate}
        \item $\widetilde{\cA_x}$ receives $(m_0,m_1)$ from $\cA$.
        \item $\widetilde{\cA_x}$ samples $r_i\la\bit^{\ell(\secp)}$ for all $i\in[n]\backslash x$, and sends $(M_0\seteq m_0+\sum_{i\in[n]\backslash x}r_i,M_1\seteq m_1+\sum_{i\in [n]\backslash x}r_i)$ to the challenger of $\Sigma_x^*$.
        \item The challenger of $\Sigma_x^*$ samples $b\la\bit$, and runs $\ct_x[M_b]^*\la\Enc_x^*(1^\secp,\sk_x^*,M_b)$.
        \item $\widetilde{\cA_x}$ receives from $\ct_x[M_b]^*$, runs $\sk_i^*\la\keygen_i^*(1^\secp)$ for all $i\in[n]\backslash x$, samples $r_i$ for all $i\in[n]\backslash x$, runs $\ct_i[r_i]^*\la\Enc_i^*(1^\secp,\sk_i^*,r_i)$, and sends $(\ct_1[r_1]^*,\cdots, \ct_{x-1}[r_{x-1}]^*,\ct_x[M_b]^*,\ct_{x+1}[r_{x+1}]^*,\cdots, \ct_{n}[r_{n}]^*)$ to $\cA$.
        \item When $\cA$ outputs $\rho_{\cB,\cC}$, $\widetilde{\cA_x}$ sends $\{\sk_i\}_{i\in[n]\backslash x}$ and the $\cB$ register (resp. the $\cC$ register) to $\widetilde{\cB_x}$ (resp. $\widetilde{\cC_x}$).
        \item $\widetilde{\cB_x}$ and $\widetilde{\cC_x}$ receive $\sk_x^*$ from the challenger of $\Sigma_x^*$.
        \item $\widetilde{\cB_{x}}$ (resp. $\widetilde{\cC_x}$) sends $\{\sk_i^*\}_{i\in[n]}$ and the $\cB$ register to $\cB$ (resp. the $\cC$ register to $\cC$).
        \item The experiment outputs $1$ if $b=b_\cB=b_\cC$, where $b_\cB$ (resp. $b_\cC$) is the output of $\cB$ (resp. $\cC$).
    \end{enumerate}
From the construction of $(\widetilde{\cA_x},\widetilde{\cB_x},\widetilde{\cC_x})$, it perfectly simulates the challenger of $\Sigma$. Therefore, if $(\cA,\cB,\cC)$ breaks the one-time unclonable IND-CPA security of $\Sigma$, then $(\widetilde{\cA_x},\widetilde{\cB_x},\widetilde{\cC_x})$ breaks the one-time unclonable IND-CPA security of $\Sigma_x^*$.
\end{proof}    
\end{proof}

\subsection{Universal Constructions}
\begin{definition}
    We say that a set of uniform QPT algorithms $\Sigma_{\mathsf{Univ}}=(\keygen,\Enc,\Dec)$ is a universal construction of (one-time) unclonable SKE (resp. PKE) if $\Sigma_{\mathsf{Univ}}$ is (one-time) unclonable SKE (resp. PKE) as long as there exists (one-time) unclonable SKE (resp. PKE).
\end{definition}
We give a universal construction of unclonable encryption via robust combiners.

\paragraph{Universal Construction via Robust Combiner}
\begin{theorem}\label{thm:univ_unc}
    There exists a universal construction of (one-time) unclonable SKE and unclonable PKE.
\end{theorem}
The proof is almost the same as \cref{thm:univ_owsg}, and thus we skip the proof.

\if0
\paragraph{Universal Construction via Decomposable Quantum Randomized Encoding}
Below, we give another universal construction of a one-time unclonable secret-key encryption for $n(\secp)$-bit plaintexts spaces by using decomposable quantum randomized encoding.
Let us introduce some notations.
\paragraph{Notations.}
\begin{itemize}
    \item
    We assume that there exists one-time unclonable secret-key encryption for $n(\secp)$-bit plaintexts.
    Then, from \cref{prop:perfect_unc}, there exists one-time unclonable secret-key encryption with perfect correctness, and the secret key is uniformly randomly sampled.
    Let $\Sigma_\unc\seteq \Unc. (\keygen,\Enc,\Dec)$ be the one-time unclonable secret-key encryption with $n(\secp)$-bit plaintexts, where it satisfies perfect correctness and the secret key is uniformly randomly sampled.
    \item Let $s$ be a polynomial such that $s(\secp)$ is the length of secret-key that $\Unc.\keygen(1^\secp)$ generates for all security parameters $\secp\in\N$.
    Let $q$ be a polynomial such that $q(\secp)$ is the length of quantum ciphertext that $\Unc.\Enc(1^\secp,\unc.\sk,m)$ generates for all security parameters $\secp\in\N$.
    \item For polynomial $p$ and $\secp\in\N$, let $U_{3p(\secp),p(\secp)}$
    be a universal quantum circuit over $\{I,H,CNOT,T\}$ (\cref{def:universal_circuit}) acting over $3p(\secp)+q(\secp)$-length input for some polynomial $q$, where the last $q(\secp)$ bit encodes circuit information.
    \item 
    For polynomial $p$, let $\Dec_{\secp,p}$ be a quantum circuit family consisting of $\{I,H,CNOT,T\}$ with $3p(\secp)$-length input and $p(\secp)$-depth that implements $\Unc.\Dec$.
    In other words, for any $C\in\Dec_{\secp,p}$, it holds that
    \begin{align}
        \Pr[m\la C((\unc\ct\otimes Z) \otimes (X\otimes Y) \otimes 0^{p(\secp)}):
        \begin{array}{ll}
            \unc.\ct\la\Unc.\Enc(1^\secp,X,m)
        \end{array}
        ]= 1
    \end{align}
    for any $m\in\bit^{n(\secp)}$, $X\in\bit^{s(\secp)}$, $Y\in\bit^{p(\secp)-s(\secp)}$ and $Z\in\bit^{p(\secp)-q(\secp)}$.
    \item 
    Let $D_{\secp,p}\subseteq \bit^{q(\secp)}$ be a family such that for all $d\in D_{\secp,p}$, there exists $D\in\Dec_{\secp,p}$ such that
    \begin{align}
        U_{3p(\secp),p(\secp)}(\ket{\psi}\otimes \ket{d})= D\ket{\psi} \otimes \ket{d}. 
    \end{align}
    \item 
    For $\secp\in\N$, polynomial $p$, $m\in\bit^{n(\secp)}$, let $\cC_{\secp,p}[m]$ be a quantum circuit family consisting of $\{I,H,CNOT,T\}$ on $3p(\secp)$-length input and $p(\secp)$-depth that outputs $m$.
    In other words, for any $C\in \cC_{\secp,p}[m]$, we have
    \begin{align}
        \Pr[m \la C(x\otimes k \otimes 0^{p(\secp)} )]=1
    \end{align}
    for any $x\in\bit^{p(\secp)}$ and $k\in\bit^{p(\secp)}$.
    \item Let $C_{\secp,p}[m]\subseteq \bit^{q(\secp) }$ be a family such that for all $c_m\in C_{\secp,p}[m]$, there exists a circuit $C[m]\in\cC_{\secp,p}[m]$ such that
    \begin{align}
        U_{3p(\secp),p(\secp)}(\ket{\psi}\otimes \ket{c_m})=C[m]\ket{\psi}\otimes\ket{y}.
    \end{align}
    \item Let $\Sigma_{\RE}\seteq \RE.(\Enc,\Dec)$ be a decomposable quantum randomized encoding.
    Given quantum circuit $C$ and $n_1$-length quantum input and $n_2$-length classical input $\mathbf{q}$ and $x$,
    the encoding $\widehat{C}(\mathbf{q},x)$ can be written
    \begin{align}
        (\widehat{C}_{\mathsf{off}},
        \widehat{C}_{1},\cdots,\widehat{C}_{n_1+n_2})\la \widehat{C}(\mathbf{q},x,r,e),
    \end{align}
    where $r$ is uniformly ransom string and $e$ is some quantum state.
    From decomposability, $\widehat{C}_{\mathsf{off}}$ acts only on $r$ and $e$.
    Moreover, 
    each $\widehat{C_i}(x_i,r_i)$ and $\widehat{C_i}(\mathbf{q}_i,r,e)$ can be computed separately, and $\widehat{C_i}(x_i,r)$ is classical string for $i\in\{n_1+1,\cdots ,n_1+n_2\}$.
    For any quantum circuit $C$, we write $\lab[i,x_i]= \widehat{C_i}(x_i,r_i)$ and $\lab[i,\mathbf{q}_i]=\widehat{C_i}(\mathbf{q}_i,r,e)$. 
\end{itemize}

\paragraph{Construction}
We give a construction of one-time unclonable secret-key encryption with $n(\secp)$-bit plaintexts $\Sigma\seteq(\keygen,\Enc,\Dec)$.
\begin{description}
    \item[$\keygen(1^\secp)$:]$ $
    \begin{itemize}
        \item Sample $x\la\bit^{p(\secp)}$.
        \item Sample $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Output $\sk\seteq \left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$.
    \end{itemize}
    \item[$\Enc(1^\secp,\sk,m)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$.
        \item Let $c_m\in C_{\secp,p}[m]$.
        \item Compute $\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}$.
        \item Compute 
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[p(\secp)]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,b]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,c_m[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item Sample $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Compute $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp),x[i]]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]+\lab[i+p(\secp),x[i]+1]$ for all $i\in[p(\secp)]$.
        \item Output 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,0]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,b]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
    \end{itemize}
    \item[$\Dec(1^\secp,\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$
        and
        \begin{align}    
        \ct=\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,b]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
        \item Compute $ \lab[i+p(\secp),x[i]]\seteq R[i]+\Lab.\ct[i+p(\secp),x[i]]$ for all $i\in[p(\secp)]$.
        \item Compute 
        \begin{align}
            \RE.\Dec\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}},
            \begin{array}{ll}
                &  \{\lab[i,0]\}_{i\in[p(\secp)]},
        \{\lab[i,x[i]]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\}} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
            \end{array}
            \right)
        \end{align}
        and outputs its output.
    \end{itemize}
\end{description}

\begin{lemma}\label{lem:univ_eff_garble}
$\Sigma$ satisfies efficiency if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding.
\end{lemma}

\begin{lemma}\label{lem:univ_cor_garble}
    $\Sigma$ satisfies correctness if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding.
\end{lemma}

\begin{lemma}\label{lem:ind-cpa_garble}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption, then $\Sigma$ satisfies one-time IND-CPA security for some polynomial $p$.
\end{lemma}

\begin{lemma}\label{thm:univ_unc_garble}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption, then $\Sigma$ satisfies one-time unclonable IND-CPA security for some polynomial $p$.
\end{lemma}
\cref{lem:univ_eff_garble} straightforwardly follows.
\cref{lem:univ_cor_garble} follows because for any $c_m\in C_{\secp,p}[m]$, we have some $C[m]\in \cC_{\secp,p}[m]$ such that
\begin{align}
    U_{3p(\secp),p(\secp)}(\ket{\psi}\otimes\ket{c_m})=C[m](\ket{\psi})\otimes\ket{c_m}
\end{align}
for any $\ket{\psi}$, and
moreover,
$C[m]$ satisfies
\begin{align}
    \Pr[m\la C[m](x\otimes k\otimes 0^{p(\secp)}) ]=1
\end{align}
for any $x\in\bit^{p(\secp)}$ and $k\in\bit^{p(\secp)}$.

\cref{lem:ind-cpa_garble} is the same as \cref{thm:univ_unc_garble}, and thus we omit the proof.
\begin{proof}[Proof of \cref{thm:univ_unc_garble}]
For appropriate polynomial $p$, there is a quantum circuit $D\in\Dec_{\secp,p}$.
From the property of $U_{3p(\secp),p(\secp)}$, there exists a subset $D_{\secp,p}\subseteq \bit^{q(\secp)}$ such that for all $d\in D_{\secp,p}$ there exists a quantum circuit $D\in\Dec_{\secp,p}$ that satisfies
\begin{align}
    U_{3p(\secp),p}(\ket{\psi}\otimes \ket{d})=D\ket{\psi}\otimes \ket{d}.
\end{align}
We fix such $d$.
We consider a fixed string $c_{m_b}\in C_{\secp,p}[m_b]$.
We describe the sequence of hybrids against adversary $(\cA,\cB,\cC)$.
\begin{description}
    \item[$\mathsf{Hyb_0}$:] This is the original one-time unclonable IND-CPA security experiment.
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}$
        and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[p(\secp)]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,c_{m_b}[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp),x[i]]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]+\lab[i+p(\secp),x[i]+1]$ for all $i\in[p(\secp)]$.
        \item The challenger sends 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,0]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,c_{m_b}[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
        to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:]$ $
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$. 
        We write $X$ to mean the first $s(\secp)$ bit of $x$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes  $\unc.\ct_b\la\Unc.\Enc(1^\secp,X,m_b)$, where $\unc.\ct_b$ is the $q(\secp)$-length quantum states.
        For $i\in\{q(\secp)+1,\cdots, p(\secp)\}$, set $\unc.\ct_b[i]\seteq 0$.
        \item The challenger computes $\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}$ and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[p(\secp)]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,d[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp),x[i]]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]+\lab[i+p(\secp),x[i]+1]$ for all $i\in[p(\secp)]$.
        \item The challenger sends 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,d[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right)
        \end{align}
        to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
\end{description}
\cref{thm:univ_unc_garble} follows from the following \cref{prop:hyb_0_hyb_1_univ_unc_garble,prop:hyb_1_univ_unc_garble}.
\begin{proposition}\label{prop:hyb_0_hyb_1_univ_unc_garble}
    If $\Sigma_\RE$ is decomposable quantum randomized encoding, then
    \begin{align}
        \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\leq \negl(\secp).
    \end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_1_univ_unc_garble}
If there exists one-time secret-key unclonable encryption with $n(\secp)$-bit plaintext, then
\begin{align}
    \Pr[\mathsf{Hyb_1}]\leq \frac{1}{2}+\negl(\secp).
\end{align}
\end{proposition}
\end{proof}
\begin{proof}[Proof of \cref{prop:hyb_0_hyb_1_univ_unc_garble}]
Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/\secp^K
\end{align}
for all sufficiently large security parameters $\secp\in\N$.
Then, construct a QPT adversary $\widetilde{\cA}$ that breaks the security of $\Sigma_{\RE}$ as follows.
\begin{enumerate}
    \item $\widetilde{\cA}$ samples $b\la\bit$.
    \item $\widetilde{\cA}$ samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$. We write $X$ to mean the first $s(\secp)$ bits of $x$.
    \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
    \item $\widetilde{\cA}$ computes $\unc.\ct_b\la\Unc.\Enc(1^\secp,X,m_b)$, where $\unc.\ct_b$ is the $q$-length quantum state.
    \item $\widetilde{\cA}$ sends $\left(\{U_{3p(\secp),p(\secp)},0^{p(\secp)},x,0^{p(\secp)},c_{m_b}\},  \{ U_{3p(\secp),p(\secp)},\left(\unc.\ct_b,0^{p(\secp)-q(\secp)}\right),x,0^{p(\secp)},d \} \right)$ to the challenger of $\Sigma_{\mathsf{RE}}$ in \cref{prop:ind_RE}.
    \item The challenger samples $b^*\la\bit$, and does the following.
    \begin{itemize}
        \item If $b^*=0$, then the challenger computes 
        \begin{align}
         \left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[3p(\secp)+q(\secp)]}\right)\la
         \RE.\Enc\left(1^\secp,U_{3p(\secp),p(\secp)},\left(0^{p(\secp)},x,0^{p(\secp)},c_{m_b}\right)\right),  
        \end{align}
         and sends $\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[3p(\secp)+q(\secp)]}\right)$ to $\widetilde{\cA}$.
        % and sends $\left(\widehat{C[m_b]}_{\mathsf{off}}, \{\widehat{C[m_b]}_i(0;r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
        \item If $b^*=1$, then the challenger computes 
        \begin{align}
         \left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[3p(\secp)+q(\secp)]}\right)\la
         \RE.\Enc\left(1^\secp,U_{3p(\secp),p(\secp)},\left(\unc.\ct_b,0^{p(\secp)-q(\secp)},x,0^{p(\secp)},d)\right)\right),  
        \end{align}
        and sends $\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[3p(\secp)+q(\secp)]}\right)$ to $\widetilde{\cA}$.
        %and sends $\left(\widehat{D}[\unc.\sk,m_0,m_1]_{\mathsf{off}}, \{\widehat{D}[\unc.\sk,m_0,m_1]_i(\unc.\ct_b[i];r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
    \end{itemize}
    %\item $\widetilde{\cA}$ receives $(\widehat{F}_{\mathsf{off}},\{\mathsf{lab}[i]\}_{i\in[s(\secp)+p(\secp)]})$ from the challenger. Here, if $b^*=0$, then $(\widehat{F}_{\mathsf{off}},\{\mathsf{lab}[i]\}_{i\in[s(\secp)+p(\secp)]})=\left(\widehat{C[m_b]}_{\mathsf{off}}, \{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{ \lab[i,0]\}_{i\in \{s(\secp)+1,\cdots,s(\secp)+p(\secp)\}}\right)$. Otherwise, $(\widehat{F}_{\mathsf{off}},\{\lab[i]\}_{i\in[s(\secp)+p(\secp)]})=\left(\widehat{\Unc.\Dec}_{\mathsf{off}}, \{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{\lab[i,\unc.\ct_b[i]]\}_{\{s(\secp)+1,\cdots,s(\secp)+p(\secp)\}}\right)$.
    %\item $\widetilde{\cA}$ computes $\{\lab[i,x[i]+1]\}_{i\in[s(\secp)]}$.
    %\taiga{I think I need to explain why $\widetilde{\cA}$ can do this.}
    \item $\widetilde{\cA}$ samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, computes $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp)]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]$ for all $i\in[p(\secp)]$, and runs $\cA$ on 
    \begin{align}    
        \ct\seteq\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right),
    \end{align}
    and generates $\rho_{\cB,\cC}$.
    \item $\widetilde{\cA}$  sends the corresponding register to $\cB$ and $\cC$, respectively.
    \item $\widetilde{\cA}$ sends $x$ and $\{R[i]\}_{i\in[p(\secp)]}$ to $\cB$ and $\cC$.
    \item $\cB$ and $\cC$ outputs $b_\cB$ and $b_\cC$, respectively.
    \item $\widetilde{\cA}$ outputs $1$ if $b=b_\cB=b_\cC$, and outputs $0$ otherwise.
\end{enumerate}
From the construction of $\widetilde{\cA}$, if $b^*=0$, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_0}$.
Otherwise, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_1}$.
Furthermore, we have 
\begin{align}
U_{3p(\secp),p(\secp)}(0^{p(\secp)},x,0^{p(\secp)},c_b)=U_{3p(\secp),p(\secp)}(\unc.\ct_b,0^{p(\secp)-q(\secp)},x,0^{p(\secp)},d)=m_b.
\end{align}
Therefore, if there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/\secp^K
\end{align}
for all sufficiently large security parameters $\secp\in\N$,
then it contradicts that $\Sigma_{\RE}$ satisfies security from \cref{prop:ind_RE}.
\end{proof}

\begin{proof}[Proof of \cref{prop:hyb_1_univ_unc_garble}]
    Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/\secp^K
    \end{align}
    for all sufficiently large security parameters $\secp\in\N$.
    Then, construct a QPT adversary $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$ that breaks the one-time unclonable IND-CPA security of $\Sigma_\unc$ as follows.
    \begin{enumerate}
        \item The challenger of $\Sigma_{\unc}$ samples $b\la\bit$.
        \item $\widetilde{\cA}$ samples $Y\la\bit^{p(\secp)-s(\secp)}$ and $R[i,\beta]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
        \item $\widetilde{\cA}$ sends $( m_0,m_1)$ to the challenger, and receives $\unc.\ct_b$, where the challenger samples $X\la\bit^{s(\secp)}$ and runs $\unc.\ct_b\la\Unc.\Enc(1^\secp,X,m_b)$.
        \item $\widetilde{\cA}$ computes $\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}$ and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[p(\secp)]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,d[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item $\widetilde{\cA}$ computes $\Lab.\ct[i+p(\secp),\beta]]\seteq R[i,\beta]+\lab[i+p(\secp),\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ runs $\cA$ on 
        \begin{align}
        \left( \widehat{U}_{3p(\secp),p(\secp)},
        \begin{array}{ll}
             \{\lab[i,\unc.\ct_b[i]]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},
             \{\lab[i,d[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right)
        \end{align}
        , obtains $\rho_{\cB,\cC}$, and sends the $\cB$ register and $(Y,\{R[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit})$ to $\widetilde{\cB}$ and $\cC$ register and $(Y,\{R[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit})$ to $\widetilde{\cC}$.
        \item $\widetilde{\cB}$ (resp. $\widetilde{\cC}$) receives the secret-key $X$ from the challenger of $\Sigma_{\unc}$, sets $x\seteq X||Y$, and sends $(x,\{R[i,x[i]]\}_{i\in[p(\secp)]})$ and the $\cB$ register (resp. $\cC$ register) to $\cB$ (resp. $\cC$). 
        \item The experiment outputs $1$ if $b=b_\cB=b_\cC$ where $b_\cB$ and $b_\cC$ are the output of $\cB$ and $\cC$, respectively.
    \end{enumerate}
    From the construction of $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$, the adversary perfectly simulates the challenger of $\mathsf{Hyb_1}$. Therefore, if there exists a QPT adversary $(\cA,\cB,\cC)$ and some constant $K$ such that 
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/\secp^K
    \end{align}
     for all sufficiently large security parameters $\secp\in\N$, it contradicts $\Sigma_{\unc}$ satisfies unclonable IND-CPA security.
\end{proof}
\fi


\section{Universal Plaintext Extension for Unclonable Encryption}\label{Sec:expanstion_UE}
In this section, we prove the following \cref{thm:unclone_multi_space}.
\begin{theorem}\label{thm:unclone_multi_space}
    If there exists a decomposable quantum randomized encoding, then for all polynomial $n$, we can construct a set of uniform QPT algorithms $\Sigma=(\keygen,\Enc,\Dec)$ such that $\Sigma$ is a one-time unclonable secret-key encryption with $n(\secp)$-bit plaintexts \takashi{"with (or for) $n(\secp)$-bit plaintexts" sounds more natural} as long as there exists one-time unclonable secret-key encryption for single-bit plaintexts.
\end{theorem}

\takashi{add a remark that in particular this gives a universal construction since the construction does not depend on the single-bit scheme that is assumed to exist.}



As corollaries,
we obtain \cref{cor:unclone_expnasion,cor:pub_unclone_expansion}
\begin{corollary}\label{cor:unclone_expnasion}
    For all polynomial $n$, there exists a set of uniform QPT algorithm $\Sigma=(\keygen,\Enc,\Dec)$ such that $\Sigma$ is unclonable secret-key encryption with $n(\secp)$-bit plaintexts as long as there exists unclonable secret-key encryption for single-bit plaintexts.
\end{corollary}
\begin{corollary}\label{cor:pub_unclone_expansion}
    For all polynomial $n$, there exists a set of uniform QPT algorithm $\Sigma=(\keygen,\Enc,\Dec)$ such that $\Sigma$ is unclonable public-key encryption with $n(\secp)$-bit plaintexts as long as there exists unclonable public-key encryption for single-bit plaintexts.
\end{corollary}
\begin{proof}[Proof of \cref{cor:pub_unclone_expansion}]
    We give a rough sketch of the proof of \cref{cor:pub_unclone_expansion}. Note that, in the same way, we can prove \cref{cor:unclone_expnasion}.
    
    We can construct PKE with quantum ciphertext and one-time unclonable SKE with single-bit plaintexts from unclonable PKE for single-bit plaintexts.
    We can construct decomposable quantum randomized encoding from PKE with quantum ciphertext.
    Furthermore, from \cref{thm:unclone_multi_space}, we can construct one-time unclonable SKE with $n(\secp)$-bit plaintexts from decomposable quantum randomized encoding and one-time unclonable SKE with single-bit plaintexts.

    On the other hand, we can construct receiver non-committing encryption with quantum ciphertext from PKE with quantum ciphertext.
    By combining the receiver non-committing encryption with quantum ciphertext and one-time unclonable secret-key encryption with $n(\secp)$-bit plaintexts, we obtain unclonable public-key encryption with $n(\secp)$-bit plaintexts (For the detail, see \cref{sec:app_unc_pke}).
\end{proof}


\begin{proof}[Proof of \cref{thm:unclone_multi_space}]
First, let us describe notations and observations.


\paragraph{Notations and observations.}
\begin{itemize}
    \color{red}
    \item
    For a polynomial $p$, let $C_{\secp,p}$ be a class of general quantum circuits of size $p(\secp)$ with $\secp$-qubit quantum inputs and $\secp$-bit classical inputs.
    For a polynomial $p$, let $U_{\secp,p}$ be a general quantum circuit that takes a description of a quantum circuit $C\in \cC_{\secp,p}$, $\secp $-qubit quantum state $\rho$, and $\secp$-bit classical string $x$ and outputs $C(\rho,x)$.
    \item 
    Let $C_{\secp,p}[m]$ be a quantum circuit of size $p(\secp)$ with $\secp$-qubit quantum inputs and $\secp$-bit classical inputs such that it outputs $m$ for any inputs.
    \color{black}
    \item
    We assume that there exists one-time unclonable secret-key encryption for single-bit plaintexts.
    Then, from \cref{prop:perfect_unc}, there exists one-time unclonable secret-key encryption with perfect correctness, and the secret key is uniformly randomly sampled.
    Let $\Sigma_\unc\seteq \Unc. (\keygen,\Enc,\Dec)$ be the one-time unclonable secret-key encryption with single-bit plaintexts, where it satisfies perfect correctness and the secret key is uniformly randomly sampled. \takashi{Note that it is not used in our construction and only appears in the security proof. It may be better to state this after the constructio to avoid the confusion.}
    \item By standard padding argument, without loss of generality, we can assume that $\abs{\sk_{\secp}}=\abs{\ct_{\secp,b}}=\secp$ for any $\secp\in\N$ and $b\in\bit$, where $\sk_{\secp}\la\Unc.\keygen(1^\secp)$ and $\ct_{\secp,b}\la\Unc.\Enc(1^\secp,\sk,b)$. 
    \item By standard padding argument, without loss of generality, we can assume that $\Unc.\Dec(1^\secp,\sk,\ct)$ works as follows.
    $\Unc.\Dec(1^\secp,\sk,\ct)$ first appends auxiliary qubits $0^{\secp}$ to $\ct$, and $\sk$, and runs some quantum circuits $\Dec_{\secp}$ with depth $\secp$ \takashi{I don't see why depth matters here.} on $(\ct,\sk,0^{\secp})$, and outputs its output.
    \takashi{I feel the following definition of $U_{p(\secp),p(\secp)}$ is unnecessarily complicated. 
    Can't we simply say as follows? 
    Let $\mathcal{C}_\secp$ be a class of general quantum circuits of size $p(\secp)$ with $\secp$-qubit quantum inputs and $\secp$-bit classical inputs. 
    Let $U_\secp$ be a general quantum circuit that takes a description of a quantum circuit $C\in \mathcal{C}_\secp$, $\secp$-qubit quantum state $\rho$, and $\secp$-bit classical string $x$ and outputs $C(\rho,\secp)$. 
    In this way, we can avoid taking about ancilla and also avoid explicitly using universal quantum circuits. 
    (The above explanation implicitly uses universal quantum circuits, but I don't think we need to make all the details formal.)  
    }
    \item 
    For a security parameter $\secp$ and $m_0,m_1\in\bit^{n(\secp)}$, let $D_{\secp}[m_0,m_1]$ be a quantum circuit over $\{I,H,CNOT,T\}$ that takes $p(\secp)$-length input and has $p(\secp)$-depth working as follows:
    If the input of $D_{\secp}[m_0,m_1]$ is of the form $(\ct,\sk,0^{p(\secp)-2\secp})$, $D_{\secp}[m_0,m_1]$ first runs the circuit $\Dec_{\secp}$ on $(\ct,\sk,0^{\secp})$, obtains $b$, and outputs $m_b$. 
    Now, we define $p$ as a polynomial large enough to run the circuit $D_{\secp}[m_0,m_1]$. \takashi{I think this makes the construction dependent on $p$, which depends on the single-bit scheme. In that case, this is not completely a universal construction?}
    \item 
    We define $d_{m_0,m_1}\in\bit^{q(\secp)}$ as the string such that:
    \begin{align}
        U_{p(\secp),p(\secp)}(\ket{\psi}\otimes \ket{d_{m_0,m_1}})= D_{\secp}[m_0,m_1]\ket{\psi} \otimes \ket{d_{m_0,m_1}}. 
    \end{align}
    \item 
    For $\secp\in\N$, and $m\in\bit^{n(\secp)}$, let $\cC_{\secp}[m]$ be a quantum circuit over $\{I,H,CNOT,T\}$ that takes $p(\secp)$-length input and $p(\secp)$-depth working as follows:
    If the input of $C_\secp[m]$ is of the form $(\ct,\sk,0^{p(\secp)-2\secp})$, then $C_{\secp}[m]$ outputs $m$ for any $\ct$ and $\sk$. 
    \item We define $c_m\in\bit^{q(\secp)}$ as the string such that:
    \begin{align}
        U_{p(\secp),p(\secp)}(\ket{\psi}\otimes \ket{c_m})= C_{\secp}[m]\ket{\psi} \otimes \ket{c_{m}}.
    \end{align}
    \item Let $\Sigma_{\RE}\seteq \RE.(\Enc,\Dec)$ be a decomposable quantum randomized encoding.
    Given quantum circuit $C$ and $n_1$-length quantum input and $n_2$-length classical input $\mathbf{q}$ and $x$,
    the encoding $\widehat{C}(\mathbf{q},x)$ can be separated as follows:
    \begin{align}
        \widehat{C}(\mathbf{q},x,r,e)=(\widehat{C}_{\mathsf{off}},
        \widehat{C}_{1},\cdots,\widehat{C}_{n_1+n_2})(\mathbf{q},x,r,e),
    \end{align}
    where $r$ is uniformly ransom string and $e$ is some quantum state.
    From decomposability, $\widehat{C}_{\mathsf{off}}$ acts only on $r$ and $e$, and $\widehat{C_i}$ acts only on $\mathbf{q_i}, r$ and $e$ for $i\in[n_1]$, and $\widehat{C_i}$ acts only on $x_i$ and $r$ for $i\in\{n_1+1,\cdots,n_1+n_2\}$.
    For any quantum circuit $C$, we write $\lab[i,x_i]= \widehat{C_i}(x_i,r_i)$ and $\lab[i,\mathbf{q}_i]=\widehat{C_i}(\mathbf{q}_i,r,e)$. 
\end{itemize}
\paragraph{Construction.}
We give a construction of one-time unclonable secret-key encryption  $\Sigma\seteq(\keygen,\Enc,\Dec)$ with $n(\secp)$-bit plaintexts by using decomposable quantum randomized encoding.
In the construction, we only use decomposable quantum randomized encoding.
The construction is secure as long as the underlying decomposable quantum randomized encoding is secure and there exists one-time unclonable secret-key encryption for single-bit plaintexts.
\begin{description}
    \item[$\keygen(1^\secp)$:]$ $
    \begin{itemize}
        \item Sample $x\la\bit^{\secp}$.
        \item Sample $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[\secp]$.
        \item Output $\sk\seteq \left(x,\{R[i]\}_{i\in[\secp]}\right)$.
    \end{itemize}
    \item[$\Enc(1^\secp,\sk,m)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[\secp]}\right)$.
        \item Compute $\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}$.
        \item Compute 
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[\secp]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,b]\}_{i\in \{\secp+1,\cdots,2\secp\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,c_m[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item Sample $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[\secp]$.
        \item Compute $\Lab.\ct[i+\secp,x[i]]\seteq R[i]+\lab[i+\secp,x[i]]$ and $\Lab.\ct[i+\secp,x[i]+1]\seteq S[i]+\lab[i+\secp,x[i]+1]$ for all $i\in[\secp]$.
        \item Output 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,0]\}_{i\in[\secp]},
        \{\Lab.\ct[i,b]\}_{i\in \{\secp+1,\cdots,2\secp\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
    \end{itemize}
    \item[$\Dec(1^\secp,\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[\secp]}\right)$
        and
        \begin{align}    
        \ct=\left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[\secp]},
        \{\Lab.\ct[i,b]\}_{i\in \{\secp+1,\cdots,2\secp\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
        \item Compute $ \lab[i+\secp,x[i]]\seteq\Lab.\ct[i+\secp,x[i]]+R[i]$ for all $i\in[\secp]$.
        \item Compute 
        \begin{align}
            \RE.\Dec\left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}},
            \begin{array}{ll}
                &  \{\lab[i,0]\}_{i\in[\secp]},
        \{\lab[i,x[i]]\}_{i\in \{\secp+1,\cdots,2\secp\}} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}
            \end{array}
            \right)
        \end{align}
        and outputs its output.
    \end{itemize}
\end{description}
\begin{lemma}\label{lem:extend_eff}
    $\Sigma$ satisfies efficiency if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding.
\end{lemma}
\begin{lemma}\label{lem:extend_cor}
    $\Sigma$ satisfies correctness if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding.
\end{lemma}
\begin{lemma}\label{lem:expand_sec}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption with single-bit plaintexts,
    $\Sigma$ satisfies one-time IND-CPA security for some polynomial $p$.
\end{lemma}

\begin{lemma}\label{thm:expnad_unc}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption with single-bit plaintexts,
    $\Sigma$ satisfies one-time unclonable IND-CPA security for some polynomial $p$.  
\end{lemma}
\cref{lem:extend_eff} straightforwardly follows.
We can see that \cref{lem:extend_cor} holds as follows.
First, if $\sk\la\keygen(1^\secp)$ and $\ct\la\Enc(\sk,m)$, $\Dec(\sk,\ct)$ outputs the output of $U_{p(\secp),p(\secp)}(0^{\secp},x,0^{p(\secp)-2\secp},c_{m})$ with overwhelming probability.
From the definition of $U_{p(\secp),p(\secp)}$ and $c_m$, $U_{p(\secp),p(\secp)}(0^{\secp},x,0^{p(\secp)-2\secp},c_{m})=C[m](0^{\secp},x,0^{p(\secp)-2\secp})=m$.

The proof of \cref{lem:expand_sec} is the same as \cref{thm:expnad_unc}, and thus we skip the proof.
\begin{proof}[Proof of \cref{thm:expnad_unc}]
Remind that, for $m_0,m_1\in\bit^{n(\secp)}$, $d_{m_0,m_1}\in\bit^{q(\secp)}$ satisfies
\begin{align}
U_{p(\secp),p(\secp)}(\ket{\psi} \otimes\ket{d_{m_0,m_1}}) = D_{\secp}[m_0,m_1] \ket{\psi} \otimes \ket{d_{m_0,m_1}}.
\end{align}
We describe the sequence of hybrids against the adversary $(\cA, \cB, \cC)$.
\begin{description}
        \item[$\mathsf{Hyb_0}$:] This is the original one-time unclonable IND-CPA security experiment.
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{\secp}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[\secp]$.
        \item $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}$
        and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[\secp]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{\secp+1,\cdots,2\secp\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,c_{m_b}[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[\secp]$, and computes $\Lab.\ct[i+\secp,x[i]]\seteq R[i]+\lab[i+\secp,x[i]]$ and $\Lab.\ct[i+\secp,x[i]+1]\seteq S[i]+\lab[i+\secp,x[i]+1]$ for all $i\in[\secp]$.
        \item The challenger sends 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,0]\}_{i\in[\secp]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{\secp+1,\cdots,2\secp\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\{\lab[i,c_{m_b}[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
        to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[\secp]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:]$ $
    \begin{enumerate}        
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{\secp}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[\secp]$. 
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\unc.\ct_b\la\Unc.\Enc(1^\secp,x,b)$, where $\unc.\ct_b$ is the $\secp$-length quantum states.
        \item The challenger computes $\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}$ and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[\secp]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{\secp+1,\cdots,2\secp\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,d_{m_0,m_1}[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[\secp]$, and computes $\Lab.\ct[i+\secp,x[i]]\seteq R[i]+\lab[i+\secp,x[i]]$ and $\Lab.\ct[i+\secp,x[i]+1]\seteq S[i]+\lab[i+\secp,x[i]+1]$ for all $i\in[\secp]$.
        \item The challenger sends 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[\secp]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{\secp+1,\cdots,2\secp\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\{\lab[i,d_{m_0,m_1}[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}
        \end{array}
        \right)
        \end{align}
        to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[\secp]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
\end{description}
\cref{thm:expnad_unc} follows from the following \cref{prop:hyb_0_hyb_1_unc_expand,prop:hyb_1_unc_expand}.
\begin{proposition}\label{prop:hyb_0_hyb_1_unc_expand}
If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding, then
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\leq\negl(\secp).
\end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_1_unc_expand}
    If there exists a one-time unclonable secret-key encryption $\Sigma_{\Unc}$ with single-bit plaintexts, then
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1=1]}\leq \frac{1}{2}+\negl(\secp).
    \end{align}
\end{proposition}
\end{proof}



\begin{proof}[Proof of \cref{prop:hyb_0_hyb_1_unc_expand}]
Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/\secp^K
\end{align}
for all sufficiently large security parameters $\secp\in\N$.
Then, construct a QPT adversary $\widetilde{\cA}$ that breaks the security of $\Sigma_{\RE}$ as follows.
\begin{enumerate}
    \item $\widetilde{\cA}$ samples $b\la\bit$.
    \item $\widetilde{\cA}$ samples $x\la\bit^{\secp}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[\secp]$.
    \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
    \item $\widetilde{\cA}$ computes $\unc.\ct_b\la\Unc.\Enc(1^\secp,x,m_b)$.
    \item $\widetilde{\cA}$ sends $\left(\{U_{p(\secp),p(\secp)},0^{\secp},x,0^{p(\secp)-2\secp},c_{m_b}\},  \{ U_{p(\secp),p(\secp)},\unc.\ct_b,x,0^{p(\secp)-2\secp},d_{m_0,m_1} \} \right)$ to the challenger of $\Sigma_{\mathsf{RE}}$ in \cref{prop:ind_RE}.
    \item The challenger samples $b^*\la\bit$, and does the following.
    \begin{itemize}
        \item If $b^*=0$, then the challenger computes 
        \begin{align}
         \left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[p(\secp)+q(\secp)]}\right)\la
         \RE.\Enc\left(1^\secp,U_{p(\secp),p(\secp)},\left(0^{\secp},x,0^{p(\secp)-2\secp},c_{m_b}\right)\right),  
        \end{align}
         and sends $\left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[p(\secp)+q(\secp)]}\right)$ to $\widetilde{\cA}$.
        % and sends $\left(\widehat{C[m_b]}_{\mathsf{off}}, \{\widehat{C[m_b]}_i(0;r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
        \item If $b^*=1$, then the challenger computes 
        \begin{align}
         \left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[p(\secp)+q(\secp)]}\right)\la
         \RE.\Enc\left(1^\secp,U_{p(\secp),p(\secp)},\left(\unc.\ct_b,,x,0^{p(\secp)-2\secp},d_{m_0,m_1}\right)\right),  
        \end{align}
        and sends $\left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[p(\secp)+q(\secp)]}\right)$ to $\widetilde{\cA}$.
        %and sends $\left(\widehat{D}[\unc.\sk,m_0,m_1]_{\mathsf{off}}, \{\widehat{D}[\unc.\sk,m_0,m_1]_i(\unc.\ct_b[i];r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
    \end{itemize}
    %\item $\widetilde{\cA}$ receives $(\widehat{F}_{\mathsf{off}},\{\mathsf{lab}[i]\}_{i\in[s(\secp)+p(\secp)]})$ from the challenger. Here, if $b^*=0$, then $(\widehat{F}_{\mathsf{off}},\{\mathsf{lab}[i]\}_{i\in[s(\secp)+p(\secp)]})=\left(\widehat{C[m_b]}_{\mathsf{off}}, \{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{ \lab[i,0]\}_{i\in \{s(\secp)+1,\cdots,s(\secp)+p(\secp)\}}\right)$. Otherwise, $(\widehat{F}_{\mathsf{off}},\{\lab[i]\}_{i\in[s(\secp)+p(\secp)]})=\left(\widehat{\Unc.\Dec}_{\mathsf{off}}, \{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{\lab[i,\unc.\ct_b[i]]\}_{\{s(\secp)+1,\cdots,s(\secp)+p(\secp)\}}\right)$.
    %\item $\widetilde{\cA}$ computes $\{\lab[i,x[i]+1]\}_{i\in[s(\secp)]}$.
    %\taiga{I think I need to explain why $\widetilde{\cA}$ can do this.}
    \item $\widetilde{\cA}$ samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, computes $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp)]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]$ for all $i\in[p(\secp)]$, and runs $\cA$ on 
    \begin{align}    
        \ct\seteq\left(\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i]\}_{i\in[\secp]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{\secp+1,\cdots,2\secp\},\beta\in\bit} \\
             &  \{\lab[i]\}_{i\in \{2\secp+1,\cdots,p(\secp)+q(\secp)\}}
        \end{array}
        \right),
    \end{align}
    and generates $\rho_{\cB,\cC}$.
    \item $\widetilde{\cA}$  sends the corresponding register to $\cB$ and $\cC$, respectively.
    \item $\widetilde{\cA}$ sends $x$ and $\{R[i]\}_{i\in[\secp]}$ to $\cB$ and $\cC$.
    \item $\cB$ and $\cC$ outputs $b_\cB$ and $b_\cC$, respectively.
    \item $\widetilde{\cA}$ outputs $1$ if $b=b_\cB=b_\cC$, and outputs $0$ otherwise.
\end{enumerate}
From the construction of $\widetilde{\cA}$, if $b^*=0$, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_0}$.
Otherwise, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_1}$.
Furthermore, we have 
\begin{align}
U_{p(\secp),p(\secp)}(0^{\secp},x,0^{p(\secp)-2\secp},c_b)=U_{p(\secp),p(\secp)}(\unc.\ct_b,x,0^{p(\secp)-2\secp},d_{m_0,m_1})=m_b.
\end{align}
Therefore, if there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/\secp^K
\end{align}
for all sufficiently large security parameters $\secp\in\N$,
then it contradicts that $\Sigma_{\RE}$ satisfies security from \cref{prop:ind_RE}.    
\end{proof}



\begin{proof}[Proof of \cref{prop:hyb_1_unc_expand}]
    Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq \frac{1}{2}+1/\secp^K
    \end{align}
    for all sufficiently large security parameters $\secp\in\N$.
    Then, construct a QPT adversary $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$ that breaks the unclonable IND-CPA security of $\Sigma_{\unc}$ as follows.
    \begin{enumerate}
        \item The challenger of $\Sigma_{\unc}$ samples $b\la\bit$.
        \item $\widetilde{\cA}$ samples $R[i,\beta]\la\bit^{\ell(\secp)}$ for all $i\in[\secp]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
        \item $\widetilde{\cA}$ sends $(0,1)$ to the challenger, and receives $\unc.\ct_b$, where $\unc.\ct_b\la \Unc.\Enc(1^\secp,x,b)$ and $x\la\bit^{\secp}$.
        \item $\widetilde{\cA}$ computes $\widehat{U}_{p(\secp),p(\secp)\mathsf{off}}$ and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[\secp]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{\secp+1,\cdots,2\secp\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,d_{m_0,m_1}[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item $\widetilde{\cA}$ computes $\Lab.\ct[i+\secp,\beta]]\seteq R[i,\beta]+\lab[i+\secp,\beta]$ for all $i\in[\secp]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ runs $\cA$ on 
        \begin{align}
        \left( \widehat{U}_{p(\secp),p(\secp)},
        \begin{array}{ll}
             \{\lab[i,\unc.\ct_b[i]]\}_{i\in[\secp]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{\secp+1,\cdots,2\secp\},\beta\in\bit} \\
             \{\lab[i,0]\}_{i\in \{2\secp+1,\cdots,p(\secp)\}},
             \{\lab[i,d_{m_0,m_1}[i]]\}_{i\in\{p(\secp)+1,\cdots,p(\secp)+q(\secp)\}}
        \end{array}
        \right),
        \end{align}
         obtains $\rho_{\cB,\cC}$, and sends the $\cB$ register and $\{R[i,\beta]\}_{i\in[\secp],\beta\in\bit}$ to $\cB$ and the $\cC$ register and $\{R[i,\beta]\}_{i\in[\secp],\beta\in\bit}$ to $\cC$.
        \item $\widetilde{\cB}$ (resp. $\widetilde{\cC}$) receives the secret-key $x$ from the challenger of $\Sigma_{\unc}$ and sends $(x,\{R[i,x[i]]\}_{i\in[\secp]})$ and the $\cB$ register (resp. $\cC$ register) to $\cB$ (resp. $\cC$). 
        \item The experiment outputs $1$ if $b=b_\cB=b_\cC$ where $b_\cB$ and $b_\cC$ are the output of $\cB$ and $\cC$, respectively.
    \end{enumerate}
From the construction of $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$, it perfectly simulates the challenger of $\mathsf{Hyb_1}$.
Therefore, if there exists some QPT adversaries $(\cA,\cB,\cC)$ and constant $K$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/\secp^K
    \end{align}
     for all sufficiently large security parameters $\secp\in\N$, it contradicts that $\Sigma_{\unc}$ satisfies unclonable IND-CPA security.
\end{proof}
\end{proof}



\if0
\paragraph{Notations.}
\begin{itemize}
    \item
    We assume that there exists one-time unclonable secret-key encryption for single-bit plaintexts.
    Then, from \cref{prop:perfect_unc}, there exists one-time unclonable secret-key encryption with perfect correctness, and the secret key is uniformly randomly sampled.
    Let $\Sigma_\unc\seteq \Unc. (\keygen,\Enc,\Dec)$ be the one-time unclonable secret-key encryption with single-bit plaintexts, where it satisfies perfect correctness and the secret key is uniformly randomly sampled.
    \item Let $s$ be a polynomial such that $s(\secp)$ is the length of secret-key that $\Unc.\keygen(1^\secp)$ generates for all security parameters $\secp\in\N$.
    Let $q$ be a polynomial such that $q(\secp)$ is the length of quantum ciphertext that $\Unc.\Enc(1^\secp,\unc.\sk,m)$ generates for all security parameters $\secp\in\N$.
    \item For polynomial $p$ and $\secp\in\N$, let $U_{3p(\secp),p(\secp)}$
    be a universal quantum circuit over $\{I,H,CNOT,T\}$ (\cref{def:universal_circuit}) acting on $3p(\secp)+q(\secp)$-length input for some polynomial $q$, where the last $q(\secp)$ bit encodes circuit information.
    \item 
    For a security parameter $\secp$, polynomial $p$, and $m_0,m_1\in\bit^{n(\secp)}$, let $\Dec_{\secp,p}[m_0,m_1]$ be a quantum circuit family consisting of $\{I,H,CNOT,T\}$ with $3p(\secp)$-length input and $p(\secp)$-depth that first implements $\Unc.\Dec$, obtains $b$, and outputs $m_b$.
    More formally, for any $D[m_0,m_1]\in\Dec_{\secp,p}[m_0,m_1]$, it holds that
    \begin{align}
        \Pr[m_b\la D[m_0,m_1]((\unc.\ct\otimes Z) \otimes (X\otimes Y) \otimes 0^{p(\secp)}):
        \begin{array}{ll}
            \unc.\ct\la\Unc.\Enc(1^\secp,X,b)
        \end{array}
        ]= 1
    \end{align}
    for any $m\in\bit^{n(\secp)}$, $X\in\bit^{s(\secp)}$, $Y\in\bit^{p(\secp)-s(\secp)}$ and $Z\in\bit^{p(\secp)-q(\secp)}$.
    \item 
    Let $D_{\secp,p}[m_0,m_1]\subseteq \bit^{q(\secp)}$ be a family such that for all $d_{m_0,m_1}\in D_{\secp,p}[m_0,m_1]$, there exists $D[m_0,m_1]\in\Dec_{\secp,p}[m_0,m_1]$ such that
    \begin{align}
        U_{3p(\secp),p(\secp)}(\ket{\psi}\otimes \ket{d_{m_0,m_1}})= D[m_0,m_1]\ket{\psi} \otimes \ket{d_{m_0,m_1}}. 
    \end{align}
    \item 
    For $\secp\in\N$, polynomial $p$, and $m\in\bit^{n(\secp)}$, let $\cC_{\secp,p}[m]$ be a quantum circuit family consisting of $\{I,H,CNOT,T\}$ on $3p(\secp)$-length input and $p(\secp)$-depth that outputs $m$.
    In other words, for any $C\in \cC_{\secp,p}[m]$, we have
    \begin{align}
        \Pr[m \la C(x\otimes k \otimes 0^{p(\secp)} )]=1
    \end{align}
    for any $x\in\bit^{p(\secp)}$ and $k\in\bit^{p(\secp)}$.
    \item Let $C_{\secp,p}[m]\subseteq \bit^{q(\secp) }$ be a family such that for all $c_m\in C_{\secp,p}[m]$, there exists a circuit $C[m]\in\cC_{\secp,p}[m]$ such that
    \begin{align}
        U_{3p(\secp),p(\secp)}(\ket{\psi}\otimes \ket{c_m})=C[m]\ket{\psi}\otimes\ket{c_m}.
    \end{align}
    \item Let $\Sigma_{\RE}\seteq \RE.(\Enc,\Dec)$ be a decomposable quantum randomized encoding.
    Given quantum circuit $C$ and $n_1$-length quantum input and $n_2$-length classical input $\mathbf{q}$ and $x$,
    the encoding $\widehat{C}(\mathbf{q},x)$ can be written
    \begin{align}
        (\widehat{C}_{\mathsf{off}},
        \widehat{C}_{1},\cdots,\widehat{C}_{n_1+n_2})\la \widehat{C}(\mathbf{q},x,r,e),
    \end{align}
    where $r$ is uniformly ransom string and $e$ is some quantum state.
    From decomposability, $\widehat{C}_{\mathsf{off}}$ acts only on $r$ and $e$.
    Moreover, 
    each $\widehat{C_i}(x_i,r_i)$ and $\widehat{C_i}(\mathbf{q}_i,r,e)$ can be computed separately, and $\widehat{C_i}(x_i,r)$ is classical string for $i\in\{n_1+1,\cdots ,n_1+n_2\}$.
    For any quantum circuit $C$, we write $\lab[i,x_i]= \widehat{C_i}(x_i,r_i)$ and $\lab[i,\mathbf{q}_i]=\widehat{C_i}(\mathbf{q}_i,r,e)$. 
\end{itemize}
\paragraph{Construction.}
We give a construction of one-time unclonable secret-key encryption  $\Sigma\seteq(\keygen,\Enc,\Dec)$ with $n(\secp)$-length plaintexts by using decomposable quantum randomized encoding.
In the construction, we only use decomposable quantum randomized encoding.
The construction is secure as long as the underlying decomposable quantum randomized encoding is secure and there exists one-time unclonable secret-key encryption.
\begin{description}
    \item[$\keygen(1^\secp)$:]$ $
    \begin{itemize}
        \item Sample $x\la\bit^{p(\secp)}$.
        \item Sample $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Output $\sk\seteq \left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$.
    \end{itemize}
    \item[$\Enc(1^\secp,\sk,m)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$.
        \item Let $c_m\in C_{\secp,p}[m]$.
        \item Compute $\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}$.
        \item Compute 
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[p(\secp)]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,b]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,c_m[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item Sample $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Compute $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp),x[i]]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]+\lab[i+p(\secp),x[i]+1]$ for all $i\in[p(\secp)]$.
        \item Output 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,0]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,b]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
    \end{itemize}
    \item[$\Dec(1^\secp,\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$
        and
        \begin{align}    
        \ct=\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,b]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},b\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
        \item Compute $ \lab[i+p(\secp),x[i]\seteq\Lab.\ct[i+p(\secp),x[i]]+R[i]]$ for all $i\in[p(\secp)]$.
        \item Compute 
        \begin{align}
            \RE.\Dec\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}},
            \begin{array}{ll}
                &  \{\lab[i,0]\}_{i\in[p(\secp)]},
        \{\lab[i,x[i]]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\}} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,c_m[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
            \end{array}
            \right)
        \end{align}
        and outputs its output.
    \end{itemize}
\end{description}
\begin{lemma}\label{lem:extend_eff}
    $\Sigma$ satisfies efficiency if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding.
\end{lemma}
\begin{lemma}\label{lem:extend_cor}
    $\Sigma$ satisfies correctness if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding.
\end{lemma}
\begin{lemma}\label{lem:expand_sec}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption with single-bit plaintexts,
    $\Sigma$ satisfies one-time IND-CPA security for some polynomial $p$.
\end{lemma}

\begin{lemma}\label{thm:expnad_unc}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption with single-bit plaintexts,
    $\Sigma$ satisfies one-time unclonable IND-CPA security for some polynomial $p$.  
\end{lemma}
\cref{lem:extend_eff} straightforwardly follows.
\cref{lem:extend_cor} follows because for any $c_m\in C_{\secp,p}[m]$ there exists $C[m]\subseteq \cC_{\secp,p}[m]$ such that
\begin{align}
    U_{3p(\secp),p(\secp)}(\ket{\psi}\otimes \ket{c_m})=C[m](\ket{\psi})\otimes \ket{c_m}
\end{align}
for any $\ket{\psi}$ and $C[m]$ satisfies
\begin{align}
    \Pr[m\la C[m](x\otimes  k\otimes 0^{p(\secp)})]=1
\end{align}
for any $x\in\bit^{p(\secp)}$ and $k\in\bit^{p(\secp)}$.

The proof of \cref{lem:expand_sec} is the same as \cref{thm:expnad_unc}, and thus we skip the proof.
\begin{proof}[Proof of \cref{thm:expnad_unc}]
For appropriate polynomial $p$, there is a quantum circuit $D_{m_0,m_1} \in \Dec_{\secp,p}[m_0,m_1]$.
From the property of $U_{3p(\secp),p(\secp)}$, there exists a subset $D_{\secp,p} \subseteq\bit^{q(\secp)}$ such that for all $d_{m_0,m_1} \in D_{\secp,p}[m_0,m_1]$ there exists a quantum circuit $D_{m_0,m_1} \in \Dec_{\secp,p}[m_0,m_1]$
that satisfies
\begin{align}
U_{3p(\secp),p(\secp)}(\ket{\psi} \otimes\ket{d_{m_0,m_1}}) = D_{m_0,m_1} \ket{\psi} \otimes \ket{d_{m_0,m_1}}.
\end{align}
We consider a fixed such $d_{m_0,m_1}$.
We consider a fixed string $c_{m_b}\in C_{\secp,p}[m_b]$.
We describe the sequence of hybrids against the adversary $(\cA, \cB, \cC)$.
\begin{description}
        \item[$\mathsf{Hyb_0}$:] This is the original one-time unclonable IND-CPA security experiment.
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}$
        and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,0]\}_{i\in[p(\secp)]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,c_{m_b}[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp),x[i]]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]+\lab[i+p(\secp),x[i]+1]$ for all $i\in[p(\secp)]$.
        \item The challenger sends 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,0]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,c_{m_b}[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
        to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:]$ $
    \begin{enumerate}        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$. 
        We write $X$ to mean the first $s(\secp)$ bit of $x$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes  $\unc.\ct_b\la\Unc.\Enc(1^\secp,X,b)$, where $\unc.\ct_b$ is the $q(\secp)$-length quantum states.
        For $i\in\{q(\secp)+1,\cdots, p(\secp)\}$, set $\unc.\ct_b[i]\seteq 0$.
        \item The challenger computes $\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}$ and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[p(\secp)]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,d_{m_0,m_1}[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp),x[i]]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]+\lab[i+p(\secp),x[i]+1]$ for all $i\in[p(\secp)]$.
        \item The challenger sends 
        \begin{align}    
        \ct\seteq\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\{\lab[i,d_{m_0,m_1}[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right).
        \end{align}
        to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
\end{description}
\cref{thm:expnad_unc} follows from the following \cref{prop:hyb_0_hyb_1_unc_expand,prop:hyb_1_unc_expand}.
\begin{proposition}\label{prop:hyb_0_hyb_1_unc_expand}
If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding, then
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\leq\negl(\secp).
\end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_1_unc_expand}
    If there exists a one-time unclonable secret-key encryption $\Sigma_{\Unc}$ with single-bit plaintexts, then
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1=1]}\leq \frac{1}{2}+\negl(\secp).
    \end{align}
\end{proposition}
\end{proof}


\begin{proof}[Proof of \cref{prop:hyb_0_hyb_1_unc_expand}]
Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/\secp^K
\end{align}
for all sufficiently large security parameters $\secp\in\N$.
Then, construct a QPT adversary $\widetilde{\cA}$ that breaks the security of $\Sigma_{\RE}$ as follows.
\begin{enumerate}
    \item $\widetilde{\cA}$ samples $b\la\bit$.
    \item $\widetilde{\cA}$ samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$. We write $X$ to mean the first $s(\secp)$ bits of $x$.
    \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
    \item $\widetilde{\cA}$ computes $\unc.\ct_b\la\Unc.\Enc(1^\secp,X,m_b)$, where $\unc.\ct_b$ is the $q$-length quantum state.
    \item $\widetilde{\cA}$ sends $\left(\{U_{3p(\secp),p(\secp)},0^{p(\secp)},x,0^{p(\secp)},c_{m_b}\},  \{ U_{3p(\secp),p(\secp)},\left(\unc.\ct_b,0^{p(\secp)-q(\secp)}\right),x,0^{p(\secp)},d_{m_0,m_1} \} \right)$ to the challenger of $\Sigma_{\mathsf{RE}}$ in \cref{prop:ind_RE}.
    \item The challenger samples $b^*\la\bit$, and does the following.
    \begin{itemize}
        \item If $b^*=0$, then the challenger computes 
        \begin{align}
         \left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[3p(\secp)+q(\secp)]}\right)\la
         \RE.\Enc\left(1^\secp,U_{3p(\secp),p(\secp)},\left(0^{p(\secp)},x,0^{p(\secp)},c_{m_b}\right)\right),  
        \end{align}
         and sends $\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[3p(\secp)+q(\secp)]}\right)$ to $\widetilde{\cA}$.
        % and sends $\left(\widehat{C[m_b]}_{\mathsf{off}}, \{\widehat{C[m_b]}_i(0;r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
        \item If $b^*=1$, then the challenger computes 
        \begin{align}
         \left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[3p(\secp)+q(\secp)]}\right)\la
         \RE.\Enc\left(1^\secp,U_{3p(\secp),p(\secp)},\left(\unc.\ct_b,0^{p(\secp)-q(\secp)},x,0^{p(\secp)},d_{m_0,m_1}\right)\right),  
        \end{align}
        and sends $\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, \{\lab[i]\}_{i\in[3p(\secp)+q(\secp)]}\right)$ to $\widetilde{\cA}$.
        %and sends $\left(\widehat{D}[\unc.\sk,m_0,m_1]_{\mathsf{off}}, \{\widehat{D}[\unc.\sk,m_0,m_1]_i(\unc.\ct_b[i];r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
    \end{itemize}
    %\item $\widetilde{\cA}$ receives $(\widehat{F}_{\mathsf{off}},\{\mathsf{lab}[i]\}_{i\in[s(\secp)+p(\secp)]})$ from the challenger. Here, if $b^*=0$, then $(\widehat{F}_{\mathsf{off}},\{\mathsf{lab}[i]\}_{i\in[s(\secp)+p(\secp)]})=\left(\widehat{C[m_b]}_{\mathsf{off}}, \{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{ \lab[i,0]\}_{i\in \{s(\secp)+1,\cdots,s(\secp)+p(\secp)\}}\right)$. Otherwise, $(\widehat{F}_{\mathsf{off}},\{\lab[i]\}_{i\in[s(\secp)+p(\secp)]})=\left(\widehat{\Unc.\Dec}_{\mathsf{off}}, \{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{\lab[i,\unc.\ct_b[i]]\}_{\{s(\secp)+1,\cdots,s(\secp)+p(\secp)\}}\right)$.
    %\item $\widetilde{\cA}$ computes $\{\lab[i,x[i]+1]\}_{i\in[s(\secp)]}$.
    %\taiga{I think I need to explain why $\widetilde{\cA}$ can do this.}
    \item $\widetilde{\cA}$ samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, computes $\Lab.\ct[i+p(\secp),x[i]]\seteq R[i]+\lab[i+p(\secp)]$ and $\Lab.\ct[i+p(\secp),x[i]+1]\seteq S[i]$ for all $i\in[p(\secp)]$, and runs $\cA$ on 
    \begin{align}    
        \ct\seteq\left(\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}, 
        \begin{array}{ll}
            &  \{\lab[i]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right),
    \end{align}
    and generates $\rho_{\cB,\cC}$.
    \item $\widetilde{\cA}$  sends the corresponding register to $\cB$ and $\cC$, respectively.
    \item $\widetilde{\cA}$ sends $x$ and $\{R[i]\}_{i\in[p(\secp)]}$ to $\cB$ and $\cC$.
    \item $\cB$ and $\cC$ outputs $b_\cB$ and $b_\cC$, respectively.
    \item $\widetilde{\cA}$ outputs $1$ if $b=b_\cB=b_\cC$, and outputs $0$ otherwise.
\end{enumerate}
From the construction of $\widetilde{\cA}$, if $b^*=0$, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_0}$.
Otherwise, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_1}$.
Furthermore, we have 
\begin{align}
U_{3p(\secp),p(\secp)}(0^{p(\secp)},x,0^{p(\secp)},c_b)=U_{3p(\secp),p(\secp)}(\unc.\ct_b,0^{p(\secp)-q(\secp)},x,0^{p(\secp)},d_{m_0,m_1})=m_b.
\end{align}
Therefore, if there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/\secp^K
\end{align}
for all sufficiently large security parameters $\secp\in\N$,
then it contradicts that $\Sigma_{\RE}$ satisfies security from \cref{prop:ind_RE}.    
\end{proof}



\begin{proof}[Proof of \cref{prop:hyb_1_unc_expand}]
    Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $K$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq \frac{1}{2}+1/\secp^K
    \end{align}
    for all sufficiently large security parameters $\secp\in\N$.
    Then, construct a QPT adversary $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$ that breaks the unclonable IND-CPA security of $\Sigma_{\unc}$ as follows.
    \begin{enumerate}        \item The challenger of $\Sigma_{\unc}$ samples $b\la\bit$.
        \item $\widetilde{\cA}$ samples $Y\la\bit^{p(\secp)-s(\secp)}$ and $R[i,\beta]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
        \item $\widetilde{\cA}$ sends $(0,1)$ to the challenger, and receives $\unc.\ct_b$, where $\unc.\ct_b\la \Unc.\Enc(1^\secp,X,b)$ and $X\la\bit^{s(\secp)}$.
        \item $\widetilde{\cA}$ computes $\widehat{U}_{3p(\secp),p(\secp)\mathsf{off}}$ and
        \begin{align}
        \begin{array}{ll}
             &  \{\lab[i,\unc.\ct_b[i]]\}_{i\in[p(\secp)]},\,\,\,\mbox{and}\,\,\,
        \{\lab[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             &  \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},\,\,\,\mbox{and}\,\,\,\{\lab[i,d_{m_0,m_1}[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}.
        \end{array}
        \end{align}
        \item $\widetilde{\cA}$ computes $\Lab.\ct[i+p(\secp),\beta]]\seteq R[i,\beta]+\lab[i+p(\secp),\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ runs $\cA$ on 
        \begin{align}
        \left( \widehat{U}_{3p(\secp),p(\secp)},
        \begin{array}{ll}
             \{\lab[i,\unc.\ct_b[i]]\}_{i\in[p(\secp)]},
        \{\Lab.\ct[i,\beta]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\},\beta\in\bit} \\
             \{\lab[i,0]\}_{i\in \{2p(\secp)+1,\cdots,3p(\secp)\}},
             \{\lab[i,d_{m_0,m_1}[i]]\}_{i\in\{3p(\secp)+1,\cdots,3p(\secp)+q(\secp)\}}
        \end{array}
        \right),
        \end{align}
         obtains $\rho_{\cB,\cC}$, and sends the $\cB$ register and $(Y,\{R[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit})$ to $\cB$ and $\cC$ register and $(Y,\{R[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit})$ to $\cC$.
        \item $\widetilde{\cB}$ (resp. $\widetilde{\cC}$) receives the secret-key $X$ from the challenger of $\Sigma_{\unc}$, sets $x\seteq X||Y$, and sends $(x,\{R[i,x[i]]\}_{i\in[p(\secp)]})$ and the $\cB$ register (resp. $\cC$ register) to $\cB$ (resp. $\cC$). 
        \item The experiment outputs $1$ if $b=b_\cB=b_\cC$ where $b_\cB$ and $b_\cC$ are the output of $\cB$ and $\cC$, respectively.
    \end{enumerate}
From the construction of $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$, it perfectly simulates the challenger of $\mathsf{Hyb_1}$.
Therefore, if there exists some QPT adversaries $(\cA,\cB,\cC)$ and constant $K$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/\secp^K
    \end{align}
     for all sufficiently large security parameters $\secp\in\N$, it contradicts that $\Sigma_{\unc}$ satisfies unclonable IND-CPA security.
\end{proof}
\end{proof}
\fi


\if0
\paragraph{Universal Construction via Decomposable Quantum Randomized Encoding}
Below, we give another universal construction of a one-time unclonable secret-key encryption for $n(\secp)$-bit plaintexts by using decomposable quantum randomized encoding.
Let us introduce some notations.
\paragraph{Notations.}
\begin{itemize}
    \item
    We assume that there exists one-time unclonable secret-key encryption for $n(\secp)$-plaintext spaces.
    Then, from \cref{prop:perfect_unc}, there exists one-time unclonable secret-key encryption with perfect correctness, and the secret key is uniformly randomly sampled.
    Let $\Sigma_\unc\seteq \Unc. (\keygen,\Enc,\Dec)$ be the one-time unclonable secret-key encryption with $n(\secp)$-length plaintext spaces, where it satisfies perfect correctness and the secret key is uniformly randomly sampled.
    \item Let $s$ be a polynomial such that $s(\secp)$ is the length of secret-key that $\Unc.\keygen(1^\secp)$ generates for all security parameters $\secp\in\N$.
    Let $q$ be a polynomial such that $q(\secp)$ is the length of quantum ciphertext that $\Unc.\Enc(1^\secp,\unc.\sk,m)$ generates for all security parameters $\secp\in\N$.
    \item Let $D$ be the quantum circuit that $\Unc.\Dec$ runs. In other words, the $D$ is the circuit that
    takes as input $s(\secp)$-length classical string $X$ and $q(\secp)$-length quantum state $\unc.\ct$ and outputs $m$, where $X\la\bit^{s(\secp)}$ and $\Unc.\ct\la\Unc.\Enc(1^\secp,X,m)$.
    \item 
    We write $\cD_p$ to mean the general quantum circuit takes as input $p(\secp)$ length classical string $x$ and $p(\secp)$ quantum states $\sigma$, and runs the circuit $D$ on the first $s(\secp)$-length of classical string $x$ and the first $q(\secp)$-length $\sigma$, and outputs its output.
    \item 
    \color{red}
    For $m\in\bit^{n(\secp)}$, let $C_{\secp,p}[m]$ be a general quantum circuit that takes as input $p(\secp)$-length classical string and $p(\secp)$-length quantum states $\sigma$, and always outputs $m$. Furthermore, $C_{\secp,p}[m]$ is padded to size $p(\secp)$ so that for appropriate $p$, $\cD_p$ can be implemented by some circuit whose topology is equal to $C[m]_{\secp,p}$ for all security parameters $\secp\in\N$.
    \taiga{I do not want to explain the detail of how to pad the circuit $C_{\secp,p}[m]$ if possible}.
    \color{black}
    \item Let $\Sigma_{\RE}\seteq \RE.(\Enc,\Dec)$ be a decomposable quantum randomized encoding.
    Given quantum circuit $C$ and $n_1$-length classical inputs $x$ and $n_2$-length quantum input  $x$ and $\mathbf{q}$,
    the encoding $\widehat{C}(\mathbf{q},x)$ can be written
    \begin{align}
        (\widehat{C}_{\mathsf{off}},
        \widehat{C}_{1},\cdots,\widehat{C}_{n_1+n_2})\la \widehat{C}(x,\mathbf{q},r,e),
    \end{align}
    where $r$ is uniformly ransom string and $e$ is some quantum state.
    From decomposability, $\widehat{C}_{\mathsf{off}}$ acts only on $r$ and $e$.
    Moreover, 
    each $\widehat{C_i}(x_i,r_i)$ and $\widehat{C_i}(\mathbf{q}_i,r,e)$ can be computed separately, and $\widehat{C_i}(x_i,r)$ is classical string for $i\in[n_1]$.
    For any quantum circuit $C$, we write $\lab[i,x_i]= \widehat{C_i}(x_i,r_i)$ and $\lab[i,\mathbf{q}_i]=\widehat{C_i}(\mathbf{q}_i,r,e)$. 
\end{itemize}

\paragraph{Construction}
We give a construction of one-time unclonable secret-key encryption with $n(\secp)$-bit plaintexts $\Sigma\seteq(\keygen,\Enc,\Dec)$.
\begin{description}
    \item[$\keygen(1^\secp)$:]$ $
    \begin{itemize}
        \item Sample $x\la\bit^{p(\secp)}$.
        \item Sample $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Output $\sk\seteq \left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$.
    \end{itemize}
    \item[$\Enc(1^\secp,\sk,m)$:]$ $
    \begin{itemize}
        \item Compute $\widehat{C_{\secp,p}[m]}_{\mathsf{off}}$.
        \item Compute $\left(\{\lab[i,b]\}_{i\in[p(\secp)],b\in\bit}, \{\lab[i,0]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\}}\right)$.
        \item Sample $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Compute $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i,x[i]]$ and $\Lab.\ct[i,x[i]+1]\seteq S[i]+\lab[i,x[i]+1]$ for all $i\in[p(\secp)]$.
        \item Output $\ct\seteq \left(\widehat{C_{\secp,p}[m]}_{\mathsf{off}},\{\Lab. \ct[i,b]\}_{i\in[p(\secp)],b\in\bit}, \{\lab[i,0]\}_{i\in \{p(\secp)+1,\cdots,2p(\secp)\}}\right)$.
    \end{itemize}
    \item[$\Dec(1^\secp,\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$ and $\ct=\left(\widehat{C_{\secp,p}[m]}_{\mathsf{off}}, \{\Lab.\ct[i,b]\}_{i\in[p(\secp)],b\in\bit},\{\lab[i,0]\}_{i\in \{p(\secp)+1,\cdots 2p(\secp)\}}\right)$.
        \item Compute $ \lab[i,x[i]\seteq\Lab.\ct[i,x[i]]+R[i]$ for all $i\in[p(\secp)]$.
        \item Compute $\RE.\Dec\left(\widehat{C_{\secp,p}[m]}_{\mathsf{off}},\{\lab[i,x[i]]\}_{i\in[p(\secp)]},\{\lab[i,0]\}_{i\in \{p(\secp)+1,\cdots, 2p(\secp)\}}\right)$ and outputs its output.
    \end{itemize}
\end{description}
\begin{lemma}\label{lem:univ_eff_garble}
$\Sigma$ satisfies efficiency if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding.
\end{lemma}

\begin{lemma}\label{lem:univ_cor_garble}
    $\Sigma$ satisfies correctness if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding.
\end{lemma}

\begin{lemma}\label{thm:univ_unc_garble}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption, then $\Sigma$ is one-time unclonable secret-key encryption for some polynomial $p$.
\end{lemma}
\cref{lem:univ_eff_garble,lem:univ_cor_garble} straightforwardly follows.

\begin{proof}[Proof of \cref{thm:univ_unc_garble}]
Assume that $\Sigma\seteq(\keygen,\Enc,\Dec)$ is one-time unclonable secret-key encryption, where it satisfies perfect correctness and the secret-key is uniformly randomly sampled.
For a security parameter $\secp$, let $s(\secp)$ be the length of secret-key that $\Unc.\keygen(1^\secp)$ generates and $q(\secp)$ be the length of quantum ciphertext that $\Unc.\Enc(1^\secp,\unc.\sk,m)$ generates. 
\color{red}
Fix the polynomial $p$ such that $D_p$ can be implemented by some circuit whose topology is equal to $C_{\secp,p}[m]$.
\color{black}
\taiga{Perhaps, I need to explain the detail of topology of $C_{\secp,p}[m]$.}
    
We describe the sequence of hybrids against adversary $(\cA,\cB,\cC)$.
\begin{description}
    \item[$\mathsf{Hyb_0}$:] This is the original one-time unclonable IND-CPA security experiment.
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\widehat{C_{\secp,p}[m]}_{\mathsf{off}}$, $\lab[i,\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$ and $\lab[i,0]$ for all $i\in\{p(\secp)+1,\cdots, 2p(\secp)\}$.
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i,x[i]]$ and $\Lab.\ct[i,x[i]+1]\seteq S[i]+\lab[i,x[i]+1]$ for all $i\in[p(\secp)]$.
        \item The challenger sends $\left(\widehat{C_{\secp,p}[m]}_{\mathsf{off}},\{\Lab.\ct[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit}, \{\lab[i,0]\}_{i\in\{p(\secp)+1,\cdots, 2p(\secp)\}}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:]$ $
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$. 
        We write $X$ to mean the first $s(\secp)$ bit of $x$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes  $\unc.\ct_b\la\Unc.\Enc(1^\secp,X,m_b)$, where $\unc.\ct_b$ is the $q(\secp)$-length quantum states.
        For $i\in\{q(\secp)+1,\cdots, p(\secp)\}$, set $\unc.\ct_b[i]\seteq 0$.
        \item The challenger computes $\widehat{\cD_p}_{\mathsf{off}}$ and $\lab[i,\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$ and $\lab[i,\unc.\ct[i]]$ for all $i\in[p(\secp)]$.
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i,x[i]]$ and $\Lab.\ct[i,x[i]+1]\seteq S[i]+\lab[i,x[i]+1]$ for all $i\in[p(\secp)]$.
        \item The challenger sends $\left(\widehat{\cD_p}_{\mathsf{off}},\{\Lab.\ct[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct[i]\}_{i\in[p(\secp)]}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
\end{description}
\cref{thm:univ_unc_garble} follows from the following \cref{prop:hyb_0_hyb_1_univ_unc_garble,prop:hyb_1_univ_unc_garble}.
\begin{proposition}\label{prop:hyb_0_hyb_1_univ_unc_garble}
    If $\Sigma_\RE$ is decomposable quantum randomized encoding, then
    \begin{align}
        \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\leq \negl(\secp).
    \end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_1_univ_unc_garble}
If there exists one-time secret-key unclonable encryption with $n(\secp)$-bit plaintexts, then
\begin{align}
    \Pr[\mathsf{Hyb_1}]\leq \frac{1}{2}+\negl(\secp).
\end{align}
\end{proposition}
\end{proof}
\begin{proof}[Proof of \cref{prop:hyb_0_hyb_1_univ_unc_garble}]
Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $c$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/\secp^c
\end{align}
for all sufficiently large security parameters $\secp\in\N$.
Then, construct a QPT adversary $\widetilde{\cA}$ that breaks the security of $\Sigma_{\RE}$ as follows.
\begin{enumerate}
    \item $\widetilde{\cA}$ samples $b\la\bit$.
    \item $\widetilde{\cA}$ samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$. We write $X$ to mean the first $s(\secp)$ bits of $x$.
    \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
    \item $\widetilde{\cA}$ computes $\unc.\ct_b\la\Unc.\Enc(1^\secp,X,m_b)$, where $\unc.\ct_b$ is the $q$-length quantum state.
    \item $\widetilde{\cA}$ sends $\left(\{C[m_b],x,0^{p(\secp)}\},  \{ \cD_p, x,\left(\unc.\ct_b,0^{p(\secp)-q(\secp)}\right) \} \right)$ to the challenger of $\Sigma_{\mathsf{RE}}$.
    \item The challenger samples $b^*\la\bit$, and do the following.
    \begin{itemize}
        \item If $b^*=0$, then the challenger computes $\left(\widehat{F}_{\mathsf{off}}, \{\lab[i]\}_{i\in[2p(\secp)]}\right)\la\RE.\Enc(1^\secp,C[m_b],x,0^{p(\secp)})$, and sends $\left(\widehat{F}_{\mathsf{off}}, \{\lab[i]\}_{i\in[2p(\secp)]}\right)$ to $\widetilde{\cA}$.
        % and sends $\left(\widehat{C[m_b]}_{\mathsf{off}}, \{\widehat{C[m_b]}_i(0;r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
        \item If $b^*=1$, then the challenger computes $\left(\widehat{F}_{\mathsf{off}}, \{\lab[i]\}_{i\in[2p(\secp)]}\right)\la\RE.\Enc(1^\secp,\cD_p,x,\unc.\ct_b,0^{p(\secp)-q(\secp)})$. 
        %and sends $\left(\widehat{D}[\unc.\sk,m_0,m_1]_{\mathsf{off}}, \{\widehat{D}[\unc.\sk,m_0,m_1]_i(\unc.\ct_b[i];r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
    \end{itemize}
    %\item $\widetilde{\cA}$ receives $(\widehat{F}_{\mathsf{off}},\{\mathsf{lab}[i]\}_{i\in[s(\secp)+p(\secp)]})$ from the challenger. Here, if $b^*=0$, then $(\widehat{F}_{\mathsf{off}},\{\mathsf{lab}[i]\}_{i\in[s(\secp)+p(\secp)]})=\left(\widehat{C[m_b]}_{\mathsf{off}}, \{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{ \lab[i,0]\}_{i\in \{s(\secp)+1,\cdots,s(\secp)+p(\secp)\}}\right)$. Otherwise, $(\widehat{F}_{\mathsf{off}},\{\lab[i]\}_{i\in[s(\secp)+p(\secp)]})=\left(\widehat{\Unc.\Dec}_{\mathsf{off}}, \{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{\lab[i,\unc.\ct_b[i]]\}_{\{s(\secp)+1,\cdots,s(\secp)+p(\secp)\}}\right)$.
    %\item $\widetilde{\cA}$ computes $\{\lab[i,x[i]+1]\}_{i\in[s(\secp)]}$.
    %\taiga{I think I need to explain why $\widetilde{\cA}$ can do this.}
    \item $\widetilde{\cA}$ samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, computes $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i]$ and $\Lab.\ct[i,x[i]+1]\seteq S[i]$ for all $i\in[p(\secp)]$, and sends $(\widehat{F}_{\mathsf{off}},\{\Lab.\ct[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit},\{\lab[i]\}_{i\in\{p(\secp)+1,\cdots,2p(\secp)\}} )$ to $\cA$.
    \item $\cA$ generates $\rho_{\cB,\cC}$ and sends the corresponding register to $\cB$ and $\cC$
    \item $\widetilde{\cA}$ sends $x$ and $\{R[i]\}_{i\in[p(\secp)]}$ to $\cB$ and $\cC$.
    \item $\widetilde{\cA}$ outputs $1$ if $b=b_\cB=b_\cC$, and outputs $0$ otherwise.
\end{enumerate}
From the construction of $\widetilde{\cA}$, if $b^*=0$, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_0}$.
Otherwise, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_1}$.
Furthermore, $C_{\secp,p}[m](x,0^{p(\secp)})=\cD_p(x,\unc.\ct_b,0^{p(\secp)-q(\secp)})$ and the topology of $C_{\secp,p}[m]_{\secp,p}$ and $\cD_p$ are equivalent.
Therefore, if there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $c$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/\secp^c
\end{align}
for all sufficiently large security parameters $\secp\in\N$,
then it contradicts that $\Sigma_{\RE}$ satisfies security from \cref{prop:ind_RE}.
\end{proof}

\begin{proof}[Proof of \cref{prop:hyb_1_univ_unc_garble}]
    Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $c$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/\secp^c
    \end{align}
    for all sufficiently large security parameters $\secp\in\N$.
    Then, construct a QPT adversary $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$ that breaks the one-time unclonable IND-CPA security of $\Sigma_\unc$ as follows.
    \begin{enumerate}
        \item The challenger of $\Sigma_{\unc}$ samples $b\la\bit$.
        \item $\widetilde{\cA}$ samples $Y\la\bit^{p(\secp)-s(\secp)}$ and $R[i,\beta]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
        \item $\widetilde{\cA}$ sends $( m_0,m_1)$ to the challenger, and receives $\unc.\ct_b$.
        \item $\widetilde{\cA}$ computes $\left(\widehat{\cD_p}_{\mathsf{off}}, \{\lab[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct_b[i]] \}_{i\in\{p(\secp)+1,\cdots,2p(\secp)\}}\right)$.
        \item $\widetilde{\cA}$ computes $\Lab.\ct[i,\beta]]\seteq R[i,\beta]+\lab[i,\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ runs $\cA$ on $\left( \widehat{\cD_p}_{\mathsf{off}}, \{\Lab.\ct[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct_b[i]] \}_{i\in\{p(\secp)+1,\cdots,2p(\secp)\}}\right)$, obtains $\rho_{\cB,\cC}$, and sends the $\cB$ register and $(Y,\{R[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit})$ to $\cB$ and $\cC$ register and $(Y,\{R[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit})$ to $\cC$.
        \item $\widetilde{\cB}$ (resp. $\widetilde{\cC}$) receives the secret-key $X$ from the challenger of $\Sigma_{\unc}$, sets $x\seteq X||Y$, and sends $(x,\{R[i,x[i]]\}_{i\in[p(\secp)]})$ and the $\cB$ register (resp. $\cC$ register) to $\cB$ (resp. $\cC$). 
        \item The experiment outputs $1$ if $b=b_\cB=b_\cC$ where $b_\cB$ and $b_\cC$ are the output of $\cB$ and $\cC$, respectively.
    \end{enumerate}
    From the construction of $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$, the adversary perfectly simulates the challenger of $\mathsf{Hyb_1}$. Therefore, if there exists a QPT adversary $(\cA,\cB,\cC)$ and some constant $c$ such that 
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/\secp^c
    \end{align}
     for all sufficiently large security parameters $\secp\in\N$, it contradicts $\Sigma_{\unc}$ satisfies unclonable IND-CPA security.
\end{proof}



\subsection{Expanding Plaintext Space}
In this section, we prove the following \cref{thm:unclone_multi_space}.
\begin{theorem}\label{thm:unclone_multi_space}
    If there exists a one-time unclonable secret-key encryption with single-bit plaintext spaces and decomposable quantum randomized encoding, then there exists a one-time unclonable secret-key encryption with $n(\secp)$-length plaintext spaces for all polynomial $n$.
\end{theorem}

\begin{corollary}\label{cor:unclone_expnasion}
    If there exists unclonable secret-key encryption with single-bit plaintext spaces, then there exists unclonable secret-key encryption with $n(\secp)$-length plaintext spaces for all polynomial $n$.
\end{corollary}
\begin{corollary}\label{cor:pub_unclone_expansion}
    If unclonable public-key encryption with single-bit plaintext spaces, then there exists unclonable public-key encryption with $n(\secp)$-length plaintext spaces for all polynomial $n$.
\end{corollary}
\begin{proof}[Proof of \cref{cor:pub_unclone_expansion}]
    We give a rough sketch of the proof of \cref{cor:pub_unclone_expansion}. Note that, in the same way, we can prove \cref{cor:unclone_expnasion}.
    If there exists unclonable public-key encryption with single-bit plaintext spaces, then there exists public-key encryption with quantum ciphertext and one-time unclonable secret-key encryption with single-bit plaintext spaces.
    The existence of public-key encryption with quantum ciphertext implies the existence of decomposable quantum randomized encoding.
    Therefore, by combining decomposable quantum randomized encoding and one-time unclonable secret-key encryption with single-bit plaintext spaces, we have one-time unclonable secret-key encryption with $n(\secp)$-plaintext spaces for all polynomial $n$.

    Furthermore, the existence of public-key encryption with quantum ciphertext implies the existence of receiver non-committing encryption with quantum ciphertext.
    By combining the receiver non-committing encryption with quantum ciphertext and one-time unclonable secret-key encryption with $n(\secp)$-plaintext spaces, we obtain unclonable public-key encryption with $n(\secp)$-plaintext spaces.
    \taiga{Here, we need to check the details. Especially, I am not so confident that PKE with q-Cipher implies the decomposable quantum randomized encoding, where the labels are classical if the inputs are classical strings. (We need the classical label or classical off-line part for our purpose.)}
    \taiga{If time remains, I think that we should include the details of the proof of corollary.}
\end{proof}

\begin{proof}[Proof of \cref{thm:unclone_multi_space}]
First, let us describe notations.
\paragraph{Notations.}
\begin{itemize}
    \item Let $\Sigma_\unc\seteq \Unc. (\keygen,\Enc,\Dec)$ be one-time unclonable secret-key encryption with single-bit plaintext spaces, where it satisfies perfect correctness and the secret key is uniformly randomly sampled.
    Note that, from \cref{prop:perfect_unc}, such one-time unclonable secret-key encryption exists if there exists plain one-time unclonable secret-key encryption exists.
    \item  For a security parameter $\secp$, we assume that $s(\secp)$ be the length of secret-key that $\Unc.\keygen(1^\secp)$ generates and $q(\secp)$ be the length of quantum ciphertext that $\Unc.\Enc(1^\secp,\unc.\sk,m)$ generates. 
    \item Let $D$ be the quantum circuit that $\Unc.\Dec$ runs. In other words, the $D$ is the circuit that
    takes as input $s(\secp)$-length classical string $x$ and $q(\secp)$-length quantum state $\unc.\ct$ and outputs $b\in\bit$, where $x\la\bit^{s(\secp)}$ and $\Unc.\ct\la\Unc.\Enc(1^\secp,x,m)$.
    \item 
    For $m_0,m_1\in\bit^{n(\secp)}$, we write $\cD_p[m_0,m_1]$ to mean the general quantum circuit takes as input $p(\secp)$ length classical string $x$ and $p(\secp)$ quantum states $\sigma$, and runs the circuit $D$ on the first $s(\secp)$-length of classical string $x$ and the first $q(\secp)$-length $\sigma$, obtains $b\in\bit$, and outputs $m_b$.
    \item 
    \color{red}
    For $m\in\bit^{n(\secp)}$, let $C_{\secp,p}[m]$ be a general quantum circuit that takes as input $p(\secp)$-length classical string and $p(\secp)$-length quantum states $\sigma$, and always outputs $m$. Furthermore, $C_{\secp,p}[m]$ is padded to size $p(\secp)$ so that for appropriate $p$, $\cD_p$ can be implemented by some circuit whose topology is equal to $C_{\secp,p}[m]$.
    \taiga{I do not want to explain the detail of how to pad the circuit $C[m]_{\secp,p}$ if possible}.
    \color{black}
    \item Let $\Sigma_{\RE}\seteq \RE.(\Enc,\Dec)$ be a decomposable quantum randomized encoding.
    For some quantum circuit $C$ and input $x$, we write $\widehat{C}_{\mathsf{off}}$ to mean the off-line part of $\widehat{C}(x;r)$, and write $\lab[i,x[i]]$ to mean the online encoding of $\widehat{C}(x;r)$, where $\widehat{C}(x;r)\la\RE.\Enc(1^\secp,C,x)$.
    Let $\ell(\secp)$ be the length of on-line part of $\lab[i,x[i]]$, where $\left(\widehat{C[m]}_{\mathsf{off}},\{\lab[i,x[i]]\}_{i\in[2p(\secp)]} \right)\la \RE.\Enc(C[m],x)$.
\end{itemize}

\paragraph{Construction.}
We give a construction of one-time unclonable secret-key encryption  $\Sigma\seteq(\keygen,\Enc,\Dec)$ with $n(\secp)$-length plaintext spaces.
\begin{description}
    \item[$\keygen(1^\secp)$:]$ $
    \begin{itemize}
        \item Sample $x\la\bit^{p(\secp)}$.
        \item Sample $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Output $\sk\seteq (x,\{R[i]\}_{i\in[p(\secp)]})$.
    \end{itemize}
    \item[$\Enc(1^\secp,\sk,m)$:]$ $
    \begin{itemize}
        \item Compute $\widehat{C_{\secp,p}[m]}_{\mathsf{off}}$.
        \item Compute $\left(\{\lab[i,b]\}_{i\in[p(\secp)],b\in\bit},\{\lab[i,0]\}_{i\in\{p(\secp)+1,\cdots,2p(\secp)\}}\right)$.
        \item Sample $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Compute $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i,x[i]]$ and $\Lab.\ct[i,x[i]+1]\seteq S[i]+\lab.\ct[i,x[i]+1]$ for all $i\in [p(\secp)]$.
        \item Output $\ct\seteq \left(\widehat{C_{\secp,p}[m]}_{\mathsf{off}}, \{\Lab.\ct[i,b]\}_{i\in[p(\secp)],b\in\bit},\{\lab[i,0]\}_{i\in\{p(\secp)+1,\cdots,2p(\secp)\}}\right)$.
    \end{itemize}
    \item[$\Dec(1^\secp,\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$ and $\ct=\left(\widehat{C_{\secp,p}[m]}_{\mathsf{off}}, \{\Lab.\ct[i,b]\}_{i\in[p(\secp)],b\in\bit},\{\lab[i,0]\}_{i\in\{p(\secp)+1,\cdots,2p(\secp)\}}\right)$.
        \item Compute $\lab[i,x[i]]\seteq \Lab.\ct[i,x[i]]+R[i]$ for all $i\in[p(\secp)]$.
        \item Compute $\RE.\Dec(1^\secp,\widehat{C_{\secp,p}[m]}_{\mathsf{off}},\{\lab[i,x[i]]\}_{i\in[p(\secp)]},\{\lab[i,0]\}_{i\in[p(\secp)]} )$ and outputs its output.
    \end{itemize}
\end{description}
\begin{theorem}\label{thm:expnad_unc}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption with single-bit plaintext spaces,
    $\Sigma$ is one-time unclonable secret-key encryption with $n(\secp)$-length plaintext spaces for some polynomial $p$.  
\end{theorem}

\begin{proof}[Proof of \cref{thm:expnad_unc}]
Assume that $\Sigma\seteq(\keygen,\Enc,\Dec)$ is one-time unclonable secret-key encryption with single-bit plaintext spaces, where it satisfies perfect correctness and the secret-key is uniformly randomly sampled. 
For a security parameter $\secp$, let $s(\secp)$ be the length of secret-key that $\Unc.\keygen(1^\secp)$ generates and $q(\secp)$ be the length of quantum ciphertext that $\Unc.\Enc(1^\secp,\unc.\sk,m)$ generates. Fix the polynomial $p$ such that $\cD_p[m_0,m_1]$ can be implemented by some circuit whose topology is equal to $C_{\secp,p}[m]$.


We describe the sequence of hybrids against adversary $(\cA,\cB,\cC)$.
\begin{description}
        \item[$\mathsf{Hyb_0}$:] This is the original one-time unclonable IND-CPA security experiment.
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\widehat{C_{\secp,p}[m_b]}_{\mathsf{off}}$, $\lab[i,\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$ and $\lab[i,0]$ for all $i\in\{p(\secp)+1,\cdots, 2p(\secp)\}$.
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i,x[i]]$ and $\Lab.\ct[i,x[i]+1]\seteq S[i]+\lab[i,x[i]+1]$ for all $i\in[p(\secp)]$.
        \item The challenger sends $\left(\widehat{C_{\secp,p}[m_b]}_{\mathsf{off}},\{\Lab.\ct[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit}, \{\lab[i,0]\}_{i\in\{p(\secp)+1,\cdots, 2p(\secp)\}}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:]$ $
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        We write $X$ to mean the first $s(\secp)$-bit of $x$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes  $\unc.\ct_b\la\Unc.\Enc(1^\secp,X,b)$, where $\unc.\ct_b$ is $q(\secp)$-length. For $i\in\{q(\secp)+1,\cdots,p(\secp)\}$, set $\unc.\ct_b[i]\seteq 0$.
        \item The challenger computes $\widehat{\cD_p}[m_0,m_1]_{\mathsf{off}}$ and $\lab[i,\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$ and $\lab[i,\unc.\ct_b[i]]$ for all $i\in[p(\secp)]$.
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i,x[i]]$ and $\Lab.\ct[i,x[i]+1]\seteq S[i]+\lab[i,x[i]+1]$ for all $i\in[p(\secp)]$.
        \item The challenger sends $\left(\widehat{\cD_p}[m_0,m_1]_{\mathsf{off}},\{\Lab.\ct[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct[i]]\}_{i\in[p(\secp)]}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
\end{description}
\cref{thm:expnad_unc} follows from the following \cref{prop:hyb_0_hyb_1_unc_expand,prop:hyb_1_unc_expand}.
\begin{proposition}\label{prop:hyb_0_hyb_1_unc_expand}
If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding, then
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\leq\negl(\secp).
\end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_1_unc_expand}
    If there exists a one-time unclonable secret-key encryption $\Sigma_{\Unc}$ with single-bit plaintext spaces, then
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1=1]}\leq \frac{1}{2}+\negl(\secp).
    \end{align}
\end{proposition}
\end{proof}

Because the proof of \cref{prop:hyb_0_hyb_1_unc_expand} is almost the same as \cref{prop:hyb_0_hyb_1_univ_unc_garble}, and thus we skip the proof.

\begin{proof}[Proof of \cref{prop:hyb_1_unc_expand}]
    Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ and constant $c$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq \frac{1}{2}+1/\secp^c
    \end{align}
    for all sufficiently large security parameters $\secp\in\N$.
    Then, construct a QPT adversary $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$ that breaks the unclonable IND-CPA security of $\Sigma_{\unc}$ as follows.
    \begin{enumerate}
        \item The challenger of $\Sigma_{\unc}$ samples $b\la\bit$.
        \item $\widetilde{\cA}$ samples $Y\la\bit^{p(\secp)-s(\secp)}$ and $R[i,\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from $\cA$.
        \item $\widetilde{\cA}$ sends $(0,1)$ to the challenger of $\Sigma_\unc$, and receives the $q(\secp)$-length quantum state $\unc.\ct_b$.
        $\widetilde{\cA}$ sets $\unc.\ct_b[i]\seteq 0$ for all $i\in\{q(\secp)+1,\cdots,p(\secp)\}$.
        \item $\widetilde{\cA}$ computes $\widehat{\cD_p}[m_0,m_1]_{\mathsf{off}}$ and $\lab[i,\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$ and $\lab[i,\unc.\ct_b[i]]$ for all $i\in[p(\secp)]$.
        \item $\widetilde{\cA}$ computes $\Lab.\ct[i,\beta]\seteq R[i,\beta]+\lab[i,\beta]$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ runs $\cA$ on $\left(\widehat{\cD_p}[m_0,m_1]_{\mathsf{off}},\{\Lab.\ct[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct_b[i]]\}_{i\in\{p(\secp)+1,\cdots,2p(\secp)\}} \right)$, obtains $\rho_{\cB,\cC}$, and sends the $\cB$ register and $\{R[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit}$ (resp. register $\cC$ and $\{R[i,\beta]\}_{i\in[p(\secp)],\beta\in\bit}$) to $\widetilde{\cB}$ (resp. $\widetilde{\cC}$).
        \item $\widetilde{\cB}$ (resp. $\widetilde{\cC}$) receives the $s(\secp)$-length secret key $X$ from the challenger of $\Sigma_\unc$, sets $x\seteq X||Y$, and sends $(x,\{R[i,x[i]]\}_{i\in[p(\secp)]})$ and the $\cB$ register (resp. $\cC$ register) to $\cB$ (resp. $\cC$).
        \item The experiment outputs $1$ if $b=b_\cB=b_\cC$, and $0$ otherwise, where $b_\cB$ and $b_\cC$ are the outputs of $\cB$ and $\cC$, respectively.
    \end{enumerate}
From the construction of $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$, it perfectly simulates the challenger of $\mathsf{Hyb_1}$.
Therefore, if there exists some QPT adversaries $(\cA,\cB,\cC)$ and constant $c$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/\secp^c
    \end{align}
     for all sufficiently large security parameters $\secp\in\N$, it contradicts that $\Sigma_{\unc}$ satisfies unclonable IND-CPA security.
\end{proof}
\end{proof}
\fi

==> Old_Univ_RE.tex <==
\paragraph{Universal Construction via Decomposable Quantum Randomized Encoding}
\taiga{I skipped many parts of the explanation below.}
We give an explicit construction of one-time unclonable secret-key encryption using decomposable quantum randomized encoding $\Sigma_\RE$, where the security relies on the existence of one-time unclonable secret-key encryption and the security of $\Sigma_\RE$. 
\paragraph{Notations.}
\begin{itemize}
    \item Let $\Sigma_\Unc\seteq \Unc(\keygen,\Enc,\Dec)$ be a one-time unclonable secret-key encryption.
    For a security parameter $\secp$, let $s(\secp)$ be the length of secret-key that $\Unc.\keygen(1^\secp)$ generates and $q(\secp)$ be the length of quantum ciphertext that $\Unc.\Enc(1^\secp,\unc.\sk,m)$ generates.
    Without loss of generality, we can assume that the secret key $\sk\la\Unc.\keygen(1^\secp)$ is uniformly sampled from $\bit^{s(\secp)}$.
    \taiga{I think I need the explanation in the sentence above.}
    \item Let $C[m]$ be a general quantum circuit that takes as input $\left(s(\secp)+q(\secp)\right)$-length quantum state, and always outputs $m$.
    Furthermore, the topology of $C[m]$ is equal to that of $\Unc.\Dec$.
    \item Let $\Sigma_{\RE}\seteq \RE.(\Enc,\Dec)$ be a decomposable quantum randomized encoding.
    For some quantum circuit $C$ and input $x$, we write $\widehat{C}_{\mathsf{off}}$ to mean the off-line part of $\widehat{C}(x;r)$, and write $\lab[i,x[i]](r)$ to mean the online encoding of $\widehat{C}(x;r)$, where $\widehat{C}(x;r)\la\RE.\Enc(1^\secp,C,x)$.
    Let $\ell(\secp)$ be the length of on-line part of $\lab[i,x[i]]$, where $\left(\widehat{C[m]}_{\mathsf{off}}(r),\{\lab[i,x[i]](r)\}_{i\in[s(\secp)+q(\secp)]} \right)\la \RE.\Enc(C[m],x)$.
\end{itemize}

\paragraph{Construction}
We give a construction of one-time unclonable secret-key encryption with $n(\secp)$-plaintext space $\Sigma\seteq(\keygen,\Enc,\Dec)$.
\begin{description}
    \item[$\keygen(1^\secp)$:]$ $
    \begin{itemize}
        \item Sample $x\la\bit^{s(\secp)}$.
        \item Sample $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
        \item Output $\sk\seteq \left(x,\{R[i]\}_{i\in[s(\secp)]}\right)$.
    \end{itemize}
    \item[$\Enc(\sk,m)$:]$ $
    \begin{itemize}
        \item Compute $\widehat{C[m]}_{\mathsf{off}}(r)$.
        \item Compute $\left(\{\lab[i,b](r)\}_{i\in[s(\secp)],b\in\bit}, \{\lab[i,0](r)\}_{i\in \{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$.
        \item Sample $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
        \item Compute $\Lab.\ct[i,x[i]](r)\seteq R[i]+\lab[i,x[i]](r)$ and $\Lab.\ct[i,x[i]+1](r)\seteq S[i]+\lab[i,x[i]+1](r)$ for all $i\in[s(\secp)]$.
        \item Output $\ct\seteq \left(\widehat{C[m]}_{\mathsf{off}}(r),\{\Lab. \ct[i,b](r)\}_{i\in[s(\secp)],b\in\bit}, \{\lab[i,0](r)\}_{i\in \{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$.
    \end{itemize}
    \item[$\Dec(\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[s(\secp)]}\right)$ and $\ct=\left(\widehat{C[m]}_{\mathsf{off}}(r), \{\Lab.\ct[i,b](r)\}_{i\in[s(\secp)],b\in\bit},\{\lab[i,0](r)\}_{i\in \{s(\secp)+1,\cdots s(\secp)+q(\secp)\}}\right)$.
        \item Compute $ \lab[i,x[i](r)\seteq\Lab.\ct[i,x[i]](r)+R[i]$ for all $i\in[s(\secp)]$.
        \item Compute $\Dec\left(\widehat{C[m]}_{\mathsf{off}}(r),\{\lab[i,x[i]](r)\}_{i\in[s(\secp)]},\{\lab[i,0](r)\}_{i\in \{s(\secp)+1,\cdots, s(\secp)+q(\secp)\}}\right)$ and outputs its output.
    \end{itemize}
\end{description}
\begin{theorem}\label{thm:univ_unc_garble}
    If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption, then $\Sigma$ is one-time unclonable secret-key encryption for some polynomial $s$ and $q$.
\end{theorem}

\begin{proof}[Proof of \cref{thm:univ_unc_garble}]
We describe the sequence of hybrids against adversary $(\cA,\cB,\cC)$.
\begin{description}
    \item[$\mathsf{Hyb_0}$:] This is the original one-time unclonable IND-CPA security experiment.
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{s(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\widehat{C[m]}_{\mathsf{off}}(r)$, $\lab[i,\beta](r)$ for all $i\in[s(\secp)]$ and $\beta\in\bit$ and $\lab[i,0](r)$ for all $i\in\{s(\secp)+1,\cdots, s(\secp)+q(\secp)\}$.
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$, and computes $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i,x[i]]$ and $\Lab.\ct[i,x[i]+1]\seteq S[i]+\lab[i,x[i]+1]$ for all $i\in[s(\secp)]$.
        \item The challenger sends $\left(\widehat{C[m]}_{\mathsf{off}}(r),\{\Lab.\ct[i,\beta]\}_{i\in[s(\secp)],\beta\in\bit}, \{\lab[i,0](r)\}_{i\in\{s(\secp)+1,\cdots, s(\secp)+q(\secp)\}}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[s(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:]$ $
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{s(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes  $\unc.\ct_b\la\Unc.\Enc(1^\secp,x,m_b)$.
        \item The challenger computes $\widehat{\Unc.\Dec}_{\mathsf{off}}(r)$ and $\lab[i,\beta]$ for all $i\in[s(\secp)]$ and $\beta\in\bit$ and $\lab[i,\unc.\ct[i]](r)$ for all $i\in[q(\secp)]$.
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$, and computes $\Lab.\ct[i,x[i]](r)\seteq R[i]+\lab[i,x[i]](r)$ and $\Lab.\ct[i,x[i]+1](r)\seteq S[i]+\lab[i,x[i]+1](r)$ for all $i\in[s(\secp)]$.
        \item The challenger sends $\left(\widehat{\Unc.\Dec}_{\mathsf{off}}(r),\{\Lab.\ct[i,\beta](r)\}_{i\in[s(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct[i](r)\}_{i\in[q(\secp)]}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[s(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
\end{description}
\cref{thm:univ_unc_garble} follows from the following \cref{prop:hyb_0_hyb_1_univ_unc_garble,prop:hyb_1_univ_unc_garble}.
\begin{proposition}\label{prop:hyb_0_hyb_1_univ_unc_garble}
    If $\Sigma_\RE$ is decomposable quantum randomized encoding, then
    \begin{align}
        \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\leq \negl(\secp).
    \end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_1_univ_unc_garble}
If there exists one-time secret-key unclonable encryption, then
\begin{align}
    \Pr[\mathsf{Hyb_1}]\leq \frac{1}{2}+\negl(\secp).
\end{align}
\end{proposition}
\end{proof}
\begin{proof}[Proof of \cref{prop:hyb_0_hyb_1_univ_unc_garble}]
Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/p(\secp)
\end{align}
for some polynomial $p$.
Then, construct a QPT adversary $\widetilde{\cA}$ that breaks the security of $\Sigma_{\RE}$ as follows.
\begin{enumerate}
    \item $\widetilde{\cA}$ samples $b\la\bit$.
    \item $\widetilde{\cA}$ samples $x\la\unc.\keygen(1^\secp)$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
    \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
    \item $\widetilde{\cA}$ computes $\unc.\ct_b\la\Unc.\Enc(1^\secp,x,m_b)$.
    \item $\widetilde{\cA}$ sends $\left(\{C[m_b],x,0^{q(\secp)}\},  \{ \Unc.\Dec, x,\unc.\ct_b \} \right)$ to the challenger of $\Sigma_{\mathsf{RE}}$.
    \item The challenger samples $b^*\la\bit$, and do the following.
    \begin{itemize}
        \item If $b^*=0$, then the challenger computes $\left(\widehat{F}_{\mathsf{off}}(r), \{\lab[i](r)\}_{i\in[s(\secp)+q(\secp)]}\right)\la\RE.\Enc(1^\secp,C[m_b],x,0^{q(\secp)})$, and sends $\left(\widehat{F}_{\mathsf{off}}(r), \{\lab[i](r)\}_{i\in[s(\secp)+q(\secp)]}\right)$ to $\widetilde{\cA}$.
        % and sends $\left(\widehat{C[m_b]}_{\mathsf{off}}(r), \{\widehat{C[m_b]}_i(0;r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
        \item If $b^*=1$, then the challenger computes $\left(\widehat{F}_{\mathsf{off}}(r), \{\lab[i](r)\}_{i\in[s(\secp)+q(\secp)]}\right)\la\RE.\Enc(1^\secp,\Unc.\Dec,x,\unc.\ct_b)$. 
        %and sends $\left(\widehat{D}[\unc.\sk,m_0,m_1]_{\mathsf{off}}(r), \{\widehat{D}[\unc.\sk,m_0,m_1]_i(\unc.\ct_b[i];r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
    \end{itemize}
    %\item $\widetilde{\cA}$ receives $(\widehat{F}_{\mathsf{off}}(r),\{\mathsf{lab}[i](r)\}_{i\in[s(\secp)+q(\secp)]})$ from the challenger. Here, if $b^*=0$, then $(\widehat{F}_{\mathsf{off}}(r),\{\mathsf{lab}[i](r)\}_{i\in[s(\secp)+q(\secp)]})=\left(\widehat{C[m_b]}_{\mathsf{off}}(r), \{\lab[i,x[i]](r)\}_{i\in[s(\secp)]},\{ \lab[i,0](r)\}_{i\in \{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$. Otherwise, $(\widehat{F}_{\mathsf{off}}(r),\{\lab[i](r)\}_{i\in[s(\secp)+q(\secp)]})=\left(\widehat{\Unc.\Dec}_{\mathsf{off}}(r), \{\lab[i,x[i]](r)\}_{i\in[s(\secp)]},\{\lab[i,\unc.\ct_b[i]](r)\}_{\{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$.
    %\item $\widetilde{\cA}$ computes $\{\lab[i,x[i]+1](r)\}_{i\in[s(\secp)]}$.
    %\taiga{I think I need to explain why $\widetilde{\cA}$ can do this.}
    \item $\widetilde{\cA}$ samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$, computes $\Lab.\ct[i,x[i]](r)\seteq R[i]+\lab[i](r)$ and $\Lab.\ct[i,x[i]+1](r)\seteq S[i]$ for all $i\in[s(\secp)]$, and sends $(\widehat{F}_{\mathsf{off}}(r),\{\Lab.\ct[i,\beta]\}_{i\in[s(\secp)],\beta\in\bit},\{\lab[i]\}_{i\in\{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}} )$ to $\cA$.
    \item $\cA$ generates $\rho_{\cB,\cC}$ and sends the corresponding register to $\cB$ and $\cC$
    \item $\widetilde{\cA}$ sends $x$ and $\{R[i]\}_{i\in[s(\secp)]}$ to $\cB$ and $\cC$.
    \item $\widetilde{\cA}$ outputs $1$ if $b=b_\cB=b_\cC$, and outputs $0$ otherwise.
\end{enumerate}
From the construction of $\widetilde{\cA}$, if $b^*=0$, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_0}$.
Otherwise, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_1}$.
Furthermore, we have $C[m](x,0^{q(\secp)})=\Unc.\Dec(x,\unc.\ct_b)$.
Therefore, if there exists a QPT adversary $(\cA,\cB,\cC)$ and polynomial $p$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/p(\secp),
\end{align}
then it contradicts that $\Sigma_{\RE}$ satisfies security.
\end{proof}

\begin{proof}[Proof of \cref{prop:hyb_1_univ_unc_garble}]
    Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/p(\secp)
    \end{align}
    for some polynomial $p$.
    Then, construct a QPT adversary $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$ as follows.
    \begin{enumerate}
        \item The challenger of $\Sigma_{\unc}$ samples $b\la\bit$.
        \item $\widetilde{\cA}$ samples $R[i,\beta]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
        \item $\widetilde{\cA}$ sends $( m_0,m_1)$ to the challenger, and receives $\unc.\ct_b$.
        \item $\widetilde{\cA}$ computes $\left(\widehat{\Unc.\Dec}_{\mathsf{off}}(r), \{\lab[i,\beta](r)\}_{i\in[s(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct_b[i]](r) \}_{i\in\{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$.
        \item $\widetilde{\cA}$ computes $\Lab.\ct[i,\beta]](r)\seteq R[i,\beta]+\lab[i,\beta](r)$ for all $i\in[s(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ runs $\cA$ on $\left( \widehat{\Unc.\Dec}_{\mathsf{off}}(r), \{\Lab.\ct[i,\beta](r)\}_{i\in[s(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct_b[i]](r) \}_{i\in\{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$, obtains $\rho_{\cB,\cC}$, and sends the $\cB$ register and $\{R[i,\beta]\}_{i\in[s(\secp)],\beta\in\bit}$ (resp. $\cC$ register and $\{R[i,\beta]\}_{i\in[s(\secp)],\beta\in\bit}$) to $\widetilde{\cB}$ (resp. $\widetilde{\cC}$).
        \item $\widetilde{\cB}$ (resp. $\widetilde{\cC}$) receives the secret-key $x$ from the challenger of $\Sigma_{\unc}$, sends $(x ,\{R[i,x[i]]\}_{i\in[s(\secp)]})$ and the $\cB$ register (resp. $\cC$ register) to $\cB$ (resp. $\cC$). 
        \item The experiment outputs $1$ if $b=b_\cB=b_\cC$ where $b_\cB$ and $b_\cC$ are the output of $\cB$ and $\cC$, respectively.
    \end{enumerate}
    From the construction of $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$, the adversary perfectly simulates the challenger of $\mathsf{Hyb_1}$. Therefore, if $(\cA,\cB,\cC)$ satisfies 
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/p(\secp)
    \end{align}
     for some polynomial $p$, it contradicts $\Sigma_{\unc}$ satisfies unclonable IND-CPA security.
\end{proof}



\subsection{Expanding Plaintext Space}

\begin{theorem}\label{thm:unclone_multi_space}
    If there exists a one-time unclonable secret-key encryption with single-plaintext space and decomposable quantum randomized encoding, then there exists a one-time unclonable secret-key encryption with multiple-plaintext space.
\end{theorem}

\begin{corollary}\label{cor:unclone_expnasion}
    If there exists unclonable secret-key encryption with single-plaintext space, then there exists unclonable secret-key encryption with multiple plaintext space.
\end{corollary}
\begin{corollary}\label{cor:pub_unclone_expandion}
    If unclonable public-key encryption with single-plaintext space, then there exists unclonable public-key encryption with multiple plaintext space.
\end{corollary}
\begin{proof}[Proof of \cref{cor:unclone_expnasion}]
    If there exists unclonable secret-key encryption with single-plaintext space, then there exists decomposable quantum randomized encoding and one-time unclonable secret-key encryption, which implies that there exists unclonable secret-key encryption with multiple plaintext space.
    Furthermore, the existence of unclonable secret-key encryption with single-plaintext space implies that secret-key receiver non-committing encryption with quantum ciphertexts. By combining secret-key receiver non-committing encryption with quantum ciphertexts and one-time unclonable secret-key encryption with multiple plaintext spaces, we can obtain unclonable secret-key encryption with multiple plaintext spaces.
\end{proof}

\begin{proof}[Proof of \cref{thm:unclone_multi_space}]
First, let us describe notations.
\paragraph{Notations.}
\begin{itemize}
    \item Let $\Sigma_{\RE}\seteq \RE.(\Enc,\Dec)$ be a decomposable quantum randomized encoding. For some quantum circuit $C$ and input $x$, we write $\widehat{C}_{\mathsf{off}}(r)$ to mean the off-line part of $\widehat{C}(x;r)$ and write $\lab[i,x[i]](r)$ to mean the $i$-th online encoding of $\widehat{C}(x;r)$, where $\RE.\Enc(1^\secp,C,x)$.
    Let $\ell(\secp)$ be the size of $\lab[i,x[i]]$.
    \item Let $\Sigma_{\mathsf{unclone}}\seteq\Unc.(\keygen,\Enc,\Dec)$ be one-time unclonable secret-key encryption with single-plaintext space.
    For a security parameter $\secp$, let $s(\secp)$ be the length of the secret-key that $\Unc.\keygen(1^\secp)$ generates and
    $q(\secp)$ be the length of ciphertext that $\Unc.\Enc$ generates.
    Without loss of generality, we can assume that the secret key $\sk$ generated by $\Unc.\keygen(1^\secp)$ is uniformly sampled from $\sk\la\bit^{s(\secp)}$.
    \item Let $\Dec[m_0,m_1]$ be a quantum circuit that takes as input a $s(\secp)$-length classical string $x$ and a $q(\secp)$-length quantum state $\sigma$ and computes $b\la\Unc.\Dec(1^\secp,x,\sigma)$, and outputs $m_b$.
    \item Let $C[m]$ be a quantum circuit that takes as input $s(\secp)+q(\secp)$-length quantum states, outputs $m$, and satisfies $\abs{C[m]}=\abs{\Dec[m_0,m_1]}$.
    %\item Let $\ell(\secp)$ be the size of $\widehat{C[m]}_{\mathsf{off}}(r)$, where  $\widehat{C[m]}_{\mathsf{off}}(r)$ is the off-line part of $\widehat{C[m]}(0;r)\la\mathsf{RE}.\Enc(1^\secp,C[m],0;r)$.
    %\item Let $\widehat{F}=(\widehat{F}_{\mathsf{off}},\widehat{F_1},\cdots,\widehat{F_p})$ be a quantum randomized circuit that $\RE.\Enc$ computes.
    %Let $\ell(\secp)$ be a length of output of $\widehat{F}_{\mathsf{off}}$.
\end{itemize}

\paragraph{Construction.}
We give a construction of one-time unclonable secret-key encryption  $\Sigma\seteq(\keygen,\Enc,\Dec)$ with multiple-plaintext space.
\begin{description}
    \item[$\keygen(1^\secp)$:]$ $
    \begin{itemize}
        \item Sample $x\la\bit^{s(\secp)}$.
        \item Sample $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
        \item Output $\sk\seteq (x,\{R[i]\}_{i\in[s(\secp)]})$.
    \end{itemize}
    \item[$\Enc(1^\secp,\sk,m)$:]$ $
    \begin{itemize}
        \item Compute $\widehat{C[m]}_{\mathsf{off}}(r)$.
        \item Compute $\left(\{\lab[i,b]\}_{i\in[s(\secp)],b\in\bit},\{\lab[i,0](r)\}_{i\in\{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$.
        \item Sample $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
        \item Compute $\Lab.\ct[i,x[i]]\seteq R[i]+\lab[i,x[i]](r)$ and $\Lab.\ct[i,x[i]+1](r)\seteq S[i]+\lab.\ct[i,x[i]+1](r)$ for all $i\in [s(\secp)]$.
        \item Output $\ct\seteq \left(\widehat{C[m]}_{\mathsf{off}}, \{\Lab.\ct[i,b]\}_{i\in[s(\secp)],b\in\bit},\{\lab[i,0]\}_{i\in\{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$.
    \end{itemize}
    \item[$\Dec(\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R[i]\}_{i\in[s(\secp)]}\right)$ and $\ct=\left(\widehat{C[m]}_{\mathsf{off}}, \{\Lab.\ct[i,b]\}_{i\in[s(\secp)],b\in\bit},\{\lab[i,0]\}_{i\in\{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}}\right)$.
        \item Compute $\lab[i,x[i]]\seteq \Lab.\ct[i,x[i]]+R[i]$ for all $i\in[s(\secp)]$.
        \item Compute $\Dec(1^\secp,\widehat{C[m]}_{\mathsf{off}},\{\lab[i,x[i]]\}_{i\in[s(\secp)]},\{\lab[i,0]\}_{i\in[q(\secp)]} )$ and outputs its output.
    \end{itemize}
\end{description}
\begin{theorem}\label{thm:expnad_unc}
    $\Sigma$ is one-time unclonable secret-key encryption with multiple plaintext spaces if $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding and there exists one-time unclonable secret-key encryption with single-plaintext space.  
\end{theorem}

\begin{proof}[Proof of \cref{thm:expnad_unc}]
We describe the sequence of hybrids against adversary $(\cA,\cB,\cC)$.
\begin{description}
        \item[$\mathsf{Hyb_0}$:] This is the original one-time unclonable IND-CPA security experiment.
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{s(\secp)}$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\widehat{C[m_b]}_{\mathsf{off}}(r)$, $\lab[i,\beta](r)$ for all $i\in[s(\secp)]$ and $\beta\in\bit$ and $\lab[i,0](r)$ for all $i\in\{s(\secp)+1,\cdots, s(\secp)+q(\secp)\}$.
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$, and computes $\Lab.\ct[i,x[i]](r)\seteq R[i]+\lab[i,x[i]](r)$ and $\Lab.\ct[i,x[i]+1](r)\seteq S[i]+\lab[i,x[i]+1](r)$ for all $i\in[s(\secp)]$.
        \item The challenger sends $\left(\widehat{C[m_b]}_{\mathsf{off}}(r),\{\Lab.\ct[i,\beta](r)\}_{i\in[s(\secp)],\beta\in\bit}, \{\lab[i,0](r)\}_{i\in\{s(\secp)+1,\cdots, s(\secp)+q(\secp)\}}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[s(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:]$ $
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\Unc.\keygen(1^\secp)$ and $R[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes  $\unc.\ct_b\la\Unc.\Enc(1^\secp,x,b)$.
        \item The challenger computes $\widehat{\Dec}[m_0,m_1]_{\mathsf{off}}(r)$ and $\lab[i,\beta](r)$ for all $i\in[s(\secp)]$ and $\beta\in\bit$ and $\lab[i,\unc.\ct_b[i]](r)$ for all $i\in[q(\secp)]$.
        \item The challenger samples $S[i]\la\bit^{\ell(\secp)}$ for all $i\in[s(\secp)]$, and computes $\Lab.\ct[i,x[i]](r)\seteq R[i]+\lab[i,x[i]](r)$ and $\Lab.\ct[i,x[i]+1](r)\seteq S[i]+\lab[i,x[i]+1](r)$ for all $i\in[s(\secp)]$.
        \item The challenger sends $\left(\widehat{\Dec}[m_0,m_1]_{\mathsf{off}}(r),\{\Lab.\ct[i,\beta](r)\}_{i\in[s(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct[i]](r)\}_{i\in[q(\secp)]}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R[i]\}_{i\in[s(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
\end{description}
\cref{thm:expnad_unc} follows from the following \cref{prop:hyb_0_hyb_1_unc_expand,prop:hyb_1_unc_expand}.
\begin{proposition}\label{prop:hyb_0_hyb_1_unc_expand}
If $\Sigma_{\mathsf{RE}}$ is decomposable quantum randomized encoding, then
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\leq\negl(\secp).
\end{align}
\end{proposition}

\begin{proposition}\label{prop:hyb_1_unc_expand}
    If there exists a one-time unclonable secret-key encryption $\Sigma_{\Unc}$ with single-plaintext space, then
    \begin{align}
        \abs{\Pr[\mathsf{Hyb}_1=1]}\leq \frac{1}{2}+\negl(\secp).
    \end{align}
\end{proposition}
\end{proof}

Because the proof of \cref{prop:hyb_0_hyb_1_unc_expand} is almost the same as \cref{prop:hyb_0_hyb_1_univ_unc_garble}, and thus we skip the proof.

\if0
\begin{proof}[Proof of \cref{prop:hyb_0_hyb_1_unc_univ}]
We prove the \cref{prop:hyb_0_hyb_1_unc_univ}, via a standard hybrid argument.
Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ such that 
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/p(\secp)
\end{align}
for some polynomial $p$.
Then, we construct a QPT adversary $\widetilde{\cA}$ that breaks the security of decomposable quantum randomized encoding $\Sigma_{\mathsf{RE}}$ as follows.
\begin{enumerate}
    \item $\widetilde{\cA}$ samples $b\la\bit$ and $x\la\bit^{\ell(\secp)}$ and $z\la\bit^{\ell(\secp)}$.
    \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from the $\cA$.
    \item $\widetilde{\cA}$ computes $\unc.\sk\la\Unc.\keygen(1^\secp)$ and $\unc.\ct_b\la\Unc.\Enc(1^\secp,\unc.\sk,b)$.
    \item $\widetilde{\cA}$ sends $\left(\{C[m_b],0^p(\secp)\},  \{\widehat{D}[\unc.\sk,m_0,m_1],\unc.\ct_b \} \right)$ to the challenger of $\Sigma_{\mathsf{RE}}$.
    \item The challenger samples $b^*\la\bit$, and do the following.
    \begin{itemize}
        \item If $b^*=0$, then the challenger computes $\left(\widehat{C[m_b]}_{\mathsf{off}}(r), \{\widehat{C[m_b]}_i(0;r)\}_{i\in[p(\secp)]}\right)\la\RE.\Enc(1^\secp,C[m_b],0^{p(\secp)})$.
        % and sends $\left(\widehat{C[m_b]}_{\mathsf{off}}(r), \{\widehat{C[m_b]}_i(0;r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
        \item If $b^*=1$, then the challenger computes $\left(\widehat{D}[\unc.\sk,m_0,m_1]_{\mathsf{off}}(r), \{\widehat{D}[\unc.\sk,m_0,m_1]_i(\unc.\ct_b[i];r)\}_{i\in[p(\secp)]}\right)\la\RE.\Enc(1^\secp,D[\unc.\sk,m_0,m_1],\unc.\ct_b)$. 
        %and sends $\left(\widehat{D}[\unc.\sk,m_0,m_1]_{\mathsf{off}}(r), \{\widehat{D}[\unc.\sk,m_0,m_1]_i(\unc.\ct_b[i];r)\}_{i\in[p(\secp)]}\right)$ to $\cB$.
    \end{itemize}
    \item $\widetilde{\cA}$ receives $(\widehat{F}_{\mathsf{off}},\{\mathsf{Lab_i}\}_{i\in[p(\secp)]})$ from the challenger.
    Here, if $b^*=0$, then $(\widehat{F}_{\mathsf{off}},\{\mathsf{Lab_i}\}_{i\in[p(\secp)]})=\left(\widehat{C[m_b]}_{\mathsf{off}}(r), \{\widehat{C[m_b]}_i(0;r)\}_{i\in[p(\secp)]}\right)$.
    Otherwise, $(\widehat{F}_{\mathsf{off}},\{\mathsf{Lab_i}\}_{i\in[p(\secp)]})=\left(\widehat{D}[\unc.\sk,m_0,m_1]_{\mathsf{off}}(r), \{\widehat{D}[\unc.\sk,m_0,m_1]_i(\unc.\ct_b[i];r)\}_{i\in[p(\secp)]}\right)$.
    \item $\widetilde{\cA}$ computes $\ske.\ct\seteq Z^zX^x\widehat{F}_{\mathsf{off}}X^xZ^z$, and sends $(\ske.\ct,\{\mathsf{Lab_i}\}_{i\in[p(\secp)]})$ to $\cA$.
    \item $\cA$ generates $\rho_{\cB,\cC}$ and sends the corresponding register to $\cB$ and $\cC$
    \item $\widetilde{\cA}$ sends $x$ and $z$ to $\cB$ and $\cC$.
    \item $\widetilde{\cA}$ outputs $1$ if $b=b_\cB=b_\cC$, and outputs $0$ otherwise.
\end{enumerate}
From the construction, if $b^*=0$, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_0}$. Otherwise, $\widetilde{\cA}$ perfectly simulates the challenger of $\mathsf{Hyb_1}$. 
Furthermore, we have $C[m_b](0^{p(\secp)})=D[\unc.\sk,m_0,m_1](\unc.\ct_b)$.
Therefore, if there exists a QPT adversary $(\cA,\cB,\cC)$ such that
\begin{align}
    \abs{\Pr[\mathsf{Hyb_0}=1]-\Pr[\mathsf{Hyb_1}=1]}\geq 1/p(\secp)
\end{align}
for some polynomial $p$, 
then it contradicts that $\Sigma_{\mathsf{RE}}$ satisfies security.
\end{proof}
\fi


\begin{proof}[Proof of \cref{prop:hyb_1_unc_expand}]
    Assume that there exists a QPT adversary $(\cA,\cB,\cC)$ such that
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq \frac{1}{2}+1/p(\secp)
    \end{align}
    for some polynomial $p$.
    Then, construct a QPT adversary $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$ that breaks the unclonable IND-CPA security of $\Sigma_{\unc}$.
    \begin{enumerate}
        \item The challenger of $\Sigma_{\unc}$ samples $b\la\bit$.
        \item $\widetilde{\cA}$ samples $R[i,\beta]$ for all $i\in[s(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ receives $(m_0,m_1)$ from $\cA$.
        \item $\widetilde{\cA}$ sends $(0,1)$ to the challenger of $\Sigma_\unc$, and receives $\unc.\ct_b$.
        \item $\widetilde{\cA}$ computes $\widehat{\Dec}[m_0,m_1]_{\mathsf{off}}(r)$ and $\lab[i,\beta](r)$ for all $i\in[s(\secp)]$ and $\beta\in\bit$ and $\lab[i,\unc.\ct_b[i]](r)$ for all $i\in[q(\secp)]$.
        \item $\widetilde{\cA}$ computes $\Lab.\ct[i,\beta]\seteq R[i,\beta]$ for all $i\in[s(\secp)]$ and $\beta\in\bit$.
        \item $\widetilde{\cA}$ runs $\cA$ on $\left(\widehat{\Dec}[m_0,m_1]_{\mathsf{off}}(r),\{\Lab.\ct[i,\beta](r)\}_{i\in[s(\secp)],\beta\in\bit},\{\lab[i,\unc.\ct_b[i]]\}_{i\in\{s(\secp)+1,\cdots,s(\secp)+q(\secp)\}} \right)$, obtains $\rho_{\cB,\cC}$, and sends the $\cB$ register and $\{R[i,\beta]\}_{i\in[s(\secp)],\beta\in\bit}$ (resp. register $\cC$ and $\{R[i,\beta]\}_{i\in[s(\secp)],\beta\in\bit}$) to $\widetilde{\cB}$ (resp. $\widetilde{\cC}$).
        \item $\widetilde{\cB}$ (resp. $\widetilde{\cC}$) receives the secret key $x$ from the challenger of $\Sigma_\unc$, sends $(x,\{R[i,x[i]]\}_{i\in[s(\secp)]})$ and the $\cB$ register (resp. $\cC$ register) to $\cB$ (resp. $\cC$).
        \item The experiment outputs $1$ if $b=b_\cB=b_\cC$, and $0$ otherwise, where $b_\cB$ and $b_\cC$ are the outputs of $\cB$ and $\cC$, respectively.
    \end{enumerate}
From the construction of $(\widetilde{\cA},\widetilde{\cB},\widetilde{\cC})$, it perfectly simulates the challenger of $\mathsf{Hyb_1}$. Therefore, if $(\cA,\cB,\cC)$ satisfies 
    \begin{align}
        \Pr[\mathsf{Hyb_1}=1]\geq 1/2+1/p(\secp)
    \end{align}
     for some polynomial $p$, it contradicts that $\Sigma_{\unc}$ satisfies unclonable IND-CPA security.
\end{proof}



\if0
\paragraph{Notations.}
\begin{itemize}
    \item Let $\Sigma_{\mathsf{unclone}}\seteq\mathsf{UN}.(\keygen,\Enc,\Dec)$ be one-time unclonable secret-key encryption with single-plaintext space.
    For a security parameter $\secp$, let $p(\secp)$ be the length of the classical secret key that $\mathsf{UN}.\keygen(1^\secp)$ generates.
    \item Let $C[m]$ be a quantum circuit that takes as input $p(\secp)$-length classical string, and outputs $m$.
    \item Let $\Sigma_{\RE}\seteq \RE.(\Enc,\Dec,\Sim)$ be a decomposable quantum randomized encoding.
    \item Let $\widehat{F}=(\widehat{F}_{\mathsf{off}},\widehat{F_1},\cdots,\widehat{F_p})$ be a quantum randomized circuit that $\RE.\Enc$ computes.
    For some $i\in[p(\secp)]$, let $\ell(\secp)$ be a length of $\widehat{F_i}$ 
\end{itemize}

\paragraph{Construction.}
We give a construction of one-time unclonable secret-key encryption with multiple plaintext space $\Sigma\seteq(\keygen,\Enc,\Dec)$.
\begin{description}
    \item[$\keygen(1^\secp)$:]$ $
    \begin{itemize}
        \item Sample $x\la\bit^{p(\secp)}$
        \item Sample $R_{i}\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Output $\sk\seteq \left(x,\{R_{i}\}_{i\in[p(\secp)]}\right)$.
    \end{itemize}
    \item[$\Enc(\sk,m)$:]$ $
    \begin{itemize}
        \item For a constant circuit $C[m]$, generate $\widehat{F}_{\mathsf{off}}(C[m];r)$.
        \item Generate $\widehat{F_{i}}(b;r)$ for all $i\in[p(\secp)]$ and $b\in\bit$.
        \item Sample $S_i\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item Compute $\ske.\ct_{i,x_i}\seteq R_i+\widehat{F}_{i}(x_i;r) $ and $\ske.\ct_{i,x_i+1}\seteq S_i+\widehat{F}_{i}(x_i+1;r)$  for all $i\in[p(\secp)]$.
        \item Output $\ct\seteq \left(\widehat{F}_{\mathsf{off}}(C[m];r), \{\ske.\ct_{i,b}\}_{i\in[p(\secp)],b\in\bit}\right)$.
    \end{itemize}
    \item[$\Dec(\sk,\ct)$:]$ $
    \begin{itemize}
        \item Parse $\sk=\left(x,\{R_i\}_{i\in[p(\secp)]}\right)$ and $\ct=\left(\widehat{F}_{\mathsf{off}}(C[m];r), \{\ske.\ct_{i,b}\}_{i\in[p(\secp)],b\in\bit}\right)$.
        \item Compute $ \widehat{F}_i(x_i;r)\seteq\ske.\ct_{i,x[i]}+R_i$ for all $i\in[p(\secp)]$.
        \item Compute $\Dec(\widehat{F}(C[m],x;r))$ and outputs its output.
    \end{itemize}
\end{description}

We describe the sequence of hybrids against adversary $(\cA,\cB,\cC)$.
\begin{description}
    \item[$\mathsf{Hyb_0}$:] This is the original one-time unclonable IND-CPA security experiment.
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R_i\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \item The challenger computes $\widehat{F}_{\mathsf{off}}(C[m_b];r)$ and $\widehat{F}_i(\beta;r)$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item The challenger samples $S_i$ for all $i\in[p(\secp)]$, and computes $\ske.\ct_{i,x_i}\seteq R_i+\widehat{F_i}(x_i;r)$ and $\ske.\ct_{i,x_i+1}\seteq S_i+\widehat{F_i}(x_i+1;r)$ for all $i\in[p(\secp)]$.
        \item The challenger sends $\left(\widehat{F}_{\mathsf{off}}(C[m_b];r),\{\ske.\ct_{i,b}\}_{i\in[p(\secp)],b\in\bit}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R_i\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
    \item[$\mathsf{Hyb_1}$:]$ $
    \begin{enumerate}
        \item The challenger samples $b\la\bit$.
        \item The challenger samples $x\la\bit^{p(\secp)}$ and $R_i\la\bit^{\ell(\secp)}$ for all $i\in[p(\secp)]$.
        \item The adversary $\cA$ sends $(m_0,m_1)$ to the challenger.
        \color{blue}
        \item The challenger computes $\mathsf{un}.\sk\la\mathsf{UN}.\keygen(1^{\secp})$.
        \color{black}
        \item The challenger computes $\widehat{F}_{\mathsf{off}}(D[\mathsf{un}.\sk,m_0,m_1];r)$ and $\widehat{F}_i(\beta;r)$ for all $i\in[p(\secp)]$ and $\beta\in\bit$.
        \item The challenger samples $S_i$ for all $i\in[p(\secp)]$, and computes $\ske.\ct_{i,x_i}\seteq R_i+\widehat{F_i}(x_i;r)$ and $\ske.\ct_{i,x_i+1}\seteq S_i+\widehat{F_i}(x_i+1;r)$ for all $i\in[p(\secp)]$.
        \item The challenger sends $\left(\widehat{F}_{\mathsf{off}}(D[x,m_0,m_1];r),\{\ske.\ct_{i,b}\}_{i\in[p(\secp)],b\in\bit}\right)$ to $\cA$.
        \item $\cA$ produces $\rho_{\cB,\cC}$ and sends the corresponding registers to $\cB$ and $\cC$.
        \item $\cB$ and $\cC$ receives $\left(x,\{R_i\}_{i\in[p(\secp)]}\right)$, and outputs $b_\cB$ and $b_\cC$.
        \item The experiment outputs $1$ if $b_\cB=b_\cC=b$, and otherwise $0$.
    \end{enumerate}
\end{description}
\fi
\end{proof}


==> Sec_Padding_Circuit.tex <==
% !TEX root = main.tex
\section{On Padding Quantum Circuits}
We give a formal definition of $C[m]_{\secp,p}$, where $m\in\bit^{n(\secp)}$ for some polynomial $n$ and $p(\secp)\geq n(\secp)$ for all $\secp\in\N$.

$C[m]_{\secp,p}$ has the following topology $\cT\seteq (\cI,\cO,\cB,\cW,\cZ,\cF)$.
The input set $\cI$ has $3p(\secp)$-vertex and the auxiliary set $\cZ$ has $p(\secp)$-vertex.
The output set $\cO$ has $3p(\secp)$-vertex and the discarded set $\cF$ has $3p(\secp)-n(\secp)$-vertex.

$\cB$ has the  


